Fitting peculiar spectral profiles in He I 10830 \r{A} absorption features

The new generation of solar instruments provides better spectral, spatial, and temporal resolution for a better understanding of the physical processes that take place on the Sun. Multiple-component profiles are more commonly observed with these instruments. Particularly, the He I 10830 \r{A} triplet presents such peculiar spectral profiles, which give information on the velocity and magnetic fine structure of the upper chromosphere. The purpose of this investigation is to describe a technique to efficiently fit the two blended components of the He I 10830 \r{A} triplet, which are commonly observed when two atmospheric components are located within the same resolution element. The observations used in this study were taken on 2015 April 17 with the very fast spectroscopic mode of the GREGOR Infrared Spectrograph (GRIS) attached to the 1.5-meter GREGOR solar telescope, located at the Observatorio del Teide, Tenerife, Spain. We apply a double-Lorentzian fitting technique using Levenberg-Marquardt least-squares minimization. This technique is very simple and much faster than inversion codes. Line-of-sight Doppler velocities can be inferred for a whole map of pixels within just a few minutes. Our results show sub- and supersonic downflow velocities of up to 32 km/s for the fast component in the vicinity of footpoints of filamentary structures. The slow component presents velocities close to rest.

==> an-jour <==
@STRING{aa      = "A\&A"}
@STRING{aar     = "A\&ARv"}
@STRING{aas     = "A\&ASS"}
@STRING{advsr   = "Adv. Space Res."}
@STRING{advast  = "Adv. Astron."}
@STRING{ajp     = "Aust. J. Phys."}
@STRING{an      = "AN"}
@STRING{ao      = "Appl. Opt."}
@STRING{apj     = "ApJ"}
@STRING{apjl    = "ApJL"}
@STRING{apjs    = "ApJS"}
@STRING{asp     = "ASP Conf. Ser."}
@STRING{araa    = "ARA\&A"}
@STRING{baas    = "Bull. Am. Astron. Soc."}
@STRING{baic    = "Bull. Astron. Insti. Czech."}
@STRING{chinjaa = "ChJAA"}
@STRING{grl     = "GRL"}
@STRING{hob     = "Hvar Obs. Bull."}
@STRING{iaus    = "IAU Symp."}
@STRING{jam     = "J. Appl. Meteor."}
@STRING{jcop    = "J. Comp. Phy."}
@STRING{lrsp    = "Liv. Rev. Space Phy."}
@STRING{nat     = "Nature"}
@STRING{nar     = "New Astron.\ Rev."}
@STRING{ol      = "Opt. Lett."}
@STRING{pasj    = "PASJ"}
@STRING{pasp    = "PASP"}
@STRING{posp    = "Proc. SPIE"}
@STRING{qjas    = "Quart. J. R. Astron. Soc"}
@STRING{sc      = "Science"}
@STRING{sp      = "SoPh"}
@STRING{sterne  = "Die Sterne"}
@STRING{sw      = "Sterne und Weltraum"}


==> sjgm <==

%====     AAAA    ==============================================================


@ARTICLE{Al2004,
   author = {{Al}, N. and {Bendlin}, C. and {Hirzberger}, J. and
            {Kneer}, F. and {Trujillo Bueno}, J.},
    title = "{Dynamics of an Enhanced Network Region Observed in H{$\alpha$}}",
  journal = aa,
     year = 2004,
   volume = 418,
    pages = {1131-1139},
      doi = {10.1051/0004-6361:20034501}
}

@INPROCEEDINGS{Al1998,
   author = {{Al}, N. and {Bendlin}, C. and {de Boer}, C. R. and
            {Denker}, C. and {Kneer}, F. and {Schmitt}, D. and
            {Volkmer}, R. and {Wilken}, V.},
    title = "{Dynamics of Solar Fine Structure. Observation with High Spatial
            Resolution}",
booktitle = {Cool Stars, Stellar Systems, and the Sun},
     year = 1998,
   series = asp,
   volume = 154,
   editor = {{Donahue}, R. A. and {Bookbinder}, J. A.},
    pages = {553-558}
}

@ARTICLE{Alissandrakis1990,
   author = {{Alissandrakis}, C. E. and {Tsiropoula}, G. and {Mein}, P.},
    title = "{Physical Parameters of Solar H$\alpha$ Absorption Features Derived
            with the Cloud Model}",
  journal = aa,
     year = 1990,
   volume = 230,
    pages = {200-212}
}

@BOOK{allen1973,
   author = {{Allen}, C. W.},
    title = "{Astrophysical Quantities}",
  edition = {3rd edn.},
publisher = {Athlone Press},
  address = {London}, 
     year = 1973
}

@ARTICLE{AllendePrieto2004,
   author = {{Allende Prieto}, C. and {Asplund}, M. and {Fabiani Bendicho}, P.
	},
    title = "{Center-to-limb variation of solar line profiles as a test of NLTE line formation 
calculations}",
  journal = aap,
   eprint = {astro-ph/0405154},
 keywords = {Sun: photosphere, line: formation, line: profiles},
     year = 2004,
   volume = 423,
    pages = {1109-1117},
      doi = {10.1051/0004-6361:20047050}
}

@ARTICLE{Asensio2008,
   author = {{Asensio Ramos}, A. and {Trujillo Bueno}, J. and {Landi Degl'Innocenti}, E.
	},
    title = "{Advanced Forward Modeling and Inversion of Stokes Profiles Resulting from the Joint Action of the Hanle and Zeeman Effects}",
  journal = apj,
archivePrefix = "arXiv",
   eprint = {0804.2695},
     year = 2008,
   volume = 683,
    pages = {542-565},
      doi = {10.1086/589433}
}

@ARTICLE{Aulanier2010,
   author = {{Aulanier}, G. and {T{\"o}r{\"o}k}, T. and
            {D{\'e}moulin}, P. and {DeLuca}, E. E.},
    title = "{Formation of Torus-Unstable Flux Ropes and Electric Currents in
            Erupting Sigmoids}",
  journal = apj,
     year = 2010,
   volume = 708,
    pages = {314-333},
      doi = {10.1088/0004-637X/708/1/314}
}

@INPROCEEDINGS{Avrett1994,
   author = {{Avrett}, E.~H. and {Fontenla}, J.~M. and {Loeser}, R.},
    title = "{Formation of the Solar 10830 Angstrom Line}",
booktitle = {Infrared Solar Physics},
     year = 1994,
   series = {IAU Symposium},
   volume = 154,
   editor = {{Rabin}, D.~M. and {Jefferies}, J.~T. and {Lindsey}, C.},
    pages = {35},
}

@ARTICLE{Azuah2009,
   author = {{Azuah}, R. T. and {Kneller},L. R. and {Qiu}, Y. and
            {Tregenna-Piggott}, P. L. W. and {Brown}, C. M. and
            {Copley}, J. R. D. and {Dimeo}, R. M.},
    title = "{DAVE: A Comprehensive Software Suite for the Reduction,
            Visualization, and Analysis of Low Energy Neutron Spectroscopic
            Data}",
  journal = "{J.\ Res.\ Natl.\ Inst.\ Stan.\ Technol.}",
     year = 2009,
   volume = 114,
    pages = {341-358}
}

@INPROCEEDINGS{AznarCuadrado2005,
   author = {{Aznar Cuadrado}, R. and {Solanki}, S.~K. and {Lagg}, A.},
    title = "{Supersonic Downflows in the Solar Chromosphere are Very Common}",
booktitle = {Chromospheric and Coronal Magnetic Fields},
     year = 2005,
   series = {ESA Special Publication},
   volume = 596,
   editor = {{Innes}, D.~E. and {Lagg}, A. and {Solanki}, S.~A.},
      eid = {49.1},
    pages = {49.1}
}

@INPROCEEDINGS{AznarCuadrado2007,
   author = {{Aznar Cuadrado}, R. and {Solanki}, S.~K. and {Lagg}, A.},
    title = "{Velocity distribution of chromospheric downflows}",
booktitle = {Modern solar facilities - advanced solar science},
     year = 2007,
   editor = {{Kneer}, F. and {Puschmann}, K.~G. and {Wittmann}, A.~D.},
    pages = {173}
}

%====     BBBB    ==============================================================

@ARTICLE{Balthasar2010,
   author = {{Balthasar}, H. and {Muglach}, K.},
    title = "{The Three-Dimensional Structure of Sunspots. II.\ The Moat Flow at
            two Different Heights}",
  journal = aa,
     year = 2010,
   volume = 511,
    pages = {A67}
}

@INPROCEEDINGS{Balthasar2009,
   author = {{Balthasar}, H. and {Bello Gonz{\'a}lez}, N. and {Collados}, M. and
            {Denker}, C. and {Hofmann}, A. and {Kneer}, F. and
            {Puschmann}, K. G.},
    title = "{A Full-Stokes Polarimeter for the GREGOR Fabry-P{\'e}rot
            Interferometer}",
booktitle = {Cosmic Magnetic Fields: From Planets, to Stars and Galaxies},
     year = 2009,
   series = iaus,
   volume = 259,
   editor = {{Strassmeier}, K. G. and {Kosovichev}, A. G. and
            {Beckmann}, J. E.},
    pages = {665-666}
}

@ARTICLE{Balthasar2008,
   author = {{Balthasar}, H. and {G{\"o}m{\"o}ry}, P.},
    title = "{The Three-Dimensional Structure of Sunspots. I. The Height
            Dependence of the Magnetic Field}",
  journal = aa,
     year = 2008,
   volume = 488,
    pages = {1085-1092}
}

@ARTICLE{Balthasar2007a,
   author = {{Balthasar}, H.},
    title = "{Rotational Periodicities in Sunspot Relative Numbers}",
  journal = aa,
     year = 2007,
   volume = 471,
    pages = {281-287}
}

@INPROCEEDINGS{Balthasar2007b,
   author = {{Balthasar}, H. and {von der L{\"u}he}, O. and {Kneer}, F. and
            {Staude}, J. and {Volkmer}, R. and {Berkefeld}, T. and
            {Caligari}, P. and {Collados}, M. and {Halbgewachs}, C. and
            {Heidecke}, F. and {Hofmann}, A. and {Klva{\v n}a}, M. and
            {Nicklas}, H. and {Popow}, E. and {Puschmann}, K. and
            {Schmidt}, W. and {Sobotka}, M. and {Soltau}, D. and
            {Strassmeier}, K. and {Wittmann}, A.},
    title = "{GREGOR: The New German Solar Telescope}",
booktitle = {The Physics of Chromospheric Plasmas},
     year = 2007,
   series = asp,
   volume = 368,
   editor = {{Heinzel}, P. and {Dorotovi{\v c}}, I. and {Rutten}, R. J.},
    pages = {605-610}
}

@ARTICLE{Balthasar2006,
   author = {{Balthasar}, H.},
    title = "{Vertical Current Densities and Magnetic Gradients in Sunspots}",
  journal = aa,
     year = 2006,
   volume = 449,
    pages = {1169-1176}
}

@ARTICLE{Balthasar2005,
   author = {{Balthasar}, H. and {Collados}, M.},
    title = "{Some Properties of an Isolated Sunspot}",
  journal = aa,
     year = 2005,
   volume = 429,
    pages = {705-711}
}

@ARTICLE{Balthasar2000,
   author = {{Balthasar}, H. and {Collados}, M. and {Muglach}, K.},
    title = "{Oscillations in a Solar Pore}",
  journal = an,
     year = 2000,
   volume = 321,
    pages = {121-127}
}

@ARTICLE{Battaglia2011,
   author = {{Battaglia}, M. and {Kontar}, E. P.},
    title = "{Height Structure of X-Ray EUV and White-Light Emission in a Solar
            Flare}",
  journal = {ArXiv e-prints},
   pages = {1107.3808},
     year = 2011
}

@ARTICLE{Beauregard2012,
   author = {{Beauregard}, L. and {Verma}, M. and {Denker}, C.},
    title = "{Horizontal Flows Concurrent with an X2.2 Flare in the Active
            Region NOAA 11158}",
  journal = an,
     year = 2012,
   volume = 333,
    pages = {125},
      doi = {10.1002/asna.201111631}
}

@ARTICLE{Beck2005,
   author = {{Beck}, C. and {Schmidt}, W. and {Kentischer}, T. and
            {Elmore}, D.},
    title = "{Polarimetric Littrow Spectrograph -- Instrument Calibration and
            First Measurements}",
  journal = aa,
     year = 2005,
   volume = 437,
    pages = {1159-1167}
}

@ARTICLE{Beckers2001,
   author = {{Beckers}, J. M.},
    title = "{A Seeing Monitor for Solar and Other Extended Object
            Observations}",
  journal = expast,
     year = 2001,
   volume = 12,
    pages = {1-20}
}

@ARTICLE{Beckers1972,
   author = {{Beckers}, J. M.},
    title = "{Solar Spicules}",
  journal = araa,
     year = 1972,
   volume = 10,
    pages = {73-100}
}

@ARTICLE{Beckers1968,
   author = {{Beckers}, J. M. and {Schr{\"o}ter}},
    title = "{The Intensity, Velocity and Magnetic Structure of a Sunspot
            Region. I.\ Observational Technique; Properties of Magnetic Knots}",
  journal = sp,
     year = 1968,
   volume = 4,
    pages = {142-164}
}

@PHDTHESIS{Beckers1964,
   author = {{Beckers}, J. M.},
    title = "{A Study of the Fine Structures in the Solar Chromosphere}",
   school = {University of Utrecht},
     year = 1964
}
@ARTICLE{Beeck2015,
   author = {{Beeck}, B. and {Sch{\"u}ssler}, M. and {Cameron}, R. H. and 
            {Reiners}, A.},
    title = "{Three-Dimensional Simulations of Near-Surface Convection in
            Main-Sequence Stars. III. The Structure of Small-Scale Magnetic
            Flux Concentrations}",
  journal = aa,
     year = 2015,
    pages = {in press}
}

@ARTICLE{BelloGonzalez2009,
   author = {{Bello Gonz{\'a}lez}, N. and {Yelles Chaouche}, L. and
            {Okunev}, O. and {Kneer}, F.},
    title = "{Dynamics of Small-Scale Magnetic Fields on the Sun: Observations
            and Numerical Simulations}",
  journal = aa,
     year = 2009,
   volume = 494,
    pages = {1091-1106}
}

@ARTICLE{BelloGonzalez2008,
   author = {{Bello Gonz{\'a}lez}, N. and {Kneer}, F.},
    title = "{Narrow-Band Full Stokes Polarimetry of Small Structures on the Sun
            with Speckle Methods}",
  journal = aa,
     year = 2008,
   volume = 480,
    pages = {265-275},
      doi = {10.1051/0004-6361:20078567}
}

@ARTICLE{BelloGonzalez2005,
   author = {{Bello Gonz{\'a}lez}, N. and {Okunev}, O. V. and
            {Dom{\'{\i}}nguez Cerde{\~n}a}, I. and {Kneer}, F. and
            {Puschmann}, K. G.},
    title = "{Polarimetry of Sunspot Penumbrae with High Spatial Resolution}",
  journal = aa,
     year = 2005,
   volume = 434,
    pages = {317-327}
}

@ARTICLE{BellotRubio2008,
   author = {{Bellot Rubio}, L. R. and {Tritschler}, A. and
            {Mart{\'{\i}}nez Pillet}, V.},
    title = "{Spectropolarimetry of a Decaying Sunspot Penumbra}",
  journal = apj,
     year = 2008,
   volume = 676,
    pages = {698-703}
}

@ARTICLE{BellotRubio2007,
   author = {{Bellot Rubio}, L. R. and {Tsuneta}, S. and {Ichimoto}, K. and
            {Katsukawa}, Y. and {Lites}, B. W. and {Nagata}, S. and
            {Shimizu}, T. and {Shine}, R. A. and {Suematsu}, Y. and 
            {Tarbell}, T. D. and {Title}, A. M. and {del Toro Iniesta}, J. C.},
    title = "{Vector Spectropolarimetry of Dark-Cored Penumbral Filaments with
            Hinode}",
  journal = apjl,
     year = 2007,
   volume = 668,
    pages = {L91-L94}
}

@ARTICLE{BellotRubio2006,
   author = {{Bellot Rubio}, L. R. and {Schlichenmaier}, R. and
            {Tritschler}, A.},
    title = "{Two-Dimensional Spectroscopy of a Sunspot. III. Thermal and
            Kinematic Structure of the Penumbra at 0.5$^{\prime\prime}$
            Resolution}",
  journal = aa,
     year = 2006,
   volume = 453,
    pages = {1117-1127}
}

@ARTICLE{BellotRubio2005,
   author = {{Bellot Rubio}, L. R. and {Langhans}, K. and 
            {Schlichenmaier}, R.},
    title = "{Multi-Line Spectroscopy of Dark-Cored Penumbral Filaments}",
  journal = aa,
     year = 2005,
   volume = 443,
    pages = {L7-L10}
}

@ARTICLE{BellotRubio2004,
   author = {{Bellot Rubio}, L. R. and {Balthasar}, H. and 
            {Collados}, M.},
    title = "{Two Magnetic Components in Sunspot Penumbrae}",
  journal = aa,
     year = 2004,
   volume = 427,
    pages = {319-334}
}

@INPROCEEDINGS{BellotRubio2003a,
   author = {{Bellot Rubio}, L. R.},
    title = "{The Fine Structure of the Penumbra: from Observations to Realistic
            Physical Models}",
booktitle = {Solar Polarization},
     year = 2003,
   series = asp,
   volume = 307,
   editor = {{Trujillo-Bueno}, J. and {Sanchez Almeida}, J.},
    pages = {301-323}
}

@ARTICLE{BellotRubio2003b,
   author = {{Bellot Rubio}, L. R. and {Balthasar}, H. and {Collados}, M.
            and {Schlichenmaier}, R.},
    title = "{Field-Aligned Evershed Flows in the Photosphere of a Sunspot
            Penumbra}",
  journal = aa,
     year = 2003,
   volume = 403,
    pages = {L47-L50}
}

@ARTICLE{Bendlin1992,
   author = {{Bendlin}, C. and {Volkmer}, R. and {Kneer}, F.},
    title = "{A New Instrument for High Resolution, Two-Dimensional Solar
            Spectroscopy}",
  journal = aa,
     year = 1992,
   volume = 257,
    pages = {817-823}
}

@ARTICLE{Benevolenskaya1998,
   author = {{Benevolenskaya}, E. E.},
    title = "{A Model of the Double Magnetic Cycle of the Sun}",
  journal = apjl,
     year = 1998,
   volume = 509,
    pages = {L49-L52}
}

@INPROCEEDINGS{Bentley1998,
   author = {{Bentley}, R. D. and {Freeland}, S. L.},
    title = "{SOLARSOFT -- An Analysis Environment for Solar Physics}",
booktitle = {Crossroads for European Solar and Heliospheric Physics.
            Recent Achievements and Future Mission Possibilities},
     year = 1998,
   series = {ESA Spec. Publ.},
   volume = 417,
    pages = {225-228}
}

@ARTICLE{Berger1998,
   author = {{Berger}, T. E. and {L{\"o}fdahl}, M. G. and {Shine}, R. S. and
            {Title}, A. M.},
    title = "{Measurements of Solar Magnetic Element Motion from High-Resolution
            Filtergrams}",
  journal = apj,
     year = 1998,
   volume = 495,
    pages = {973-993}
}

@ARTICLE{Berger1995,
   author = {{Berger}, T. E. and {Schrijver}, C. J. and {Shine}, R. A. and
            {Tarbell}, T. D. and {Title}, A. M. and {Scharmer}, G.},
    title = "{New Observations of Subarcsecond Photospheric Bright Points}",
  journal = apj,
     year = 1995,
   volume = 454,
    pages = {531-544}
}

@ARTICLE{Berkefeld2012,
   author = {{Berkefeld }, T. and {Schmidt}, D. and {Soltau}, D. and
            {von der L{\"u}he}, O. and {Heidecke}, F.},
    title = "{The GREGOR Adaptive Optics System}",
  journal = an,
     year = 2012,
   volume = 333,
    pages = {863},
      doi = {10.1002/asna.201211739}
}

@ARTICLE{Berkefeld2010,
   author = {{Berkefeld}, T. and {Soltau}, D. and {Schmidt}, D. and
            {von der L{\"u}he}, O.},
    title = "{Adaptive Optics Development at the German Solar Telescopes}",
  journal = ao,
     year = 2010,
   volume = 49,
    pages = {G155-G166},
      doi = {10.1364/AO.49.00G155}
}

@INPROCEEDINGS{Berkefeld2006,
   author = {{Berkefeld}, T. and {Soltau}, D. and {von der L{\"u}he}, O.},
    title = "{Multi-Conjugate Solar Adaptive Optics with the VTT and GREGOR}",
booktitle = {Advances in Adaptive Optics II},
     year = 2006,
   series = posp,
   volume = 6272,
   editor = {{Ellerbroek}, B. L. and {Bonaccini Calia}, D.},
    pages = {627205}
}

@INPROCEEDINGS{Berkefeld2005,
   author = {{Berkefeld}, T. and {Soltau}, D. and {von der L{\"u}he}, O.},
    title = "{Results of the Multi-Conjugate Adaptive Optics System at the
            German Solar Telescope, Tenerife}",
booktitle = {Astronomical Adaptive Optics Systems and Applications II},
     year = 2005,
   series = posp,
   volume = 5903,
   editor = {{Tyson}, R. K. and {Lloyd-Hart}, M.},
    pages = {219-226}
}

@INPROCEEDINGS{Berkefeld2004,
   author = {{Berkefeld}, T. and {Soltau}, D. and {von der L{\"u}he}, O.},
    title = "{Second-Generation Adaptive Optics for the 1.5-Meter Solar
            Telescope GREGOR, Tenerife}",
booktitle = {Advancements in Adaptive Optics},
     year = 2004,
   series = posp,
   volume = 5490,
   editor = {{Bonaccini Calia}, D. and {Ellerbroek}, B. L. and {Ragazzoni}, R.},
    pages = {260-267}
}

@INPROCEEDINGS{Bettonvil2008,
   author = {{Bettonvil}, F. C. M. and {Hammerschlag}, R. H. and
            {J{\"a}gers}, A. P. L. and {Sliepen}, G.},
    title = "{Large Fully Retractable Telescope Enclosures Still Closable in
            Strong Wind}",
booktitle = {Advanced Optical and Mechanical Technologies in Telescopes and
            Instrumentation},
     year = 2008,
   series = posp,
   volume = 7018,
   editor = {{Atad-Ettedgui}, E. and {Lemke}, D.},
    pages = {70181N}
}

@ARTICLE{Bharti2007,
   author = {{Bharti}, L. and {Joshi}, C. and {Jaaffrey}, S. N. A.},
    title = "{Observations of Dark Lanes in Umbral Fine Structure from the
            Hinode Solar Optical Telescope: Evidence for Magnetoconvection}",
  journal = apjl,
     year = 2007,
   volume = 669,
    pages = {L57-L60}
}

@ARTICLE{Borrero2008,
   author = {{Borrero}, J. M. and {Lites}, B. W. and {Solanki}, S. K.},
    title = "{Evidence of Magnetic Field Wrapping around Penumbral Filaments}",
  journal = aa,
     year = 2008,
   volume = 481,
    pages = {L13-L16}
}

@ARTICLE{Borrero2007a,
   author = {{Borrero}, J. M. and {Bellot Rubio}, L. R. and 
            {M{\"u}ller}, D. A. N.},
    title = "{Flux Tubes as the Origin of Net Circular Polarization in Sunspot
            Penumbrae}",
  journal = apjl,
     year = 2007,
   volume = 666,
    pages = {L133-L136}
}

@ARTICLE{Borrero2007b,
   author = {{Borrero}, J. M.},
    title = "{The Structure of Sunspot Penumbrae. IV. MHS Equilibrium for
            Penumbral Flux Tubes and the Origin of Dark Core Penumbral
            Filaments and Penumbral Grains}",
  journal = aa,
     year = 2007,
   volume = 471,
    pages = {967-975}
}

@ARTICLE{Borrero2007c,
   author = {{Borrero}, J. M. and {Tomczyk}, S. and {Norton}, A. and
            {Darnell}, T. and {Schou}, J. and {Scherrer}, P. and {Bush}, R. and
            {Liu}, Y.},
    title = "{Magnetic Field Vector Retrieval With the Helioseismic and Magnetic
            Imager}",
  journal = sp,
     year = 2007,
   volume = 240,
    pages = {177-196}
}

@ARTICLE{Borrero2005,
   author = {{Borrero}, J. M. and {Lagg}, A. and {Solanki}, S. K. and
            {Collados}, M.},
    title = "{On the Fine Structure of Sunspot Penumbrae. II.\ The Nature of the
            Evershed Flow}",
  journal = aa,
     year = 2005,
   volume = 436,
    pages = {333-345}
}

@ARTICLE{Borrero2004,
   author = {{Borrero}, J. M. and {Solanki}, S. K. and 
            {Bellot Rubio}, L. R. and {Lagg}, A. and {Mathew}, S. K.},
    title = "{On the Fine Structure of Sunspot Penumbrae. I. A Quantitative
            Comparison of Two Semiempirical Models with Implications for the
            Evershed Effect}",
  journal = aa,
     year = 2004,
   volume = 422,
    pages = {1093-1104}
}

@ARTICLE{Bostanci2011,
   author = {{Bostanci}, Z. F.},
    title = "{Cloud Modeling of a Network Region in H$\alpha$}",
  journal = an,
     year = 2011,
   volume = 332,
    pages = {815-820}
}

@ARTICLE{Bostanci2010,
   author = {{Bostanci}, Z. F. and {Erdogan}, N. A.},
    title = "{Cloud Modeling of a Quiet Solar Region in H$\alpha$}",
  journal = msai,
     year = 2010,
   volume = 81,
    pages = {769-772}
}

@ARTICLE{Bovelet2003,
   author = {{Bovelet}, B. and {Wiehr}, E.},
    title = "{Dynamics of the Solar Active Region Finestructure}",
  journal = aa,
     year = 2003,
   volume = 412,
    pages = {249-255}
}

@ARTICLE{Bradley2006,
   author = {{Bradley}, E. S. and {Roberts}, Jr., L. C. and
            {Bradford}, L. W. and {Skinner}, M. A. and {Nahrstedt}, D. A. and
            {Waterson}, M. F. and {Kuhn}, J. R.},
    title = "{Characterization of Meteorological and Seeing Conditions at
            Haleakala}",
  journal = pasp,
     year = 2006,
   volume = 118,
    pages = {172-182},
      doi = {10.1086/497622}
}

@ARTICLE{Brandt1988,
   author = {{Brandt}, P. N. and {Scharmer}, G. B. and {Ferguson}, S. and
            {Shine}, R. A. and {Tarbell}, T. D.},
    title = "{Vortex Flow in the Solar Photosphere}",
  journal = nat,
     year = 1988,
   volume = 335,
    pages = {238-240}
}

@ARTICLE{Brandt1982,
   author = {{Brandt}, P. N. and {W{\"o}hl}, H.},
    title = "{Solar Site-Testing Campaign of JOSO on the Canary Islands in
            1979}",
  journal = aa,
     year = 1982,
   volume = 109,
    pages = {77-89}
}

@BOOK{Bray1964,
   author = {{Bray}, R. J. and {Loughhead}, R. E.},
    title = "{Sunspots}",
publisher = {Chapman \& Hall},
   series = "{The International Astrophysics Series}",
  address = "London",
     year = 1964
}

@ARTICLE{Brickhouse1988,
   author = {{Brickhouse}, N. S. and {Labonte}, B. J.},
    title = "{Mass and Energy Flow Near Sunspots. I.\ Observations of Moat
            Properties}",
  journal = sp,
     year = 1988,
   volume = 115,
    pages = {43-60},
      doi = {10.1007/BF00146229}
}

@ARTICLE{Brown1971,
   author = {{Brown}, J. C.},
    title = "{The Deduction of Energy Spectra of Non-Thermal Electrons in Flares
            from the Observed Dynamic Spectra of Hard X-Ray Bursts}",
  journal = sp,
     year = 1971,
   volume = 18,
    pages = {489-502}
}

@ARTICLE{Bruzek1969,
   author = {{Bruzek}, A.},
    title = "{Motions in Arch Filament Systems}",
  journal = sp,
     year = 1969,
   volume = 8,
    pages = {29-36},
      doi = {10.1007/BF00150655}
}

@ARTICLE{Bruzek1967,
   author = {{Bruzek}, A.},
    title = "{On Arch-Filament Systems in Spotgroups}",
  journal = sp,
     year = 1967,
   volume = 2,
    pages = {451-461},
      doi = {10.1007/BF00146493}
}

@ARTICLE{Bumba1963,
   author = {{Bumba}, V.},
    title = "{Development of SPOT Group Areas in Dependence on the Local
            Magnetic Field}",
  journal = baic,
     year = 1963,
   volume = 14,
    pages = {91-97}
}



%====     CCCC    ==============================================================

@ARTICLE{CabreraSolana2007,
   author = {{Cabrera Solana}, D. and {Bellot Rubio}, L.~R. and {Beck}, C. and 
	{Del Toro Iniesta}, J.~C.},
    title = "{Temporal evolution of the Evershed flow in sunspots. I. Observational characterization of 
Evershed clouds}",
  journal = aap,
archivePrefix = "arXiv",
   eprint = {0707.2629},
 keywords = {sunspots, magnetic fields, Sun: photosphere},
     year = 2007,
   volume = 475,
    pages = {1067-1079},
      doi = {10.1051/0004-6361:20077819},
}

@ARTICLE{CabreraSolana2006,
   author = {{Cabrera Solana}, D. and {Bellot Rubio}, L. R. and {Beck}, C. and
            {del Toro Iniesta}, J. C.},
    title = "{Evershed Clouds as Precursors of Moving Magnetic Features around
            Sunspots}",
  journal = apjl,
     year = 2006,
   volume = 649,
    pages = {L41-L44}
}

@ARTICLE{Cameron2007,
   author = {{Cameron}, R. and {Sch{\"u}ssler}, M. and {V{\"o}gler}, A. and 
            {Zakharov}, V.},
    title = "{Radiative Magnetohydrodynamic Simulations of Solar pores}",
  journal = aa,
     year = 2007,
   volume = 474,
    pages = {261-272}
}

@ARTICLE{Cao2006,
   author = {{Cao}, W. and {Jing}, J. and {Ma}, J. and {Xu}, Y. and
            {Wang}, H. and {Goode}, P. R.},
    title = "{Diffraction-Limited Polarimetry from the Infrared Imaging
            Magnetograph at Big Bear Solar Observatory}",
  journal = pasp,
     year = 2006,
   volume = 118,
    pages = {838-844}
}

@INPROCEEDINGS{Cao2005,
   author = {{Cao}, W. and {Xu}, Y. and {Denker}, C. and {Wang}, H.},
    title = "{$1024 \times 1024$ Hg\,Cd\,Te CMOS Camera for Infrared Imaging
            Magnetograph of Big Bear Solar Observatory}",
booktitle = {Infrared and Photoelectronic Imagers and Detector Devices},
     year = 2005,
   series = posp,
   volume = 5881,
   editor = {{Longshore}, R. E.},
    pages = {245-252}
}

@INPROCEEDINGS{Cao2004,
   author = {{Cao}, W. and {Denker}, C. and {Wang}, H. and {Ma}, J. and
            {Qu}, M. and {Wang}, J. and {Goode}, P. R.},
    title = "{Characteristic Evaluation of a Near-Infrared Fabry-P{\'e}rot
            Filter for the InfraRed Imaging Magnetograph (IRIM)}",
booktitle = {Telescopes and Instrumentation for Solar Astrophysics},
   series = posp,
     year = 2004,
   volume = 5171,
   editor = {{Fineschi}, S. and {Gummin}, M. A.},
    pages = {307-315}
}

@ARTICLE{Carlsson2004,
   author = {{Carlsson}, M. and {Stein}, R. F. and {Nordlund}, {\AA}. and 
            {Scharmer}, G. B.},
    title = "{Observational Manifestations of Solar Magnetoconvection:
            Center-to-Limb Variation}",
  journal = apjl,
     year = 2004,
   volume = 610,
    pages = {L137-L140},
      doi = {10.1086/423305}
}

@ARTICLE{Cavallini2006,
   author = {{Cavallini}, F.},
    title = "{IBIS: A New Post-Focus Instrument for Solar Imaging
            Spectroscopy}",
  journal = sp,
     year = 2006,
   volume = 236,
    pages = {415-439}
}

@ARTICLE{Cebula1998,
   author = {{Cebula}, R. P. and {Deland}, M. T.},
    title = "{Comparisons of the NOAA-11 SBUV/2, UARS SOLSTICE, and UARS SUSIM
            Mg\,\textsc{ii} Solar Activity Proxy Indexes}",
  journal = sp,
     year = 1998,
   volume = 177,
    pages = {117-132}
}

@ARTICLE{Chae2014,
   author = {{Chae}, J.},
    title = "{Spectral Inversion of the H{$\alpha$} Line for a Plasma Feature in 
            the Upper Chromosphere of the Quiet Sun}",
  journal = apj,
     year = 2014,
   volume = 780,
      eid = {109},
    pages = {109},
      doi = {10.1088/0004-637X/780/1/109}
}

@ARTICLE{Chae2010,
   author = {{Chae}, J. and {Goode}, P. R. and {Ahn}, K. and
            {Yurchysyn}, V. and {Abramenko}, V. and {Andic}, A. and
            {Cao}, W. and {Park}, Y. D.},
    title = "{New Solar Telescope Observations of Magnetic Reconnection
            Occurring in the Chromosphere of the Quiet Sun}",
  journal = apjl,
     year = 2010,
   volume = 713,
    pages = {L6-L10}
}

@ARTICLE{Chae2008,
   author = {{Chae}, J. and {Sakurai}, T.},
    title = "{A Test of Three Optical Flow Techniques-LCT, DAVE, and NAVE}",
  journal = apj,
     year = 2008,
   volume = 689,
    pages = {593-612}
}

@ARTICLE{Chae2007,
   author = {{Chae}, J. and {Park}, {H.-M.} and {Park}, {Y.-D.}},
    title = "{H{$\alpha$} Spectral Properties of Velocity Threads Constituting a
            Quiescent Solar Filament}",
  journal = jkas,
     year = 2007,
   volume = 40,
    pages = {67-82}
}

@ARTICLE{Chae2004,
   author = {{Chae}, J. and {Moon}, {Y.-J.} and {Park}, {Y.-D.}},
    title = "{Determination of Magnetic Helicity Content of Solar Active Regions
            from SOHO/MDI Magnetograms}",
  journal = sp,
     year = 2004,
   volume = 223,
    pages = {39-55}
}

@ARTICLE{Chae2000,
   author = {{Chae}, J. and {Denker}, C. and {Spirock}, T. J. and
            {Wang}, H. and {Goode}, P. R.},
    title = "{High-Resolution H$\alpha$ Observations of Proper Motion in NOAA
            8668. Evidence for Filament Mass Injection by Chromospheric
            Reconnection}",
  journal = sp,
     year = 2000,
   volume = 195,
    pages = {333-346}
}

@INPROCEEDINGS{Chae1999,
   author = {{Chae}, J.},
    title = "{Small-Scale Magnetic Reconnection in the Quiet Sun}",
booktitle = {High Resolution Solar Physics: Theory, Observations, and
            Techniques},
     year = 1999,
   series = asp,
   volume = 183,
   editor = {{Rimmele}, T. R. and {Balasubramaniam}, K. S. and {Radick}, R. R.},
    pages = {375-382}
}

@ARTICLE{Chae1998,
   author = {{Chae}, J. and {Wang}, H. and {Lee}, C.-Y. and {Goode}, P. R. and
            {Sch{\"u}hle}, U.},
    title = "{Chromospheric Upflow Events Associated with Transition Region
            Explosive Events}",
  journal = apjl,
     year = 1998,
   volume = 504,
    pages = {L123-L126}
}

@BOOK{Chandrasekhar1960,
   author = {{Chandrasekhar}, S.},
    title = "{Radiative Transfer}",
publisher = {Dover Publishers},
  address = {New York},
     year = 1960
}

@ARTICLE{Cheung2008,
   author = {{Cheung}, M. C. M. and {Sch{\"u}ssler}, M. and
            {Tarbell}, T. D. and {Title}, A. M.},
    title = "{Solar Surface Emerging Flux Regions: A Comparative Study of 
            Radiative MHD Modeling and Hinode SOT Observations}",
  journal = apj,
     year = 2008,
   volume = 687,
    pages = {1373-1387},
      doi = {10.1086/591245}
}

@ARTICLE{Chou1988,
   author = {{Chou}, D.-Y. and {Zirin}, H.},
    title = "{The Vertical Structure of Arch Filament Systems in Solar Emerging
            Flux Regions}",
  journal = apj,
     year = 1988,
   volume = 333,
    pages = {420-426},
      doi = {10.1086/166757}
}

@ARTICLE{Collados2012,
   author = {{Collados}, M. and {L{\'o}pez}, R. and {P{\'a}ez}, E. and
            {Hern{\'a}ndez}, E. and {Reyes}, M. and {Calcines}, A. and
            {Ballesteros}, E. and {D{\'{\i}}az}, J. J. and {Denker}, C. and
            {Lagg}, A. and {Schlichenmaier}, R. and {Schmidt}, W. and 
            {Solanki}, S.K. and {Strassmeier}, K. G. and 
            {von der L{\"u}he}, O. and {Volkmer}, R.},
    title = "{GRIS: The GREGOR Infrared Spectrograph}",
  journal = an,
     year = 2012,
   volume = 333,
    pages = {872-879},
      doi = {10.1002/asna.201211738}
}

@INPROCEEDINGS{Collados2010,
   author = {{Collados}, M. and {Bettonvil}, F. and {Cavaller}, L. and
            {Ermolli}, I. and {Gelly}, B. and {Grivel-Gelly}, C. and
            {P{\'e}rez}, A. and {Socas-Navarro}, H. and {Soltau}, D. and
            {Volkmer}, R.},
    title = "{European Solar Telescope: Project Status}",
booktitle = {Ground-Based and Airborne Telescopes IIII},
     year = 2010,
   series = posp,
   volume = 7733,
   editor = {{Stepp}, L. M. and Gilmozzi, R. and {Hall}, H. J.},
    pages = {77330H}
}

@INPROCEEDINGS{Collados2008a,
   author = {{Collados}, M.},
    title = "{European Solar Telescope (EST): Project Status}",
booktitle = {Ground-Based and Airborne Telescopes II},
     year = 2008,
   series = posp,
   volume = 7012,
   editor = {{Stepp}, L. M. and {Gilmozzi}, R.},
    pages = {70120J}
}

@INPROCEEDINGS{Collados2008b,
   author = {{Collados}, M. and {Calcines}, A. and {D{\'{\i}}az}, J. J. and
            {Hernn{\'a}dez}, E. and {L{\'o}pez}, R. and {P{\'a}ez}, E.},
    title = "{A High-Resolution Spectrograph for the Solar Telescope GREGOR}",
booktitle = {Ground-Based and Airborne Instrumentation for Astronomy II},
     year = 2008,
   series = posp,
   volume = 7014,
   editor = {{McLean}, I. S. and {Casali}, M. M.},
    pages = {70145Z}
}

@INPROCEEDINGS{Collados2007,
   author = {{Collados}, M. and {Lagg}, A. and
            {D{\'{\i}}az Garc{\'{\i}}a}, J. J. and
            {Hern{\'a}ndez Su{\'a}rez}, E. and {L{\'o}pez L{\'o}pez}, R. and
            {P{\'a}ez Ma{\~n}{\'a}}, E. and {Solanki}, S. K.},
    title = "{Tenerife Infrared Polarimeter II}",
booktitle = {The Physics of Chromospheric Plasmas},
     year = 2007,
   series = asp,
   volume = 368,
   editor = {{Heinzel}, P. and {Dorotovi{\v c}}, I. and \& {Rutten}, R. J.},
    pages = {611-616}
}

@ARTICLE{Contarino2009,
   author = {{Contarino}, L. and {Zuccarello}, F. and {Romano}, P. and
            {Spadaro}, D. and {Ermolli}, I.},
    title = "{Morphological and Dynamical Properties of Small-Scale
            Chromospheric Features Deduced from IBIS Observations}",
  journal = aa,
     year = 2009,
   volume = 507,
    pages = {1625-1633}
}

@ARTICLE{Cotton1995,
   author = {{Cotton}, W. D. and {Tody}, D. and {Pence}, W. D.},
    title = "{Binary Table Extension to FITS}",
  journal = aas,
     year = 1995,
   volume = 113,
    pages = {159-166}
}

@ARTICLE{Couvidat2011,
   author = {{Couvidat}, S. and {Schou}, J. and {Shine}, R. A. and {Bush}, R. I.
            and {Miles}, J. W. and {Scherrer}, P. H. and {Rairden}, R. L.},
    title = "{Wavelength Dependence of the Helioseismic and Magnetic Imager
            (HMI) Instrument onboard the Solar Dynamics Observatory (SDO)}",
  journal = sp,
     year = 2011,
    pages = {33-74}
}



%====     DDDD    ==============================================================

@INPROCEEDINGS{Dame2010,
   author = {{Dam{\'e}}, L. and {Andretta}, V. and
            {The ARENA Solar Astrophysics Working Group Members}},
    title = "{ARENA Solar Astrophysics Working Group Reporting on Dome C
            Exceptional Potential for Solar Observations}",
booktitle = {3$^{\rm rd}$ ARENA Conference: An Astronomical Observatory at
            CONCORDIA (Dome C, Antarctica)},
     year = 2010,
   series = easps,
   volume = 40,
   editor = {{Spinoglio}, L. and {Epchtein}, N.},
    pages = {451-466}
}

@ARTICLE{David1961,
   author = {{David}, K.-H.},
    title = "{Die Mitte-Rand Variation der Balmerlinien H{$\alpha$}--H{$\delta$} auf
            der Sonnenscheibe}",
  journal = zap,
     year = 1961,
   volume = 53,
    pages = {37-67},
}

@ARTICLE{deBoer1992,
   author = {{de Boer}, C. R. and {Kneer}, F.},
    title = "{Speckle Observations of Abnormal Solar Granulation}",
  journal = aa,
     year = 1992,
   volume = 264,
    pages = {L24-L26}
}

@ARTICLE{DeForest2007,
   author = {{DeForest}, C. E. and {Hagenaar}, H. J. and {Lamb}, D. A. and
            {Parnell}, C. E. and {Welsch}, B. T.},
    title = "{Solar Magnetic Tracking. I. Software Comparison and Recommended
            Practices}",
  journal = apj,
     year = 2007,
   volume = 666,
    pages = {576-587}
}

@ARTICLE{DeForest2004,
   author = {{DeForest}, C. E.},
    title = "{On Re-sampling of Solar Images}",
  journal = sp,
     year = 2004,
   volume = 219,
    pages = {3-23}
}

@ARTICLE{Degenhardt1991,
   author = {{Degenhardt}, D. and {Wiehr}, E.},
    title = "{Spatial Variation of the Magnetic Field Inclination in a Sunspot
            Penumbra}",
  journal = aa,
     year = 1991,
   volume = 252,
    pages = {821-826}
}

@ARTICLE{delaCruzRodriguez2015,
   author = {{de la Cruz Rodr{\'{\i}}guez}, J. and {L{\"o}fdahl}, M. G. and 
            {S{\"u}tterlin}, P. and {Hillberg}, T. and {Rouppe van der Voort}, L.},
    title = "{CRISPRED: A Data Pipeline for the CRISP Imaging Spectropolarimeter}",
  journal = aa,
     year = 2015,
   volume = 573,
      eid = {A40},
    pages = {A40},
      doi = {10.1051/0004-6361/201424319}
}

@BOOK{Delbouille1973,
   author = {{Delbouille}, L. and {Roland}, G. and {Neven}, L.},
    title = "{Atlas photometrique du spectre solaire de $\lambda$ 3000 a $\lambda$ 10000}",
booktitle = {Liege: Universite de Liege, Institut d'Astrophysique, 1973},
     year = 1973
}

@INPROCEEDINGS{Deng2011,
   author = {{Deng}, N. and {Shimizu}, T. and {Choudhary}, D. P. and
            {Wang}, H.},
    title = "{What Determines the Penumbral Size and Evershed Flow Speed?}",
booktitle = "{The Physics of Sun and Star Spots}",
     year = 2011,
   series = iaus,
   volume = 273,
   editor = {{Prasad Choudhary}, D. and {Strassmeier}, K. G.},
    pages = {216-220},
      doi = {10.1017/S1743921311015274}
}

@ARTICLE{Deng2007,
   author = {{Deng}, N. and {Choudhary}, D. P. and {Tritschler}, A. and
            {Denker}, C. and {Liu}, C. and {Wang}, H.},
    title = "{Flow Field Evolution of a Decaying Sunspot}",
  journal = apj,
     year = 2007,
   volume = 671,
    pages = {1013-1021}
}

@ARTICLE{Deng2006,
   author = {{Deng}, N. and {Xu}, Y. and {Yang}, G. and {Cao}, W. and
            {Liu}, C. and {Rimmele}, T. R. and {Wang}, H. and {Denker}, C.},
    title = "{Multiwavelength Study of Flow Fields in Flaring Super Active
            Region NOAA 10486}",
  journal = apj,
     year = 2006,
   volume = 644,
    pages = {1278-1291}
}

@ARTICLE{Deng2005,
   author = {{Deng}, N. and {Liu}, C. and {Yang}, G. and {Wang}, H. and
            {Denker}, C.},
    title = "{Rapid Penumbral Decay Associated with an X2.3 Flare in NOAA
            Active Region 9026}",
  journal = apj,
     year = 2005,
   volume = 623,
    pages = {1195-1201}
}

@ARTICLE{Deng2000,
   author = {{Deng}, Y. Y. and {Schmieder}, B. and {Engvold}, O. and
            {DeLuca}, E. and {Golub}, L.},
    title = "{Emergence of Sheared Magnetic Flux Tubes in an Active Region
            Observed with the SVST and TRACE}",
  journal = sp,
     year = 2000,
   volume = 195,
    pages = {347-366},
      doi = {10.1023/A:1005299227675}
}

@ARTICLE{Denker2012,
   author = {{Denker}, C. and {von der L{\"u}he}, O. and {Feller}, A. and 
            {Arlt}, K. and {Balthasar}, H. and {Bauer}, S.-M. and
            {Bello Gonz{\'a}lez}, N. and {Berkefeld}, T. and {Caligari}, P. and
            {Collados}, M. and {Fischer}, A. and {Granzer}, T. and
            {Hahn}, T. and {Halbgewachs}, C. and {Heidecke}, F. and 
            {Hofmann}, A. and {Kentischer}, T. and {Klva{\v n}a}, M. and 
            {Kneer}, F. and {Lagg}, A. and {Nicklas}, H. and {Popow}, E. and 
            {Puschmann}, K. G. and {Rendtel}, J. and {Schmidt}, D. and
            {Schmidt}, W. and {Sobotka}, M. and {Solanki}, S. K. and
            {Soltau}, D. and {Staude}, J. and {Strassmeier}, K. G. and
            {Volkmer}, R. and {Waldmann}, T. and {Wiehr}, E. and
            {Wittmann}, A. D. and {Woche}, M.},
    title = "{A Retrospective of the GREGOR Solar Telescope in Scientific
            Literature}",
  journal = an,
     year = 2012,
   volume = 333,
    pages = {810},
      doi = {10.1002/asna.201211728}
}

@INPROCEEDINGS{Denker2011,
   author = {{Denker}, C. and {Verma}, M.},
    title = "{Velocity Fields in and around Sunspots at the Highest
            Resolution}",
booktitle = {The Physics of Sun and Star Spots},
   series = iaus,
     year = 2011,
   volume = 273,
   editor = {{Choudhary}, D. P. and {Strassmeier}, K. G.},
    pages = {204-211},
      doi = {10.1017/S1743921311015250}
}

@INPROCEEDINGS{Denker2010a,
   author = {{Denker}, C. and {Balthasar}, H. and {Hofmann}, A. and
            {Bello Gonz{\'a}lez}, N. and {Volkmer}, R.},
    title = "{The GREGOR Fabry-P{\'e}rot Interferometer: A New Instrument for
            High-Resolution Solar Observations}",
booktitle = {Ground-Based and Airborne Instrumentation for Astronomy III},
   series = posp,
     year = 2010,
   volume = {7735},
   editor = {{McLean}, I. S. and {Ramsay}, S. K. and {Takami}, H.},
    pages = {77356M}
}

@ARTICLE{Denker2010b,
   author = {{Denker}, C.},
    title = "{Instrument and Data Analysis Challenges for Imaging
            Spectropolarimetry}",
  journal = an,
     year = 2010,
   volume = 331,
    pages = {648-651}
}

@INPROCEEDINGS{Denker2009,
   author = {{Denker}, C. and {Tritschler}, A.},
    title = "{Mini-Filaments --- Small-Scale Analogues of Solar Eruptive
            Events?}",
 booktitle = {Cosmic Magnetic Fields: From Planets, to Stars and Galaxies},
     year = 2009,
   series = iaus,
   volume = 259,
   editor = {{Strassmeier}, K. G. and {Kosovichev}, A. G. and
            {Beckmann}, J. E.},
    pages = {223-224}
}

@INPROCEEDINGS{Denker2008a,
   author = {{Denker}, C. and {Strassmeier}, K. G.},
    title = "{Solar Physics and the Solar-Stellar Connection at Dome C}",
booktitle = {2$^{\rm nd}$ ARENA Conference: The Astrophysical Science Cases
            at Dome C},
     year = 2008,
   series = easps,
   volume = 33,
   editor = {{Zinnecker}, H. and {Epchtein}, N. and {Rauer}, H.},
    pages = {97-104}
}

@ARTICLE{Denker2008b,
   author = {{Denker}, C. and {Tritschler}, A. and {Deng}, N.},
    title = "{High-Resolution Observations of Extremely Bright  Penumbral
            Grains}",
  journal = an,
     year = 2008,
   volume = 329,
    pages = {773-779}
}

@ARTICLE{Denker2007a,
   author = {{Denker}, C. and {Deng}, N. and {Rimmele}, T. R. and
            {Tritschler}, A. and {Verdoni}, A.},
    title = "{Field-Dependent Adaptive Optics Correction Derived with the
            Spectral Ratio Technique}",
  journal = sp,
     year = 2007,
   volume = 241,
    pages = {411-426}
}

@ARTICLE{Denker2007b,
   author = {{Denker}, C. and {Tritschler}, A. and {Rimmele}, T. R. and
            {Richards}, K. and {Hegwer}, S. L. and {W{\"o}ger}, F.},
    title = "{Adaptive Optics at the Big Bear Solar Observatory: Instrument
            Description and First Observations}",
  journal = pasp,
     year = 2007,
   volume = 119,
    pages = {170-182}
}

@ARTICLE{Denker2007c,
   author = {{Denker}, C. and {Deng}, N. and {Tritschler}, A. and
            {Yurchyshyn}, V.},
    title = "{Two-Dimensional Spectroscopy of Photospheric Shear Flows in a
            Small {$\delta$} Spot}",
  journal = sp,
     year = 2007,
   volume = 245,
    pages = {219-238}
}

@INPROCEEDINGS{Denker2006a,
   author = {{Denker}, C. and {Verdoni}, A. P.},
    title = "{Integrating Seeing Measurements into the Operations of Solar
            Telescopes}",
booktitle = {Ground-Based and Airborne Telescopes},
   series = posp,
     year = 2006,
   volume = 6267,
    pages = {62670L},
   editor = {{Stepp}, L. M.}
}

@INPROCEEDINGS{Denker2006b,
   author = {{Denker}, C. and {Goode}, P. R. and {Ren}, D. and
            {Saadeghvaziri}, M. A. and {Verdoni}, A. P. and {Wang}, H. and
            {Yang}, G. and {Abramenko}, V. and {Cao}, W. and {Coulter}, R. and
            {Fear}, R. and {Nenow}, J. and {Shoumko}, S. and
            {Spirock}, T. J. and {Varsik}, J. R. and {Chae}, J. and
            {Kuhn}, J. R. and {Moon}, Y. and {Park}, Y. D. and
            {Tritschler}, A.},
    title = "{Progress on the 1.6-Meter New Solar Telescope at Big Bear Solar
            Observatory}",
booktitle = {Ground-Based and Airborne Telescopes},
   series = posp,
     year = 2006,
   volume = 6267,
    pages = {62670A},
   editor = {{Stepp}, L. M.}
}

@ARTICLE{Denker2005a,
   author = {{Denker}, C. and {Tritschler}, A.},
    title = "{Measuring and Maintaining the Plate Parallelism of Fabry-P{\'e}rot
            Etalons}",
  journal = pasp,
     year = 2005,
   volume = 117,
    pages = {1435-1444}
}

@ARTICLE{Denker2005b,
   author = {{Denker}, C. and {Mascarinas}, D. and {Xu}, Y. and {Cao}, W. and
            {Yang}, G. and {Wang}, H. and {Goode}, P. R. and {Rimmele}, T. R.},
    title = "{High-Spatial Resolution Imaging Combining High-Order Adaptive
            Optics, Frame Selection, and Speckle Masking Reconstruction}",
  journal = sp,
     year = 2005,
   volume = 227,
    pages = {217-230}
}

@INPROCEEDINGS{Denker2005c,
   author = {{Denker}, C.},
    title = "{Observations of Photosphere and Chromosphere}",
booktitle = {Astrophysics and Space Science Library},
publisher = {Springer},
  address = {Dordrecht, The Netherlands},
     year = 2005,
   series = {Astrophysics and Space Science Library},
   volume = 320,
   editor = {{Hanslmeier}, A. and {Veronig}, A. and {Messerotti}, M.},
    pages = {1-25}
}

@ARTICLE{Denker2003a,
   author = {{Denker}, C. and {Didkovsky}, L. and {Ma}, J. and {Shumko}, S. and
            {Varsik}, J. and {Wang}, J. and {Wang}, H. and {Goode}, P. R.},
    title = "{Imaging Magnetographs for High-Resolution Solar Observations in
            the Visible and Near-Infrared Wavelength Region}",
  journal = an,
     year = 2003,
   volume = 324,
    pages = {332-333}
}

@INPROCEEDINGS{Denker2003b,
   author = {{Denker}, C. and {Ma}, J. and {Wang}, J. and {Didkovsky}, L. V. and
            {Varsik}, J. R. and {Wang}, H. and {Goode}, P. R.},
    title = "{IRIM: An Imaging Magnetograph for High-Resolution Solar
            Observations in the Near-Infrared}",
booktitle = {Innovative Telescopes and Instrumentation for Solar Astrophysics},
   series = posp,
     year = 2003,
   volume = 4853,
   editor = {{Keil}, S. L. and {Avakyan}, S. V.},
    pages = {223-234}
}

@INPROCEEDINGS{Denker2003c,
   author = {{Denker}, C. and {Didkovsky}, L. and {Marquette}, W. H. and
            {Goode}, P. R. and {Venkateswaran}, K. and {Rimmele}, T. R.},
    title = "{Seeing Characteristic at a Lake-Site Observatory}",
booktitle = {Current Theoretical Models and Future High Resolution Solar
            Observations: Preparing for ATST},
     year = 2003,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 286,
   editor = {{Pevtsov}, A. A. and {Uitenbroek}, H.},
    pages = {23-30}
}

@ARTICLE{Denker2001a,
   author = {{Denker}, C. and {Yang}, G. and {Wang}, H.},
    title = "{Near Real-Time Image Reconstruction}",
  journal = sp,
     year = 2001,
   volume = 202,
    pages = {63-70}
}

@INPROCEEDINGS{Denker2001b,
   author = {{Denker}, C. and {Spirock}, T. and {Varsik}, J. R. and
            {Chae}, J. and {Marquette}, W. H. and {Wang}, H. and
            {Goode}, P. R.},
    title = "{Dynamics of Quiet Sun Magnetic Fields}",
booktitle = {Advanced Solar Polarimetry -- Theory, Observation, and
            Instrumentation},
     year = 2001,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 236,
   editor = {{Sigwarth}, M.},
    pages = {463-470}
}

@INPROCEEDINGS{Denker2001c,
   author = {{Denker}, C. and {Spirock}, T. J. and {Jefferies}, S. M. and
            {Chen}, H. and {Marquette}, W. H. and {Wang}, H. and
            {Goode}, P. R.},
    title = "{Multi-Wavelength Observations of Solar Fine-Structure with High
            Spatial Resolution}",
booktitle = {11th Cambridge Workshop on Cool Stars, Stellar Systems and the
            Sun},
     year = 2001,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 223,
   editor = {{Garcia Lopez}, R. J. and {Rebolo}, R. and 
            {Zapaterio Osorio}, M. R.},
    pages = {607-612}
}

@ARTICLE{Denker1999a,
   author = {{Denker}, C. and {Johannesson}, A. and {Marquette}, W. and
            {Goode}, P. R. and {Wang}, H. and {Zirin}, H.},
    title = "{Synoptic H{$\alpha$} Full-Disk Observations of the Sun from Big
            Bear Solar Observatory. I. Instrumentation, Image Processing,
            Data Products, and First Results}",
  journal = sp,
     year = 1999,
   volume = 184,
    pages = {87-102}
}

@INPROCEEDINGS{Denker1999b,
   author = {{Denker}, C. and {Spirock}, T. and {Goode}, P. and {Wang}, H.},
    title = "{Properties of Sunspots and Pores}",
booktitle = {High Resolution Solar Physics: Theory, Observations, and
            Techniques},
     year = 1999,
   series = asp,
   volume = 183,
   editor = {{Rimmele}, T. R. and {Balasubramaniam}, K. S. and
            {Radick}, R. R.},
    pages = {124-131}
}

@ARTICLE{Denker1998a,
   author = {{Denker}, C. and {Wang}, H.},
    title = "{High Spatial Resolution Observations of a Small $\delta$-Spot}",
  journal = apj,
     year = 1998,
   volume = 502,
    pages = {493-497}
}

@ARTICLE{Denker1998b,
   author = {{Denker}, C.},
    title = "{Speckle Masking Imaging of Sunspots and Pores}",
  journal = sp,
     year = 1998,
   volume = 180,
    pages = {81-108}
}

@ARTICLE{Denker1997,
   author = {{Denker}, C.},
    title = "{Two-Dimensional Speckle Spectroscopy of the Moustache Phenomenon
            on the Sun}",
  journal = aa,
     year = 1997,
   volume = 323,
    pages = {599-605}
}

@PHDTHESIS{Denker1996,
   author = {{Denker}, C.},
    title = "{Untersuchung der Feinstruktur von Sonnenflecken mit Methoden der
            Speckle-Interferometrie}",
   school = {Georg-August Universit{\"a}t G{\"o}ttingen, Germany},
     year = 1996,
publisher = {Aktiv Druck Verlag},
  address = {G{\"o}ttingen, Germany}
}

@ARTICLE{Denker1995a,
   author = {{Denker}, C. and {de Boer}, C. R. and {Volkmer}, R. and
            {Kneer}, F.},
    title = "{Speckle Masking Imaging of the Moustache Phenomenon}",
  journal = aa,
     year = 1995,
   volume = 296,
    pages = {567-573}
}

@INPROCEEDINGS{Denker1995b,
   author = {{Denker}, C. and {de Boer}, C. R. and {Kneer}, F.},
    title = "{Speckle-Masking Imaging of Bright Points (Moustaches)}",
booktitle = {IAU Symposium},
     year = 1995,
   series = {IAU Symposium},
   volume = 176,
    pages = {51-53}
}

@INPROCEEDINGS{Denker1994,
   author = {{Denker}, C.},
    title = "{Speckle Observations of Sunspots}",
booktitle = {Solar Magnetic Fields},
     year = 1994,
   editor = {{Sch{\"u}ssler}, M. and {Schmidt}, W.},
    pages = {194-199}
}

@ARTICLE{deToma2004,
   author = {{de Toma}, G. and {White}, O. R. and {Chapman}, G. A. and
            {Walton}, S. R. and {Preminger}, D. G. and {Cookson}, A. M.},
    title = "{Solar Cycle 23. An Anomalous Cycle?}",
  journal = apj,
     year = 2004,
   volume = 609,
    pages = {1140-1152}
}

@INPROCEEDINGS{Didkovsky2003a,
   author = {{Didkovsky}, L. V. and {Dolgushyn}, A. and {Marquette}, W. and
            {Nenow}, J. and {Varsik}, J. and {Goode}, P. R. and
            {Hegwer}, S. L. and {Ren}, D. and {Fletcher}, S. and
            {Richards}, K. and {Rimmele}, T. and {Denker}, C. and {Wang}, H.},
    title = "{High-Order Adaptive Optical System for Big Bear Solar
            Observatory}",
booktitle = {Innovative Telescopes and Instrumentation for Solar Astrophysics},
   series = posp,
     year = 2003,
   volume = 4853,
   editor = {{Keil}, S. L. and {Avakyan}, S. V.},
    pages = {630-639}
}

@ARTICLE{Didkovsky2003b,
   author = {{Didkovsky}, L. V. and {Denker}, C. and {Goode}, P. R. and
            {Wang}, H. and {Rimmele}, T. R.},
    title = "{High-Order Adaptive Optical System for Big Bear Solar
            Observatory}",
  journal = an,
     year = 2003,
   volume = 324,
    pages = {297-298}
}

@ARTICLE{Dunn1973,
   author = {{Dunn}, R. B. and {Zirker}, J. B.},
    title = "{The Solar Filigree}",
  journal = sp,
     year = 1973,
   volume = 33,
    pages = {281-304}
}

@ARTICLE{Durrant1975,
   author = {{Durrant}, C. J.},
    title = "{Spectroscopic Investigation of the Chromosphere. IV.\ A
            Reassessment of the Cloud Model}",
  journal = sp,
     year = 1975,
   volume = 44,
    pages = {41-53}
}



%====     EEEE    ==============================================================

@INPROCEEDINGS{Emde2004,
   author = {{Emde}, P. and {K{\"u}hn}, J. and {Weis}, U. and {Bornkessel}, T.},
    title = "{Thermal Design Features of the Solar Telescope GREGOR}",
booktitle = {Astronomical Structures and Mechanisms Technology},
     year = 2004,
   series = posp,
   volume = 5495,
   editor = {{Antebi}, J. and {Lemke}, D.},
    pages = {238-246}
}

@INPROCEEDINGS{Emde2003,
   author = {{Emde}, P. and {Suss}, M. and {Eisentr{\"a}ger}, P. and
            {Moik}, R. and {Karcher}, H.},
    title = "{Design of the Solar Telescope GREGOR under Dynamic Wind Loads}",
booktitle = {Optical Materials and Structures Technologies},
     year = 2003,
   series = posp,
   volume = 5179,
   editor = {{Goodman}, W. A.},
    pages = {282-291}
}

@ARTICLE{Emslie2005,
   author = {{Emslie}, A. G. and {Dennis}, B. R. and {Holman}, G. D. and
            {Hudson}, H. S.},
    title = "{Refinements to Flare Energy Estimates: A Followup to ``Energy
            Partition in Two Solar Flare/CME Events''}",
     year = 2005,
   volume = 110,
   number = A9,
    pages = {11103}
}

@ARTICLE{Ermolli2009a,
   author = {{Ermolli}, I. and {Marchei}, E. and {Centrone}, M. and
            {Criscuoli}, S. and {Giorgi}, F. and {Perna}, C.},
    title = "{The Digitized Archive of the Arcetri Spectroheliograms.
            Preliminary Results from the Analysis of Ca\,\textsc{ii}\,K
            Images}",
  journal = aa,
     year = 2009,
   volume = 499,
    pages = {627-632}
}

@ARTICLE{Ermolli2009b,
   author = {{Ermolli}, I. and {Solanki}, S. K. and {Tlatov}, A. G. and
            {Krivova}, N. A. and {Ulrich}, R. K. and {Singh}, J.},
    title = "{Comparison Among Ca\,\textsc{ii}\,K Spectroheliogram Time Series
            with an Application to Solar Activity Studies}",
  journal = apj,
     year = 2009,
   volume = 698,
    pages = {1000-1009}
}

@ARTICLE{Ermolli2007,
   author = {{Ermolli}, I. and {Criscuoli}, S. and {Centrone}, M. and {Giorgi},
            F. and {Penza}, V.},
    title = "{Photometric Properties of Facular Features over the Activity
            Cycle}",
  journal = aa,
     year = 2007,
   volume = 465,
    pages = {305-314}
}

@ARTICLE{Ermolli2003,
   author = {{Ermolli}, I. and {Berrilli}, F. and {Florio}, A.},
    title = "{A Measure of the Network Radiative Properties over the Solar
            Activity Cycle}",
  journal = aa,
     year = 2003,
   volume = 412,
    pages = {857-864}
}

@ARTICLE{Ermolli1998,
   author = {{Ermolli}, I. and {Fofi}, M. and {Bernacchia}, C. and
            {Berrilli}, F. and {Caccin}, B. and {Egidi}, A. and {Florio}, A.},
    title = "{The Prototype RISE-PSPT Instrument Operating in Rome}",
  journal = sp,
     year = 1998,
   volume = 177,
    pages = {1-10}
}

@book{Everitt2011,
author = "{Everitt}, B. and {Landau}, S. and {Leese}, M. and {Stahl}, D.",
title = "{Cluster analysis}",
publisher = "Wiley",
year = 2011,
}

@ARTICLE{Evershed1909,
   author = {{Evershed}, J.},
    title = "{Radial Movement in Sun-Spots}",
  journal = mn,
     year = 1909,
   volume = 69,
    pages = {454-457}
}

%====     FFFF    ==============================================================

@BOOK{Fanning2011,
   author = {{Fanning}, D. W.},
    title = "{Coyote's Guide to Traditional IDL Graphics}",
publisher = "Coyote Book Publishing",
  address = "Fort Collins, Colorado",
     year = 2011
}

@BOOK{Fanning2003,
   author = {{Fanning}, D. W.},
    title = "{IDL Programming Techniques}",
  edition = {2nd edn.},
publisher = "Fanning Software Consulting",
  address = "Fort Collins, Colorado",
     year = 2003
}

@ARTICLE{Floyd2005,
   author = {{Floyd}, L. and {Newmark}, J. and {Cook}, J. and {Herring}, L. and
            {McMullin}, D.},
    title = "{Solar EUV and UV Spectral Irradiances and Solar Indices}",
  journal = jatp,
     year = 2005,
   volume = 67,
    pages = {3-15}
}

@ARTICLE{Foukal2009,
   author = {{Foukal}, P. and {Bertello}, L. and {Livingston}, W. C. and
            {Pevtsov}, A. A. and {Singh}, J. and {Tlatov}, A. G. and
            {Ulrich}, R. K.},
    title = "{A Century of Solar Ca\,\textit{ii} Measurements and Their
            Implication for Solar UV Driving of Climate}",
  journal = sp,
     year = 2009,
   volume = 255,
    pages = {229-238}
}

@ARTICLE{Franz2009,
   author = {{Franz}, M. and {Schlichenmaier}, R.},
    title = "{The Velocity Field of Sunspot Penumbrae. I.\ A Global View}",
  journal = aa,
     year = 2009,
   volume = 508,
    pages = {1453-1460}
}

@ARTICLE{Freeland1998,
   author = {{Freeland}, S. L. and {Handy}, B. N.},
    title = "{Data Analysis with the SolarSoft System}",
  journal = sp,
     year = 1998,
   volume = 182,
    pages = {497-500}
}

@ARTICLE{Fried1974,
   author = {{Fried}, D. L. and {Mevers}, G. E.},
    title = "{Evaluation of $r_{0}$ for Propagation Down Through the
            Atmosphere}",
  journal = ao,
     year = 1974,
   volume = 13,
    pages = {2620-2622}
}

@ARTICLE{Froehlich2009,
   author = {{Fr{\"o}hlich}, C.},
    title = "{Evidence of a Long-Term Trend in Total Solar Irradiance}",
  journal = aa,
     year = 2009,
   volume = 501,
    pages = {L27-L30}
}



%====     GGGG    ==============================================================

@ARTICLE{Gafeira2014,
   author = {{Gafeira}, R. and {Fonte}, C. C. and {Pais}, M. A. and
            {Fernandes}, J.},
    title = "{Temporal Evolution of Sunspot Areas and Estimation of Related
            Plasma Flows}",
  journal = sp,
     year = 2014,
      doi = {10.1007/s11207-013-0440-3},
   volume = 289,
    pages = {1531-1542}
}

@ARTICLE{Gallagher2002,
   author = {{Gallagher}, P. T. and {Denker}, C. and {Yurchyshyn}, V. and
            {Spirock}, T. and {Qiu}, J. and {Wang}, H. and {Goode}, P. R.},
    title = "{Solar Activity Monitoring and Forecasting Capabilities at Big
            Bear Solar Observatory}",
  journal = ag,
     year = 2002,
   volume = 20,
    pages = {1105-1115}
}

@ARTICLE{Georgakilas2003,
   author = {{Georgakilas}, A. A. and {Christopoulou}, E. B.},
    title = "{Temporal Behavior of the Evershed Effect}",
  journal = apj,
     year = 2003,
   volume = 584,
    pages = {509-523}
}

@ARTICLE{Georgakilas2002,
   author = {{Georgakilas}, A. A. and {Muglach}, K. and {Christopoulou}, E. B.},
    title = "{Ultraviolet Observations of Periodic Annular Intensity
            Fluctuations Propagating Around Sunspots}",
  journal = apj,
     year = 2002,
   volume = 576,
    pages = {561-566}
}

@INPROCEEDINGS{Giorgini1996,
   author = {{Giorgini}, J. D. and {Yeomans}, D. K. and {Chamberlin}, A. B. and
            {Chodas}, P. W. and {Jacobson}, R. A. and {Keesey}, M. S. and
            {Lieske}, J. H. and {Ostro}, S. J. and {Standish}, E. M. and
            {Wimberly}, R. N.},
    title = "{JPL's On-Line Solar System Data Service}",
booktitle = baas,
     year = 1996,
   series = baas,
   volume = 28,
    pages = {1158}
}

@BOOK{Gonzalez2002,
   author = {{Gonzalez}, R. C. and {Woods}, R. E.},
    title = "{Digital Image Processing}",
publisher = "Prentice-Hall",
  address = "Upper Saddle River, New Jersey",
     year = 2002
}

@ARTICLE{Goode2010,
   author = {{Goode}, P. R. and {Yurchyshyn}, V. and {Cao}, W. and
            {Abramenko}, V. and {Andic}, A. and {Ahn}, K. and {Chae}, J.},
    title = "{Highest Resolution Observations of the Quietest Sun}",
  journal = apjl,
     year = 2010,
   volume = 714,
    pages = {L31-L35}
}

@ARTICLE{Goode2003a,
   author = {{Goode}, P. R. and {Denker}, C. and {Didkovsky}, L. I. and
            {Kuhn}, J. R. and {Wang}, H.},
    title = "{1.6-Meter Solar Telescope in Big Bear -- The NST}",
  journal = jkas,
     year = 2003,
   volume = 36,
    pages = {125-133}
}

@INPROCEEDINGS{Goode2003b,
   author = {{Goode}, P. R. and {Denker}, C. and {Wang}, H.},
    title = "{The Sun from Big Bear}",
booktitle = {Astrophysics and Space Science Library},
     year = 2003,
   series = {Astrophysics and Space Science Library},
   volume = 288,
   editor = {{Oswalt}, T. D.},
    pages = {137-155}
}

@ARTICLE{Goode2000,
   author = {{Goode}, P. R. and {Wang}, H. and {Marquette}, W. H. and
            {Denker}, C.},
    title = "{Measuring Seeing from Solar Scintillometry and the Spectral Ratio
            Technique}",
  journal = sp,
     year = 2000,
   volume = 195,
    pages = {421-431}
}

@ARTICLE{Gosain2009,
   author = {{Gosain}, S. and {Venkatakrishnan}, P. and {Tiwari}, S. K.},
    title = "{HINODE Observations of Coherent Lateral Motion of Penumbral
            Filaments During an X-Class Flare}",
  journal = apjl,
     year = 2009,
   volume = 706,
    pages = {L240-L245}
}

@INPROCEEDINGS{Graham2003,
   author = {{Graham}, J. D. and {Norton}, A. and {L{\'o}pez Ariste}, A. and 
            {Lites}, B. and {Socas-Navarro}, H. and {Tomczyk}, S.},
    title = "{The Helioseismic and Magnetic Imager (HMI) on SDO: Full Vector
            Magnetography with a Filtergraph Polarimeter}",
booktitle = {Solar Polarization},
     year = 2003,
   series = asp,
   volume = 307,
   editor = "{{Trujillo-Bueno}, J. and {Sanchez Almeida}, J.}",
    pages = {131-136},
}

@ARTICLE{Grossmann-Doerth1973,
   author = {{Grossmann-Doerth}, U. and {von Uexk{\"u}ll}, M.},
    title = "{Spectral Investigation of the Chromosphere. II.\ The Nature of the
            Mottles and a Model of the Overall Structure}",
  journal = sp,
     year = 1973,
   volume = 28,
    pages = {319-332}
}

@ARTICLE{Guglielmino2012,
   author = {{Guglielmino}, S. L. and {Mart{\'{\i}}nez Pillet}, V. and
            {Bonet}, J. A. and {del Toro Iniesta}, J. C. and
            {Bellot Rubio}, L. R. and {Solanki}, S. K. and  {Schmidt}, W. and
            {Gandorfer}, A. and {Barthol}, P. and {Kn{\"o}lker}, M.},
    title = "{The Frontier between Small-Scale Bipoles and Ephemeral Regions in
            the Solar Photosphere: Emergence and Decay of an Intermediate-Scale
            Bipole Observed with SUNRISE/IMaX}",
  journal = apj,
     year = 2012,
   volume = 745,
      eid = {160},
    pages = {160},
      doi = {10.1088/0004-637X/745/2/160}
}



%====     HHHH    ==============================================================

@ARTICLE{Hagenaar2005,
   author = {{Hagenaar}, H. J. and {Shine}, R. A.},
    title = "{Moving Magnetic Features around Sunspots}",
  journal = apj,
     year = 2005,
   volume = 635,
    pages = {659-669}
}

@ARTICLE{Hagenaar2001,
   author = {{Hagenaar}, H. J.},
    title = "{Ephemeral Regions on a Sequence of Full-Disk Michelson Doppler
            Imager Magnetograms}",
  journal = apj,
     year = 2001,
   volume = 555,
    pages = {448-461}
}

@ARTICLE{Hale1905,
   author = {{Hale}, G. E.},
    title = "{A Study of the Conditions for Solar Research at Mount Wilson,
            California}",
  journal = apj,
     year = 1905,
   volume = 21,
    pages = {124-155}
}

@INPROCEEDINGS{Hammerschlag2010,
   author = {{Hammerschlag}, R. H. and {Kommers}, J. N. M. and
            {van Leverink}, S. J. and {Bettonvil}, F. C. M. and {Visser}, S. and
            {J{\"a}gers}, A. P. L. and {Sliepen}, G.},
    title = "{Mechanical Design of a Completely Open-Foldable Dome for EST}",
booktitle = {Ground-Based and Airborne Telescopes III},
     year = 2010,
   series = posp,
   volume = 7733,
   editor = {{Stepp}, L. M. and {Gilmozzi}, R. and {Hall}, H. J.},
    pages = {77330J},
      doi = {10.1117/12.857807}
}

@ARTICLE{Handy1999,
   author = {{Handy}, B. N. and {Acton}, L. W. and {Kankelborg}, C. C. and
            {Wolfson}, C. J. and {Akin}, D. J. and {Bruner}, M. E. and
            {Caravalho}, R. and {Catura}, R. C. and {Chevalier}, R. and
            {Duncan}, D. W. and {Edwards}, C. G. and {Feinstein}, C. N. and
            {Freeland}, S. L. and {Friedlaender}, F. M. and 
            {Hoffmann}, C. H. and {Hurlburt}, N. E. and {Jurcevich}, B. K. and
            {Katz}, N. L. and {Kelly}, G. A. and {Lemen}, J. R. and
            {Levay}, M. and {Lindgren}, R. W. and {Mathur}, D. P. and
            {Meyer}, S. B. and {Morrison}, S. J. and {Morrison}, M. D. and
            {Nightingale}, R. W. and {Pope}, T. P. and {Rehse}, R. A. and
            {Schrijver}, C. J. and {Shine}, R. A. and {Shing}, L. and
            {Strong}, K. T. and {Tarbell}, T. D. and {Title}, A. M. and
            {Torgerson}, D. D. and {Golub}, L. and {Bookbinder}, J. A. and
            {Caldwell}, D. and {Cheimets}, P. N. and {Davis}, W. N. and
            {Deluca}, E. E. and {McMullen}, R. A. and {Warren}, H. P. and
            {Amato}, D. and {Fisher}, R. and {Maldonado}, H. and
            {Parkinson} C.},
    title = "{The Transition Region and Coronal Explorer}",
  journal = sp,
     year = 1999,
   volume = 187,
    pages = {229-260}
}

@ARTICLE{Hanisch2001,
   author = {{Hanisch}, R. J. and {Farris}, A. and {Greisen}, E. W. and
            {Pence}, W. D. and {Schlesinger}, B. M. and {Teuben}, P. J. and
            {Thompson}, R. W. and {Warnock}, A.},
    title = "{Definition of the Flexible Image Transport System (FITS)}",
  journal = aa,
     year = 2001,
   volume = 376,
    pages = {359-380}
}

@ARTICLE{Hanson2000,
   author = {{Hanson}, P. J. and {Weltzin}, J. F.},
    title = "{Drought Disturbance from Climate Change. Response of United
            States Forests}",
  journal = ste,
     year = 2000,
   volume = 262,
    pages = {205-220}
}

@ARTICLE{Hartlep2012,
   author = {{Hartlep}, T. and {Busse}, F. H. and {Hurlburt}, N. E. and
            {Kosovichev}, A. G.},
    title = "{Magnetohydrodynamic Simulations of Flows Around Rotating and
            Non-Rotating Axisymmetric Magnetic Flux Concentrations}",
  journal = mn,
     year = 2012,
   volume = 419,
    pages = {2325-2328}
}

@ARTICLE{Hartlep2010,
   author = {{Hartlep}, T. and {Kosovichev}, A. G. and {Zhao}, J. and
            {Mansour}, N. N.},
    title = "{Signatures of Emerging Subsurface Structures in Acoustic Power
            Maps}",
  journal = sp,
     year = 2010,
     note = {in press}
}

@ARTICLE{Harvey1976,
   author = {{Harvey}, K. L. and {Harvey}, J. W.},
    title = "{A Study of the Magnetic and Velocity Fields in an Active Region}",
  journal = sp,
     year = 1976,
   volume = 47,
    pages = {233-246}
}

@ARTICLE{Harvey1973,
   author = {{Harvey}, K. L. and {Martin}, S. F.},
    title = "{Ephemeral Active Regions}",
  journal = sp,
     year = 1973,
   volume = 32,
    pages = {389-402},
      doi = {10.1007/BF00154951}
}

@ARTICLE{Heggland2009,
   author = {{Heggland}, L. and {De Pontieu}, B. and {Hansteen}, V. H.},
    title = "{Observational Signatures of Simulated Reconnection Events in the
            Solar Chromosphere and Transition Region}",
  journal = apj,
     year = 2009,
    pages = {submitted}
}

@ARTICLE{Heinemann2007,
   author = {{Heinemann}, T. and {Nordlund}, {\AA}. and {Scharmer}, G. B. and
            {Spruit}, H. C.},
    title = "{MHD Simulations of Penumbra Fine Structure}",
  journal = apj,
     year = 2007,
   volume = 669,
    pages = {1390-1394}
}

@ARTICLE{Heinzel1999,
   author = {{Heinzel}, P. and {Mein}, N. and {Mein}, P.},
    title = "{Cloud Model with Variable Source Function for Solar H$\alpha$
            Structures. II.\ Dynamical Models}",
  journal = aa,
     year = 1999,
   volume = 346,
    pages = {322-328}
}

@INPROCEEDINGS{Henney2009,
   author = {{Henney}, C. J. and {Keller}, C. U. and {Harvey}, J. W. and
            {Georgoulis}, M. K. and {Hadder}, N. L. and {Norton}, A. A. and
            {Raouafi}, N.-E. and {Toussaint}, R. M.},
    title = "{SOLIS Vector Spectromagnetograph: Status and Science}",
booktitle = {Solar Polarization V},
     year = 2009,
   series = asp,
   volume = 405,
   editor = {{Berdyugina}, S. V. and {Nagendra}, K. N. and {Ramelli}, R.},
    pages = {47-50}
}

@BOOK{Hentschel1992,
   author = {{Hentschel}, K.},
    title = "{Der Einstein-Turm}",
publisher = {Spektrum Akademischer Verlag, Heidelberg},
     year = 1992
}

@INPROCEEDINGS{Hermans1986,
   author = {{Hermans}, L. M. and {Martin}, S. F.},
    title = "{Small-Scale Eruptive Filaments on the Quiet Sun}",
booktitle = {Coronal and Prominence Plasmas},
     year = 1986,
   editor = {{Poland}, A. I.},
    pages = {369-375}
}

@INPROCEEDINGS{Hill2006,
   author = {{Hill}, F. and {Beckers}, J. and {Brandt}, P. and {Briggs}, J. and
            {Brown}, T. and {Brown}, W. and {Collados}, M. and {Denker}, C. and
            {Fletcher}, S. and {Hegwer}, S. and {Horst}, T. and {Komsa}, M. and
            {Kuhn}, J. and {Lecinski}, A. and {Lin}, H. and {Oncley}, S. and
            {Penn}, M. and {Radick}, R. and {Rimmele}, T. and
            {Socas-Navarro}, H. and {Streander}, K.},
    title = "{Site Testing for the Advanced Technology Solar Telescope}",
booktitle = {Ground-Based and Airborne Telescopes},
     year = 2006,
   series = posp,
   volume = 6267,
   editor = {{Stepp}, L. M.},
    pages = {62671T}
}

@article{Hill2004a,
   author = {{Hill}, F. and {Beckers}, J. and {Brown}, T. and {Collados}, M.
            and {Denker}, C. and {Kuhn}, J. and {Penn}, M. and {Socas-Navarro},
            H. and {Soltau}, D. and {Streander}, K.},
    title = "{ATST Site Survey Working Group Final Report}",
  journal = {ATST Project Document},
     year = 2004,
   volume = 21
}

@INPROCEEDINGS{Hill2004b,
   author = {{Hill}, F. and {Beckers}, J. and {Brandt}, P. and {Briggs}, J. and
            {Brown}, T. and {Brown}, W. and {Collados}, M. and {Denker}, C. and
            {Fletcher}, S. and {Hegwer}, S. and {Horst}, T. and {Komsa}, M. and
            {Kuhn}, J. and {Lecinski}, A. and {Lin}, H. and {Oncley}, S. and
            {Penn}, M. and {Rimmele}, T. R. and {Socas-Navarro}, H. and
            {Streander}, K.},
    title = "{Solar Site Testing for the Advanced Technology Solar Telescope}",
booktitle = {Ground-Based Telescopes},
   series = posp,
     year = 2004,
   volume = 5489,
   editor = {{Oschmann}, J. M.},
    pages = {122-129}
}

@ARTICLE{Hill1994,
   author = {{Hill}, F. and {Fischer}, G. and {Forgach}, S. and {Grier}, J. and
            {Leibacher}, J. W. and {Jones}, H. P. and {Jones}, P. B. and
            {Kupke}, R. and {Stebbins}, R. T. and {Clay}, D. W.},
    title = "{The Global Oscillation Network Group Site Survey. II. Results}",
  journal = sp,
     year = 1994,
   volume = 152,
    pages = {351-379}
}

@ARTICLE{Hirzberger2009,
   author = {{Hirzberger}, J. and {Riethm{\"u}ller}, T. and {Lagg}, A. and
            {Solanki}, S. K. and {Kobel}, P.},
    title = "{High-Resolution Spectro-Polarimetry of a Flaring Sunspot
            Penumbra}",
  journal = aa,
     year = 2009,
   volume = 505,
    pages = {771-790}
}

@ARTICLE{Hirzberger2003,
   author = {{Hirzberger}, J.},
    title = "{Imaging Spectroscopy of Solar Pores}",
  journal = aa,
     year = 2003,
   volume = 405,
    pages = {331-340}
}

@ARTICLE{Hirzberger2001,
   author = {{Hirzberger}, J. and {Koschinsky}, M. and {Kneer}, F. and
            {Ritter}, C.},
    title = "{High Resolution 2D-Spectroscopy of Granular Dynamics}",
  journal = aa,
     year = 2001,
   volume = 367,
    pages = {1011-1021}
}

@ARTICLE{Hock2008,
   author = {{Hock}, R. A. and {Eparvier}, F. G.},
    title = "{Cross-Calibration of TIMED SEE and SOHO EIT Irradiances}",
  journal = sp,
     year = 2008,
   volume = 250,
    pages = {207-219}
}

@ARTICLE{Hofmann2009,
   author = {{Hofmann}, A. and {Rendtel}, J. and {Arlt}, K.},
    title = "{Toward Polarimetry with GREGOR -- Testing the GREGOR Polarimetric
            Unit}",
  journal = ceab,
     year = 2009,
   volume = 33,
    pages = {317-325}
}

@ARTICLE{Hofmann2008,
   author = {{Hofmann}, A.},
    title = "{Polarimetric Projects with GREGOR}",
  journal = ceab,
     year = 2008,
   volume = 32,
    pages = {17-24}
}

@ARTICLE{Holman2003,
   author = {{Holman}, G. D. and {Sui}, L. and {Schwartz}, R. A. and
            {Emslie}, A. G.},
    title = "{Electron Bremsstrahlung Hard X-Ray Spectra, Electron
            Distributions, and Energetics in the 2002 July 23 Solar Flare}",
  journal = apjl,
     year = 2003,
   volume = 595,
    pages = {L97-L101}
}

@ARTICLE{Hong2014,
   author = {{Hong}, J. and {Ding}, M. D. and {Li}, Y. and {Fang}, C. and 
            {Cao}, W.},
    title = "{Spectral Observations of Ellerman Bombs and Fitting with a 
            Two-Cloud Model}",
  journal = apj,
     year = 2014,
   volume = 792,
      eid = {13},
    pages = {13},
      doi = {10.1088/0004-637X/792/1/13}
}

@ARTICLE{Howard1990,
   author = {{Howard}, R. F.},
    title = "{The Magnetic Fields of Active Regions. II - Rotation}",
  journal = sp,
     year = 1990,
   volume = 126,
    pages = {299-309}
}

@ARTICLE{Hu2003,
   author = {{Hu}, H. and {Liu}, W. T.},
    title = "{Oceanic Thermal and Biological Responses to Santa Ana Winds}",
  journal = grl,
     year = 2003,
   volume = 30,
    pages = {50-51}
}

@ARTICLE{Hudson1972,
   author = {{Hudson}, H. S.},
    title = "{Thick-Target Processes and White-Light Flares}",
  journal = sp,
     year = 1972,
   volume = 24,
    pages = {414-428},
      doi = {10.1007/BF00153384}
}



%====     IIII    ==============================================================

@ARTICLE{Ichimoto2008,
   author = {{Ichimoto}, K. and {Lites}, B. and {Elmore}, D. and {Suematsu}, Y.
            and{Tsuneta}, S. and {Katsukawa}, Y. and {Shimizu}, T. and {Shine},
            R. and {Tarbell}, T. and {Title}, A. and {Kiyohara}, J. and
           {Shinoda}, K. and {Card}, G. and {Lecinski}, A. and {Streander}, K.
           and {Nakagiri}, M. and {Miyashita}, M. and {Noguchi}, M. and
           {Hoffmann}, C. and {Cruz}, T.},
    title = "{Polarization Calibration of the Solar Optical Telescope onboard
             Hinode}",
  journal = sp,
     year = 2008,
   volume = 249,
    pages = {233-261}
}

@ARTICLE{Ichimoto2007,
   author = {{Ichimoto}, K. and {Suematsu}, Y. and {Tsuneta}, S. and
            {Katsukawa}, Y. and {Shimizu}, T. and {Shine}, R. A. and
            {Tarbell}, T. D. and {Title}, A. M. and {Lites}, B. W. and
            {Kubo}, M. and {Nagata}, S.},
    title = "{Twisting Motions of Sunspot Penumbral Filaments}",
  journal = pasj,
     year = 2007,
   volume = 318,
    pages = {1597-1599}
}

@ARTICLE{Ishikawa2010,
   author = {{Ishikawa}, R. and {Tsuneta}, S.},
    title = "{Spatial and Temporal Distributions of Transient Horizontal
            Magnetic Fields with Deep Exposure}",
  journal = apjl,
     year = 2010,
   volume = 718,
    pages = {L171-L175},
      doi = {10.1088/2041-8205/718/2/L171}
}



%====     JJJJ    ==============================================================

@INPROCEEDINGS{Jaegers2008,
   author = {{J{\"a}gers}, A. P. L. and {Sliepen}, G. and
            {Bettonvil}, F. C. M. and {Hammerschlag}, R. H.},
    title = "{Fast Foldable Tent Domes}",
booktitle = {Advanced Optical and Mechanical Technologies in Telescopes and
            Instrumentation},
     year = 2008,
   series = posp,
   volume = 7018,
   editor = {{Atad-Ettedgui}, E. and {Lemke}, D.},
    pages = {70181R}
}

@ARTICLE{Johannesson1998,
   author = {{Johannesson}, A. and {Marquette}, W. H. and {Zirin}, H.},
    title = "{A 10-Year Set of Ca\,{\sc ii} K-Line Filtergrams}",
  journal = sp,
     year = 1998,
   volume = 177,
    pages = {265-278}
}

@ARTICLE{Johannesson1995,
   author = {{Johannesson}, A. and {Marquette}, W. and {Zirin}, H.},
    title = "{Reproduction of the Lyman-$\alpha$ Irradiance Variability from
            Analysis of Full-Disk Images in the Ca\,{\sc ii} K-Line}",
  journal = sp,
     year = 1995,
   volume = 161,
    pages = {201-204}
}

@ARTICLE{Judge2010,
   author = {{Judge}, P. G. and {Tritschler}, A. and {Uitenbroek}, H. and 
            {Reardon}, K. and {Cauzzi}, G. and {de Wijn}, A.},
    title = "{Fabry-P{\'e}rot Versus Slit Spectropolarimetry of Pores and
            Active Network: Analysis of IBIS and Hinode Data}",
  journal = apj,
     year = 2010,
   volume = 710,
    pages = {1486-1497}
}



%====     KKKK    ==============================================================

@BOOK{Kalkofen2009,
   author = {{Kalkofen}, W.},
    title = "{Numerical Radiative Transfer}",
publisher = {Cambridge University Press},
  address = {New York},
     year = 2009
}

@ARTICLE{Kane2010,
   author = {{Kane}, R. P.},
    title = "{Gnevyshev Peaks in the CME Average Speeds in Cycle 23}",
  journal = sp,
     year = 2010,
   volume = 261,
    pages = {209-213}
}

@INPROCEEDINGS{Keil2004,
   author = {{Keil}, S. and {Oschmann}, J. M. and {Rimmele}, T. R. and
            {Hubbard}, R. and {Warner}, M. and {Price}, R. and
            {Dalrymple}, N. and {Goodrich}, B. and {Hegwer}, S. and
            {Hill}, F. and {Wagner}, J.},
    title = "{Advanced Technology Solar Telescope: Conceptual Design and
            Status}",
booktitle = {Ground-Based Telescopes},
   series = posp,
     year = 2004,
   volume = 5489,
   editor = {{Oschmann}, J. M.},
    pages = {625-637}
}

@ARTICLE{Keil1999,
   author = {{Keil}, S. L. and {Balasubramaniam}, K. S. and
            {Smaldone}, L. A. and {Reger}, B.},
    title = "{Velocities in Solar Pores}",
  journal = apj,
     year = 1999,
    volume = 510,
    pages = {422-443}
}

@INPROCEEDINGS{Keller2003,
   author = {{Keller}, C. U. and {Harvey}, J. W. and {Giampapa}, M. S.},
    title = "{SOLIS: An Innovative Suite of Synoptic Instruments}",
booktitle = {Innovative Telescopes and Instrumentation for Solar Astrophysics},
     year = 2003,
   series = posp,
   volume = 4853,
   editor = {{Keil}, S. L. and {Avakyan}, S. V.},
    pages = {194-204}
}

@ARTICLE{Keller1992,
   author = {{Keller}, C. U. and {von der L{\"u}he}, O.},
    title = "{Solar Speckle Polarimetry}",
  journal = aa,
     year = 1992,
   volume = 261,
    pages = {321-328}
}

@ARTICLE{Kentischer1998,
   author = {{Kentischer}, T. J. and {Schmidt}, W. and {Sigwarth}, M. and
            {Uexkuell}, M. V.},
    title = "{TESOS, a Double Fabry-Perot Instrument for Solar Spectroscopy}",
  journal = aa,
     year = 1998,
   volume = 340,
    pages = {569-578}
}

@ARTICLE{Keppens1996,
   author = {{Keppens}, R. and {Martinez Pillet}, V.},
    title = "{The Magnetic Structure of Pores and Sunspots Derived from Advanced
            Stokes Polarimeter Data}",
  journal = aa,
     year = 1996,
   volume = 316,
    pages = {229-242}
}

@PHDTHESIS{Kiess2013,
   author = {{Kiess}, C.},
    title = "{Cycle Dependence of Sunspot Properties}",
     type = {Diploma Thesis}, 
   school = {Universit{\"a}t Freiburg},
     year = 2013
}


@ARTICLE{Komm2010,
   author = {{Komm}, R. and {Ferguson}, R. and {Hill}, F. and {Barnes}, G. and
            {Leka}, K. D.},
    title = "{Subsurface Vorticity of Flaring versus Flare-Quiet Active
            Regions}",
  journal = sp,
     year = 2010,
     note = {in press}
}

@ARTICLE{Kontar2006,
   author = {{Kontar}, E. P. and {MacKinnon}, A. L. and {Schwartz}, R. A. 
            and {Brown}, J. C.},
    title = "{Compton Backscattered and Primary X-Rays from Solar Flares: Angle
            Dependent Green's Function Correction for Photospheric Albedo}",
  journal = aa,
     year = 2006,
   volume = 446,
    pages = {1157-1163}
}

@ARTICLE{Kosovichev2007,
   author = {{Kosovichev}, A. G. and {HMI Science Team}},
    title = "{Helioseismology Program for Solar Dynamics Observatory}",
  journal = an,
     year = 2007,
   volume = 328,
    pages = {339-351}
}

@ARTICLE{Kosugi2007,
   author = {{Kosugi}, T. and {Matsuzaki}, K. and {Sakao}, T. and {Shimizu}, T.
            and {Sone}, Y. and {Tachikawa}, S. and {Hashimoto}, T. and
            {Minesugi}, K. and {Ohnishi}, A. and {Yamada}, T. and {Tsuneta}, S.
            and {Hara}, H. and {Ichimoto}, K. and {Suematsu}, Y. and {Shimojo},
            M. and {Watanabe}, T. and {Shimada}, S. and {Davis}, J. M. and
            {Hill}, L. D. and {Owens}, J. K. and {Title}, A. M. and {Culhane},
            J. L. and {Harra}, L. K. and {Doschek}, G. A. and {Golub}, L.},
    title = "{The Hinode (Solar-B) Mission: An Overview}",
  journal = sp,
     year = 2007,
   volume = 243,
    pages = {3-17},
      doi = {10.1007/s11207-007-9014-6}
}

@INPROCEEDINGS{Kroedel2006,
   author = {{Kr{\"o}del}, M. R. and {Luichtel}, G. and {Volkmer}, R.},
    title = "{The Cesic Ceramic Optics of the GREGOR Telescope}",
booktitle = {Optomechanical Technologies for Astronomy},
     year = 2006,
   series = posp,
   volume = 6273,
   editor = {{Atad-Ettedgui}, E. and {Lemke}, D.},
    pages = {62730Q}
}

@ARTICLE{Krucker2011,
   author = {{Krucker}, S. and {Hudson}, H. S. and {Jeffrey}, N. L. S. and
            {Battaglia}, M. and {Kontar}, E. P. and {Benz}, A. O. and
            {Csillaghy}, A. and {Lin}, R. P.},
    title = "{High-Resolution Imaging of Solar Flare Ribbons and its Implication
            on the Thick-Target Beam Model}",
  journal = apj,
     year = 2011,
   volume = 739,
    pages = {96},
      doi = {10.1088/0004-637X/739/2/96}
}

@INPROCEEDINGS{Koutchmy2009,
   author = {{Koutchmy}, S. and {Le Piouffle}, V.},
    title = "{Isolated Quasi-Axisymmetric sunspots}",
booktitle = "{Cosmic Magnetic Fields: From Planets, to Stars and Galaxies}",
     year = 2009,
   series = iaus,
   volume = 259,
   editor = {{Strassmeier}, K. G. and {Kosovichev}, A. G. and
            {Beckman}, J. E.},
    pages = {227-228},
      doi = {10.1017/S174392130903049X}
}

@ARTICLE{Kubo2008,
   author = {{Kubo}, M. and {Lites}, B. W. and {Ichimoto}, K. and
            {Shimizu}, T. and {Suematsu}, Y. and {Katsukawa}, Y. and
            {Tarbell}, T. D. and {Shine}, R. A. and {Title}, A. M. and
            {Nagata}, S. and {Tsuneta}, S.},
    title = "{Disintegration of Magnetic Flux in Decaying Sunspots as Observed
            with the Hinode SOT}",
  journal = apj,
     year = 2008,
   volume = 681,
    pages = {1677-1687}
}

@ARTICLE{Kubo2007,
   author = {{Kubo}, M. and {Yokoyama}, T. and {Katsukawa}, Y. and 
            {Lites}, B. and {Tsuneta}, S. and {Suematsu}, Y. and 
            {Ichimoto}, K. and {Shimizu}, T. and {Nagata}, S. and 
            {Tarbell}, T. D. and {Shine}, R. A. and {Title}, A. M. and 
            {Elmore}, D.},
    title = "{Hinode Observations of a Vector Magnetic Field Change Associated
            with a Flare on 2006 December 13}",
  journal = pasj,
     year = 2007,
   volume = 59,
    pages = {779-784}
}

@ARTICLE{Kuckein2012b,
   author = {{Kuckein}, C. and {Mart{\'{\i}}nez Pillet}, V. and {Centeno}, R.
	},
    title = "{An active region filament studied simultaneously in the chromosphere and photosphere. II. Doppler velocities}",
  journal = aa,
archivePrefix = "arXiv",
   eprint = {1204.5090},
 primaryClass = "astro-ph.SR",
     year = 2012,
   volume = 542,
      eid = {A112},
    pages = {A112},
      doi = {10.1051/0004-6361/201218887},
}

@ARTICLE{Kuhn1991,
   author = {{Kuhn}, J. R. and {Lin}, H. and {Loranz}, D.},
    title = "{Gain Calibrating Nonuniform Image-Array Data Using Only the Image
            Data}",
  journal = pasp,
     year = 1991,
   volume = 103,
    pages = {1097-1108}
}

@ARTICLE{Kumar2010,
   author = {{Kumar}, P. and {Srivastava}, A. K. and {Filippov}, B. and
            {Uddin}, W.},
    title = "{Multiwavelength Study of M8.9/3B Solar Flare from AR NOAA 10960}",
  journal = sp,
     year = 2010,
   volume = 266,
    pages = {39-58}
}

@ARTICLE{Kuenzel1960,
   author = {{K{\"u}nzel}, H.},
    title = "{Die Flare-H{\"a}ufigkeit in Fleckengruppen unterschiedlicher
            Klasse und magnetischer Struktur}",
  journal = an,
     year = 1960,
   volume = 285,
    pages = {271-273}
}

%====     LLLL    ==============================================================

@ARTICLE{Labonte1979,
   author = {{Labonte}, B. J.},
    title = "{Activity in the Quiet Sun. I.\ Observations of Macrospicules in
            H$\alpha$ and D3}",
  journal = sp,
     year = 1979,
   volume = 61,
    pages = {283-296}
}

@ARTICLE{Labs1968,
   author = {{Labs}, D. and {Neckel}, H.},
    title = "{The Radiation of the Solar Photosphere from 2000 {\AA} to 100
            {$\mu$}m}",
  journal = zap,
     year = 1968,
   volume = 69,
    pages = {1-73}
}

@ARTICLE{Lagg2007,
   author = {{Lagg}, A. and {Woch}, J. and {Solanki}, S.~K. and {Krupp}, N.
	},
    title = "{Supersonic downflows in the vicinity of a growing pore. 
        Evidence of unresolved magnetic fine structure at chromospheric heights}",
  journal = aa,
 keywords = {Sun: chromosphere, Sun: magnetic fields, Sun: infrared},
     year = 2007,
   volume = 462,
    pages = {1147-1155},
      doi = {10.1051/0004-6361:20054700}
}

@INPROCEEDINGS{Lagg2009,
   author = {{Lagg}, A. and {Ishikawa}, R. and {Merenda}, L. and {Wiegelmann}, T. and 
	{Tsuneta}, S. and {Solanki}, S.~K.},
    title = "{Internetwork Horizontal Magnetic Fields in the Quiet Sun Chromosphere: Results from a 
Joint 
Hinode/VTT Study}",
booktitle = {The Second Hinode Science Meeting: Beyond Discovery-Toward Understanding},
     year = 2009,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 415,
   editor = {{Lites}, B. and {Cheung}, M. and {Magara}, T. and {Mariska}, J. and 
	{Reeves}, K.},
    pages = {327}
}

@ARTICLE{Lagg2004,
   author = {{Lagg}, A. and {Woch}, J. and {Krupp}, N. and {Solanki}, S.~K.
	},
    title = "{Retrieval of the full magnetic vector with the He I multiplet at 1083 nm. Maps of an emerging flux region}",
  journal = aa,
     year = 2004,
   volume = 414,
    pages = {1109-1120},
      doi = {10.1051/0004-6361:20031643}
}

@ARTICLE{Lamb2008,
   author = {{Lamb}, D. A. and {DeForest}, C. E. and {Hagenaar}, H. J. and
            {Parnell}, C. E. and {Welsch}, B. T.},
    title = "{Solar Magnetic Tracking. II. The Apparent Unipolar Origin of
            Quiet-Sun Flux}",
  journal = apj,
     year = 2008,
   volume = 674,
    pages = {520-529}
}

@ARTICLE{Langhans2007,
   author = {{Langhans}, K. and {Scharmer}, G. B. and {Kiselman}, D. and
            {L{\"o}fdahl}, M. G.},
    title = "{Observations of Dark-Cored Filaments in Sunspot Penumbrae}",
  journal = aa,
     year = 2007,
   volume = 464,
    pages = {763-774}
}

@ARTICLE{Langhans2005,
   author = {{Langhans}, K. and {Scharmer}, G. B. and {Kiselman}, D. and
            {L{\"o}fdahl}, M. G. and {Berger}, T. E.},
    title = "{Inclination of Magnetic Fields and Flows in Sunspot Penumbrae}",
  journal = aa,
     year = 2005,
   volume = 436,
    pages = {1087-1101}
}

@ARTICLE{Landi2006,
   author = {{Landi}, E. and {Del Zanna}, G. and {Young}, P. R. and
            {Dere}, K. P. and {Mason}, H. E. and {Landini}, M.},
    title = "{CHIANTI--An Atomic Database for Emission Lines. VII. New Data for
            X-Rays and Other Improvements}",
  journal = apjss,
     year = 2006,
   volume = 162,
    pages = {261-280}
}

@ARTICLE{Lean1998,
   author = {{Lean}, J. L. and {Cook}, J. and {Marquette}, W. and
            {Johannesson}, A.},
    title = "{Magnetic Sources of the Solar Irradiance Cycle}",
  journal = apj,
     year = 1998,
   volume = 492,
    pages = {390-401}
}

@ARTICLE{Lean1997,
   author = {{Lean}, J.},
    title = "{The Sun's Variable Radiation and its Relevance for Earth}",
  journal = araa,
     year = 1997,
   volume = 35,
    pages = {33-67}
}

@ARTICLE{Lee2000,
   author = {{Lee}, C.-Y. and {Chae}, J. and {Wang}, H.},
    title = "{Dynamical Characteristics of Small-Scale H{$\alpha$} Upflow Events
            on the Quiet Sun}",
  journal = apj,
     year = 2000,
   volume = 545,
    pages = {1124-1134}
}

@ARTICLE{Lee1980,
   author = {{Lee}, D. T. and {Schachter}, B. J.},
    title = "{Two Algorithms for Constructing a Delaunay Triangulation}",
  journal = "Int.\ J.\ Comp.\ Inform.\ Sci",
     year = 1980,
   volume = 9,
    pages = {219-242}
}

@ARTICLE{Leighton1969,
   author = {{Leighton}, R. B.},
    title = "{A Magneto-Kinematic Model of the Solar Cycle}",
  journal = apj,
     year = 1969,
   volume = 156,
    pages = {1-26}
}

@ARTICLE{Leighton1962,
   author = {{Leighton}, R. B. and {Noyes}, R. W. and {Simon}, G. W.},
    title = "{Velocity Fields in the Solar Atmosphere. I. Preliminary Report.}",
  journal = apj,
     year = 1962,
   volume = 135,
    pages = {474-510}
}

@ARTICLE{Leka2001,
   author = {{Leka}, K. D. and {Steiner}, O.},
    title = "{Understanding Small Solar Magnetic Structures: Comparing Numerical
            Simulations to Observations}",
  journal = apj,
     year = 2001,
   volume = 552,
    pages = {354-371}
}

@ARTICLE{Leka1998,
   author = {{Leka}, K. D. and {Skumanich}, A.},
    title = "{The Evolution of Pores and the Development of Penumbrae}",
  journal = apj,
     year = 1998,
   volume = 507,
    pages = {454-469}
}

@ARTICLE{Leenaarts2006,
   author = {{Leenaarts}, J. and {Rutten}, R. J. and {Carlsson}, M. and
            {Uitenbroek}, H.},
    title = "{A Comparison of Solar Proxy-Magnetometry Diagnostics}",
  journal = aa,
     year = 2006,
   volume = 452,
    pages = {L15-L18}
}

@ARTICLE{Lemen2012,
   author = {{Lemen}, J. R. and {Title}, A. M. and {Akin}, D. J. and
            {Boerner}, P. F. and {Chou}, C. and {Drake}, J. F. and
            {Duncan}, D. W. and {Edwards}, C. G. and {Friedlaender}, F. M. and
            {Heyman}, G. F. and {Hurlburt}, N. E. and {Katz}, N. L. and
            {Kushner}, G. D. and {Levay}, M. and {Lindgren}, R. W. and 
            {Mathur}, D. P. and {McFeaters}, E. L. and {Mitchell}, S. and 
            {Rehse}, R. A. and {Schrijver}, C. J. and {Springer}, L. A. and 
            {Stern}, R. A. and {Tarbell}, T. D. and {Wuelser}, J.-P. and 
            {Wolfson}, C. J. and {Yanari}, C. and {Bookbinder}, J. A. and 
            {Cheimets}, P. N. and {Caldwell}, D. and {Deluca}, E. E. and 
            {Gates}, R. and {Golub}, L. and {Park}, S. and
            {Podgorski}, W. A. and {Bush}, R. I. and {Scherrer}, P. H. and
            {Gummin}, M. A. and {Smith}, P. and {Auker}, G. and {Jerram}, P. and
            {Pool}, P. and {Soufli}, R. and {Windt}, D. L. and
            {Beardsley}, S. and {Clapp}, M. and {Lang}, J. and {Waltham}, N.},
    title = "{The Atmospheric Imaging Assembly (AIA) on the Solar Dynamics
            Observatory (SDO)}",
  journal = sp,
     year = 2012,
   volume = 275,
    pages = {17-40},
      doi = {10.1007/s11207-011-9776-8}
}

@ARTICLE{Lin2004,
   author = {{Lin}, H. and {Penn}, M. J.},
    title = "{The Advanced Technology Solar Telescope Site Survey Sky
            Brightness Monitor}",
  journal = pasp,
     year = 2004,
   volume = 116,
    pages = {652-666}
}

@ARTICLE{Lin2003,
   author = {{Lin}, Y. and {Engvold}, O. R. and {Wiik}, J. E.},
    title = "{Counterstreaming in a Large Polar Crown Filament}",
  journal = sp,
     year = 2003,
   volume = 216,
    pages = {109-120}
}

@ARTICLE{Lin2002,
   author = {{Lin}, R. P. and {Dennis}, B. R. and {Hurford}, G. J. and 
            {Smith}, D. M. and {Zehnder}, A. and {Harvey}, P. R. and 
            {Curtis}, D. W. and {Pankow}, D. and {Turin}, P. and 
            {Bester}, M. and {Csillaghy}, A. and {Lewis}, M. and 
            {Madden}, N. and {van Beek}, H. F. and {Appleby}, M. and 
            {Raudorf}, T. and {McTiernan}, J. and {Ramaty}, R. and 
            {Schmahl}, E. and {Schwartz}, R. and {Krucker}, S. and 
            {Abiad}, R. and {Quinn}, T. and {Berg}, P. and {Hashii}, M. and
            {Sterling}, R. and {Jackson}, R. and {Pratt}, R. and 
            {Campbell}, R. D. and {Malone}, D. and {Landis}, D. and
            {Barrington-Leigh}, C. P. and {Slassi-Sennou}, S. and {Cork}, C. and
            {Clark}, D. and {Amato}, D. and {Orwig}, L. and {Boyle}, R. and
            {Banks}, I. S. and {Shirey}, K. and {Tolbert}, A. K. and 
            {Zarro}, D. and {Snow}, F. and {Thomsen}, K. and {Henneck}, R. and
            {McHedlishvili}, A. and {Ming}, P. and {Fivian}, M. and 
            {Jordan}, J. and {Wanner}, R. and {Crubb}, J. and {Preble}, J. and
            {Matranga}, M. and {Benz}, A. and {Hudson}, H. and 
            {Canfield}, R. C. and {Holman}, G. D. and {Crannell}, C. and
            {Kosugi}, T. and {Emslie}, A. G. and {Vilmer}, N. and 
            {Brown}, J. C. and {Johns-Krull}, C. and {Aschwanden}, M. and
            {Metcalf}, T. and {Conway}, A.},
    title = "{The Reuven Ramaty High-Energy Solar Spectroscopic Imager
            (RHESSI)}",
  journal = sp,
     year = 2002,
   volume = 210,
    pages = {3-32}
}

@ARTICLE{Lin1999,
   author = {{Lin}, H. and {Rimmele}, T.},
    title = "{The Granular Magnetic Fields of the Quiet Sun}",
  journal = apj,
     year = 1999,
   volume = 514,
    pages = {448-455}
}

@INPROCEEDINGS{Lites2007,
   author = {{Lites}, B. W. and {Elmore}, D. F. and {Streander}, K. V. and 
            {Hoffmann}, C. M. and {Tarbell}, T. D. and {Title}, A. M. and
            {Shine}, R. A. and {Ichimoto}, K. and {Tsuneta}, S. and
            {Shimizu}, T. and {Suematsu}, Y.},
    title = "{Performance Characteristics of the Solar-B Spectro-Polarimeter}",
booktitle = {New Solar Physics with Solar-B Mission},
     year = 2007,
   series = asp,
   volume = 369,
   editor = {{Shibata}, K. and {Nagata}, S. and {Sakurai}, T.},
   pages = {55-58}
}

@ARTICLE{Lites1998,
   author = {{Lites}, B. W. and {Skumanich}, A. and {Martinez Pillet}, V.},
    title = "{Vector Magnetic Fields of Emerging Solar Flux. I.\ Properties at
            the Site of Emergence}",
  journal = aa,
     year = 1998,
   volume = 333,
    pages = {1053-1068}
}

@ARTICLE{Lites1993,
   author = {{Lites}, B. W. and {Elmore}, D. F. and {Seagraves}, P. 
            and {Skumanich}, A. P.},
    title = "{Stokes Profile Analysis and Vector Magnetic Fields. VI. Fine Scale
            Structure of a Sunspot}",
  journal = apj,
     year = 1993,
   volume = 418,
    pages = {928-942}
}

@ARTICLE{Lites1990a,
   author = {{Lites}, B. W. and {Scharmer}, G. B. and {Skumanich}, A.},
    title = "{High-Resolution Spectra of Solar Magnetic Features. I. Analysis
            of Penumbral Fine Structure}",
  journal = apj,
     year = 1990,
   volume = 355,
    pages = {329-341}
}

@ARTICLE{Lites1990b,
   author = {{Lites}, B. W. and {Skumanich}, A.},
    title = "{Stokes Profile Analysis and Vector Magnetic Fields. V.\ The
            Magnetic Field Structure of Large Sunspots Observed with Stokes II}",
  journal = apj,
     year = 1990,
   volume = 348,
    pages = {747-760}
}

@ARTICLE{Liu2010,
   author = {{Liu}, R. and {Liu}, C. and {Wang}, S. and {Deng}, N. and
            {Wang}, H.},
    title = "{Sigmoid-to-Flux-Rope Transition Leading to a Loop-Like Coronal
            Mass Ejection}",
  journal = apjl,
     year = 2010,
   volume = 725,
    pages = {L84-L90},
      doi = {10.1088/2041-8205/725/1/L84}
}

@ARTICLE{Liu2005,
   author = {{Liu}, C. and {Deng}, N. and {Liu}, Y. and {Falconer}, D. and
            {Goode}, P. R. and {Denker}, C. and {Wang}, H.},
    title = "{Rapid Change of $\delta$ Spot Structure Associated with Seven
            Major Flares}",
  journal = apj,
     year = 2005,
   volume = 622,
    pages = {722-736}
}

@ARTICLE{Liu2001,
   author = {{Liu}, Z. and {Beckers}, J. M.},
    title = "{Comparative Solar Seeing and Scintillation Studies at the Fuxian
            Lake Solar Station}",
  journal = sp,
     year = 2001,
   volume = 198,
    pages = {197-209}
}

@ARTICLE{Livi1985,
   author = {{Livi}, S. H. B. and {Wang}, J. and {Martin}, S. F.},
    title = "{The Cancellation of Magnetic Flux. I.\ On the Quiet Sun}",
  journal = ajp,
     year = 1985,
   volume = 38,
    pages = {855-873}
}

@ARTICLE{Loefdahl2010,
   author = {{L{\"o}fdahl}, M. G.},
    title = "{Evaluation of Image-Shift Measurement Algorithms for Solar
            Shack-Hartmann Wavefront Sensors}",
  journal = aa,
     year = 2010,
     note = {in press}
}

@INPROCEEDINGS{Loefdahl2002,
   author = {{L{\"o}fdahl}, M. G.},
    title = "{Multi-Frame Blind Deconvolution with Linear Equality Constraints}",
booktitle = {Image Reconstruction from Incomplete Data},
     year = 2002,
   series = posp,
   volume = 4792,
   editor = {{Bones}, P. J. and {Fiddy}, M. A. and {Millane}, R. P.},
    pages = {146-155},
      doi = {10.1117/12.451791}
}

@INPROCEEDINGS{Loefdahl2007,
   author = {{L{\"o}fdahl}, M. G. and {van Noort}, M. J. and {Denker}, C.},
    title = "{Solar Image Restoration}",
booktitle = {Modern Solar Facilities -- Advanced Solar Science},
     year = 2007,
   editor = {{Kneer}, F. and {Puschmann}, K. G. and {Wittmann}, A. D.},
    pages = {119-126}
}

@ARTICLE{LoehnerBoettcher2013,
   author = {{L{\"o}hner-B{\"o}ttcher}, J. and {Schlichenmaier}, R.},
    title = "{Correlations between Sunspots and their Moat Flows}",
  journal = aa,
     year = 2013,
   volume = 551,
      eid = {A105},
    pages = {A105},
      doi = {10.1051/0004-6361/201220543}
}

@ARTICLE{Lohmann1983,
   author = {{Lohmann}, A. W. and {Weigelt}, G. and {Wirnitzer}, B.},
    title = "{Speckle Masking in Astronomy -- Triple Correlation Theory and
            Applications}",
  journal = ao,
     year = 1983,
   volume = 22,
    pages = {4028-4037}
}

@ARTICLE{LopezFuentes2000,
   author = {{L{\'o}pez Fuentes}, M. C. and {Demoulin}, P. and
            {Mandrini}, C. H. and {van Driel-Gesztelyi}, L.},
    title = "{The Counterkink Rotation of a Non-Hale Active Region}",
  journal = apj,
     year = 2000,
   volume = 544,
    pages = {540-549}
}



%====     MMMM    ==============================================================

@ARTICLE{Ma2008,
   author = {{Ma}, J. and {Wang}, J.-S. and {Denker}, C. and {Wang}, H.-M.},
    title = "{Optical Design of Multilayer Achromatic Waveplate by Simulated
            Annealing Algorithm}",
  journal = chinjaa,
     year = 2008,
   volume = 8,
    pages = {349-361}
}

@INPROCEEDINGS{Ma2004,
   author = {{Ma}, J. and {Wang}, J. and {Cao}, W. and {Denker}, C. and
            {Wang}, H.},
    title = "{Near Infrared (NIR) Achromatic Phase Retarder}",
booktitle = {Current Developments in Lens Design and Optical Engineering},
     year = 2004,
   series = posp,
   volume = 5523,
   editor = {{Mouroulis}, P. Z. and {Smith}, W. J. and {Johnson}, R. B.},
    pages = {139-147}
}

@ARTICLE{Maltby1975,
   author = {{Maltby}, P.},
    title = "{The Chromospheric Evershed Flow}",
  journal = sp,
     year = 1975,
   volume = 43,
    pages = {91-105}
}

@ARTICLE{Mariska2007,
   author = {{Mariska}, J. T. and {Warren}, H. P. and {Ugarte-Urra}, I. and
            {Brooks}, D. H. and {Williams}, D. R. and {Hara}, H.},
    title = "{Hinode EUV Imaging Spectrometer Observations of Solar Active
            Region Dynamics}",
  journal = pasj,
     year = 2007,
   volume = 59,
    pages = {713-719}
}

@ARTICLE{Marquez2006,
   author = {{M{\'a}rquez}, I. and {S{\'a}nchez Almeida}, J. and
            {Bonet}, J. A.},
    title = "{High-Resolution Proper Motions in a Sunspot Penumbra}",
  journal = apj,
     year = 2006,
   volume = 638,
    pages = {553-563}
}

@INPROCEEDINGS{Markwardt2009,
   author = {{Markwardt}, C. B.},
    title = "{Non-Linear Least-Squares Fitting in IDL with MPFIT}",
booktitle = {Astronomical Data Analysis Software and Systems XVIII},
   series = asp,
     year = 2009,
   volume = 411,
   editor = {{Bohlender}, D. A. and {Durand}, D. and {Dowler}, P.},
    pages = {251-254}
}

@INPROCEEDINGS{Martin2004,
   author = {{Martin}, H. M. and {Burge}, J. H. and {Cuerden}, B. and
            {Miller}, S. M. and {Smith}, B. and {Zhao}, C.},
    title = "{Manufacture of 8.4-m Off-Axis Segments. A 1/5-Scale
            Demonstration}",
booktitle = {Optical Fabrication, Metrology, and Material Advancements for
            Telescopes},
   series = posp,
     year = 2004,
   volume = 5494,
   editor = {{Atad-Ettedgui}, E. and {Dierickx}, P.},
    pages = {62-70}
}

@ARTICLE{Martin1998,
   author = {{Martin}, S. F.},
    title = "{Conditions for the Formation and Maintenance of Filaments}",
  journal = sp,
     year = 1998,
   volume = 182,
    pages = {107-137},
      doi = {10.1023/A:1005026814076}
}

@ARTICLE{Martin1985,
   author = {{Martin}, S. F. and {Livi}, S. H. B. and {Wang}, J.},
    title = "{The Cancellation of Magnetic Flux. II.\ In a Decaying Active
            Region}",
  journal = ajp,
     year = 1985,
   volume = 38,
    pages = {929-959}
}

@ARTICLE{MartinezGonzalez2010,
   author = {{Mart{\'{\i}}nez Gonz{\'a}lez}, M.~J. and {Manso Sainz}, R. and 
	{Asensio Ramos}, A. and {Bellot Rubio}, L.~R.},
    title = "{Small Magnetic Loops Connecting the Quiet Surface and the Hot Outer Atmosphere of the Sun}",
  journal = {apjl},
archivePrefix = "arXiv",
   eprint = {1003.1255},
     year = 2010,
   volume = 714,
    pages = {L94-L97},
      doi = {10.1088/2041-8205/714/1/L94}
}

@ARTICLE{MartinezOliveros2011,
   author = {{Mart{\'{\i}}nez Oliveros}, J. C. and {Couvidat}, S. and
            {Schou}, J. and {Krucker}, S. and {Lindsey}, C. and
            {Hudson}, H. S. and {Scherrer}, P.},
    title = "{Imaging Spectroscopy of a White-Light Solar Flare}",
  journal = sp,
     year = 2011,
   volume = 269,
    pages = {269-281}
}

@ARTICLE{MartinezPillet2009,
   author = {{Mart{\'{\i}}nez Pillet}, V. and {Katsukawa}, Y. and
            {Puschmann}, K. G. and {Ruiz Cobo}, B.},
    title = "{Supersonic Continuation of the Evershed Flow Outside a Sunspot as
            Observed with Hinode}",
  journal = apjl,
     year = 2009,
   volume = 701,
    pages = {L79-L82}
}

@ARTICLE{MartinezPillet2002,
   author = {{Mart{\'{\i}}nez Pillet}, V.},
    title = "{Decay of Sunspots}",
  journal = an,
     year = 2002,
   volume = 323,
    pages = {342-348}
}

@ARTICLE{MartinezPillet1993,
   author = {{Mart{\'{\i}}nez Pillet}, V. and {Moreno-Insertis}, F. and {Vazquez}, M.},
    title = "{The Distribution of Sunspot Decay Rates}",
  journal = aa,
     year = 1993,
   volume = 274,
    pages = {521-533}
}

@ARTICLE{Mathew2009,
   author = {{Mathew}, S. K. and {Zakharov}, V. and {Solanki}, S. K.},
    title = "{Stray Light Correction and Contrast Analysis of Hinode Broad-Band
            Images}",
  journal = aa,
     year = 2009,
   volume = 501,
    pages = {L19-L22}
}

@ARTICLE{Maurya2011,
   author = {{Maurya}, R. A. and {Reddy}, V. and {Ambastha}, A.},
    title = "{Velocity and Magnetic Transients Driven by the X2.2 White-Light
            Flare of 2011 February 15 in NOAA 11158}",
  journal = {ArXiv e-prints},
   pages = {1106.4166},
     year = 2011
}

@ARTICLE{McIntosh1990,
   author = {{McIntosh}, P. S.},
    title = "{The Classification of Sunspot Groups}",
  journal = sp,
     year = 1990,
   volume = 125,
    pages = {251-267}
}

@INPROCEEDINGS{McIntosh1981,
   author = {{McIntosh}, P. S.},
    title = "{The Birth and Evolution of Sunspots - Observations}",
booktitle = {The Physics of Sunspots},
     year = 1981,
   editor = "{L. E. Cram \& J. H. Thomas}",
    pages = {7-54}
}

@ARTICLE{Mein2000,
   author = {{Mein}, P. and {Briand}, C. and {Heinzel}, P. and
            {Mein}, N.},
    title = "{Solar Arch Filaments Observed with THEMIS}",
  journal = aa,
     year = 2000,
   volume = 355,
    pages = {1146-1151}
}

@ARTICLE{Mein1996,
   author = {{Mein}, N. and {Mein}, P. and {Heinzel}, P. and {Vial}, {J.-C.} and
            {Malherbe}, J. M. and {Staiger}, J.},
    title = "{Cloud Model With Variable Source Function for Solar H$\alpha$
            Structures.}",
  journal = aa,
     year = 1996,
   volume = 309,
    pages = {275-283}
}

@ARTICLE{Mein1988,
   author = {{Mein}, P. and {Mein}, N.},
    title = "{Differential Cloud Models for Solar Velocity Field Measurements}",
  journal = aa,
     year = 1988,
   volume = 203,
    pages = {162-169}
}

@ARTICLE{MolownyHoras1999,
   author = {{Molowny-Horas}, R. and {Heinzel}, P. and {Mein}, P. and
            {Mein}, N.},
    title = "{A Non-LTE Inversion Procedure for Chromospheric Cloud-Like
            Features}",
  journal = aa,
     year = 1999,
   volume = 345,
    pages = {618-628}
}

@ARTICLE{MolownyHoras1994a,
   author = {{Molowny-Horas}, R.},
    title = "{Modelling of Geometric Transformations of Solar Images}",
  journal = aas,
     year = 1994,
   volume = 107,
    pages = {121-127}
}

@ARTICLE{MolownyHoras1994b,
   author = {{Molowny-Horas}, R.},
    title = "{Proper Motion Measurements of Umbral and Penumbral Structure}",
  journal = sp,
     year = 1994,
   volume = 154,
    pages = {29-39}
}

@PHDTHESIS{MolownyHoras1994c,
   author = {{Molowny-Horas}, R.},
    title = "{Dynamics and Structure of the Solar Chromosphere}",
   school = {University of Oslo},
     year = 1994
}

@ARTICLE{Montesinos1997,
   author = {{Montesinos}, B. and {Thomas}, J. H.},
    title = "{The Evershed Effect in Sunspots as a Siphon Flow along a Magnetic
            Flux Tube}",
  journal = nat,
     year = 1997,
   volume = 390,
    pages = {485-487}
}

@ARTICLE{Moore1965,
   author = {{Moore}, G. E.},
    title = "{Cramming More Components on Integrated Circuits}",
  journal = elec,
     year = 1965,
   volume = 38
}

@ARTICLE{Moore2001,
   author = {{Moore}, R. L. and {Sterling}, A. C. and {Hudson}, H. S. and
            {Lemen}, J. R.},
    title = "{Onset of the Magnetic Explosion in Solar Flares and Coronal Mass
            Ejections}",
  journal = apj,
     year = 2001,
   volume = 552,
    pages = {833-848},
      doi = {10.1086/320559}
}

@ARTICLE{Moore1977,
   author = {{Moore}, R. L. and {Tang}, F. and {Bohlin}, J. D. and
            {Golub}, L.},
    title = "{H$\alpha$ Macrospicules -- Identification with EUV Macrospicules
            and with Flares in X-Ray Bright Points}",
  journal = apj,
     year = 1977,
   volume = 218,
    pages = {286-290}
}

@INCOLLECTION{More1977,
   author = {{Mor{\'e}}, J. J.},
    title = "{The Levenberg-Marquardt Algorithm: Implementation and Theory}",
booktitle = "{Numerical Analysis,}",
   series = "{Lecture Notes in Mathematics}",
     year = 1977,
publisher = "Springer-Verlag",
  address = "Berlin",
   editor = {{Watson}, G. A.},
   volume = 630,
    pages = {105-116}
}

@BOOK{More1993,
   author = {{Mor{\'e}}, J. J. and {Wright}, S. J.},
    title = "{Optimization Software Guide}",
   series = "{Frontiers in Applied Mathematics}",
publisher = "Society for Industrial and Applied Mathematics (SIAM)",
     year = 1993,
  address = {Philadelphia},
   volume = 14
}

@ARTICLE{MorenoInsertis1988,
   author = {{Moreno-Insertis}, F. and {Vazquez}, M.},
    title = "{A Statistical Study of the Decay Phase of Sunspot Groups from 1874 to 1939}",
  journal = aa,
     year = 1988,
   volume = 205,
    pages = {289-296}
}

@ARTICLE{Moreton1960,
   author = {{Moreton}, G. E. and {Ramsey}, H. E.},
    title = "{Recent Observations of Dynamical Phenomena Associated with Solar
            Flares}",
  journal = pasp,
     year = 1960,
   volume = 72,
    pages = {357-358},
      doi = {10.1086/127549}
}

@ARTICLE{Morimoto2003,
   author = {{Morimoto}, T. and {Kurokawa}, H.},
    title = "{A Method for the Determination of 3-D Velocity Fields of
            Disappearing Solar Filaments}",
  journal = pasj,
     year = 2003,
   volume = 55,
    pages = {505-520}
}

@INPROCEEDINGS{Muglach1998,
   author = {{Muglach}, K. and {S{\"u}tterlin}, P.},
    title = "{Simultaneous Observations with the GCT and SoHO: High Velocity Events in the Upper 
Chromosphere}",
booktitle = {Three-Dimensional Structure of Solar Active Regions},
     year = 1998,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 155,
   editor = {{Alissandrakis}, C.~E. and {Schmieder}, B.},
    pages = {341}
}

@ARTICLE{Muglach1997,
   author = {{Muglach}, K. and {Schmidt}, W. and {Knoelker}, M.},
    title = "{Multiple velocities observed in HeI 1083 NM}",
  journal = sp,
     year = 1997,
   volume = 172,
    pages = {103-108},
      doi = {10.1023/A:1004988205716}
}

@ARTICLE{Muller1973,
   author = {{Muller}, R.},
    title = "{{\'E}tude Morphologique et Cin{\'e}matique des Structures Fines
            d'une Tache Solaire}",
  journal = sp,
     year = 1973,
   volume = 29,
    pages = {55-73}
}



%====     NNNN    ==============================================================

@ARTICLE{Naqvi2010,
   author = {{Naqvi}, M. F. and {Marquette}, W. H. and {Tritschler}, A. and
            {Denker}, C.},
    title = "{Tge Big Bear Solar Observatory Ca\,\textsc{ii}\,K-Line Index
            for Solar Cycle 23}",
  journal = an,
     year = 2010,
   volume = 331,
    pages = {696-703}
}

@ARTICLE{Neckel1984,
   author = {{Neckel}, H. and {Labs}, D.},
    title = "{The solar radiation between 3300 and 12500 A}",
  journal = sp,
     year = 1984,
   volume = 90,
    pages = {205-258},
      doi = {10.1007/BF00173953}
}

@ARTICLE{Nielsen2011,
   author = {{Nielsen}, M. L. and {Kjeldsen}, H.},
    title = "{Is Cycle 24 the Beginning of a Dalton-Like Minimum?}",
  journal = sp,
     year = 2011,
   volume = 270,
    pages = {385-392}
}

@INPROCEEDINGS{November1989,
   author = {{November}, L. J.},
    title = "{Proper Motion Measurements of Solar Granulation: The Case for
            Mesogranulation}",
booktitle = {High Spatial Resolution Solar Observations},
     year = 1989,
   series = "Proc. $10^{\mathrm{th}}$ Sacramento Peak Summer Workshop",
   editor = {{von der L\"uhe}, O.},
    pages = {457}
}

@ARTICLE{November1988,
   author = {{November}, L. J. and {Simon}, G. W.},
    title = "{Precise Proper-Motion Measurement of Solar Granulation}",
  journal = apj,
     year = 1988,
   volume = 333,
    pages = {427-442},
      doi = {10.1086/166758}
}



%====     OOOO    ==============================================================

@ARTICLE{OrozcoSuarez2012,
   author = {{Orozco Su{\'a}rez}, D. and {Katsukawa}, Y. and {Bellot Rubio}, L.~R.
	},
    title = "{The Connection between Internetwork Magnetic Elements and Supergranular Flows}",
  journal = apjl,
     year = 2012,
   volume = 758,
      eid = {L38},
    pages = {L38},
      doi = {10.1088/2041-8205/758/2/L38},
}

@ARTICLE{OrozcoSuarez2007,
   author = {{Orozco Su{\'a}rez}, D. and {Bellot Rubio}, L. R. and
            {del Toro Iniesta}, J. C.},
    title = "{Quiet-Sun Magnetic Fields from Space-Borne Observations:
            Simulating Hinode's Case}",
  journal = apjl,
     year = 2007,
   volume = 662,
    pages = {L31-L34}
}

@ARTICLE{Ortiz2010,
   author = {{Ortiz}, A. and {Bellot Rubio}, L. R. and
            {Rouppe van der Voort}, L.},
    title = "{Downflows in Sunspot Umbral Dots}",
  journal = apj,
     year = 2010,
   volume = 713,
    pages = {1282-1291}
}



%====     PPPP    ==============================================================

@ARTICLE{Pence2009,
   author = {{Pence}, W. D. and {Seaman}, R. and {White}, R. L.},
    title = "{Lossless Astronomical Image Compression and the Effects of Noise}",
  journal = pasp,
     year = 2009,
   volume = 121,
    pages = {414-427}
}

@ARTICLE{Penn1995,
   author = {{Penn}, M.~J. and {Kuhn}, J.~R.},
    title = "{Imaging spectropolarimetry of the He I 1083 nanometer line in a flaring solar active 
region}",
  journal = apjl,
 keywords = {Chromosphere, Circular Polarization, Coronal Holes, Helium, Infrared Astronomy, Line 
Spectra, Linear Polarization, Photosphere, Solar Flares, Solar Magnetic Field, Astronomical Spectroscopy, 
Cameras, Charge Coupled Devices, Field Of View, Infrared Photography, Magnetic Signatures, Red Shift, 
Spectroheliographs, Spectroscopic Telescopes},
     year = 1995,
   volume = 441,
    pages = {L51-L54},
      doi = {10.1086/187787}
}

@ARTICLE{Perona1990,
   author = {{Perona}, P. and {Malik}, J.},
    title = "{Scale-Space and Edge Detection Using Anisotropic Diffusion}",
  journal = {IEEE Trans. Pattern Anal. Mach. Intell.},
     year = 1990,
   volume = 12,
    pages = {629-639},
      doi = {10.1109/34.56205}
}

@ARTICLE{Pesnell2012,
   author = {{Pesnell}, W. D. and {Thompson}, B. J. and {Chamberlin}, P. C.},
    title = "{The Solar Dynamics Observatory (SDO)}",
  journal = sp,
     year = 2012,
   volume = 275,
    pages = {3-15}
}

@ARTICLE{Peter1996,
   author = {{Peter}, H.},
    title = "{Superpenumbral Vortices}",
  journal = mn,
     year = 1996,
   volume = 278,
    pages = {821-828}
}

@ARTICLE{Petrie2012,
   author = {{Petrie}, G. J. D.},
    title = "{Evolution of Active and Polar Photospheric Magnetic Fields During
            the Rise of Cycle 24 Compared to Previous Cycles}",
  journal = sp,
     year = 2012,
   volume = 281,
    pages = {577-598}
}

@ARTICLE{Petrovay2010,
   author = {{Petrovay}, K.},
    title = "{Solar Cycle Prediction}",
  journal = {Living Rev. Sol. Phys.},
     year = 2010,
   volume = 7,
    pages = {6}
}

@ARTICLE{Petrovay1999,
   author = {{Petrovay}, K. and {Mart{\'{\i}}nez Pillet}, V. and
            {van Driel-Gesztelyi}, L.},
    title = "{Making Sense of Sunspot Decay. II. Deviations from the Mean Law
            and Plage Effects}",
  journal = sp,
     year = 1999,
   volume = 188,
    pages = {315-330}
}

@ARTICLE{Petrovay1997,
   author = {{Petrovay}, K. and {van Driel-Gesztelyi}, L.},
    title = "{Making Sense of Sunspot Decay. I. Parabolic Decay Law and
             Gnevyshev-Waldmeier Relation}",
  journal = sp,
     year = 1997,
   volume = 176,
    pages = {249-266}
}

@ARTICLE{Pevtsov2002,
   author = {{Pevtsov}, A. A.},
    title = "{Active-Region Filaments and X-Ray Sigmoids}",
  journal = sp,
     year = 2002,
   volume = 207,
    pages = {111-123}
}

@ARTICLE{Pierce1977b,
   author = {{Pierce}, A. K. and {Slaughter}, C. D.},
    title = "{Solar Limb Darkening. I. $\lambda\lambda$(3033--7297)}",
  journal = sp,
     year = 1977,
   volume = 51,
    pages = {25-41}
}


@ARTICLE{Pierce1977a,
   author = {{Pierce}, A. K. and {Slaughter}, C. D. and {Weinberger}, D.},
    title = "{Solar Limb Darkening in the Interval 7404--24018\AA, II}",
  journal = sp,
     year = 1977,
   volume = 52,
    pages = {179-189}
}
@ARTICLE{Ponz1994,
   author = {{Ponz}, J. D. and {Thompson}, R. W. and {Munoz}, J. R.},
    title = "{The FITS Image Extension}",
  journal = aas,
     year = 1994,
   volume = 105,
    pages = {53-55}
}

@ARTICLE{Potts2010,
   author = {{Potts}, H. and {Hudson}, H. and {Fletcher}, L. and {Diver}, D.},
    title = "{The Optical Depth of White-light Flare Continuum}",
  journal = apj,
     year = 2010,
   volume = 722,
    pages = {1514-1521},
      doi = {10.1088/0004-637X/722/2/1514}
}

@ARTICLE{Potts2008,
   author = {{Potts}, H. E. and {Diver}, D. A.},
    title = "{Automatic Recognition and Characterisation of Supergranular Cells
            from Photospheric Velocity Fields}",
  journal = sp,
     year = 2008,
   volume = 248,
    pages = {263-275}
}

@ARTICLE{Potts2004,
   author = {{Potts}, H. E. and {Barrett}, R. K. and {Diver}, D. A.},
    title = "{Balltracking: An Highly Efficient Method for Tracking Flow
            Fields}",
  journal = aa,
     year = 2004,
   volume = 424,
    pages = {253-262}
}

@ARTICLE{Potts2003,
   author = {{Potts}, H. E. and {Barrett}, R. K. and {Diver}, D. A.},
    title = "{Reduction of Interpolation Errors when Using Local Correlation
            Tracking for Motion Detection}",
  journal = sp,
     year = 2003,
   volume = 217,
    pages = {69-78}
}

@BOOK{Press1992,
   author = {{Press}, W. H. and {Teukolsky}, S. A. and {Vetterling}, W. T. and
            {Flannery}, B. P.},
    title = "{Numerical Recipes in C. The Art of Scientific Computing}",
publisher = {Cambridge University Press},
     year = 1992,
  address = {New York}
}

@ARTICLE{Puschmann2013,
   author = {{Puschmann}, K. G. and {Denker}, C. and {Balthasar}, H. and
            {Louis}, R. E. and {Popow}, E. and {Woche}, M. and {Beck}, C. and 
            {Seelemann}, T. and {Volkmer}, R.},
    title = "{GREGOR Fabry-P{\'e}rot Interferometer and its Companion the Blue
            Imaging Solar Spectrometer}",
  journal = oe,
     year = 2013,
   volume = 52,
   number = 8,
      eid = {081606},
    pages = {081606},
      doi = {10.1117/1.OE.52.8.081606}
}

@ARTICLE{Puschmann2012,
   author = {{Puschmann}, K. G. and {Denker}, C. and {Kneer}, F. and
            {Al Erdogan}, N. and {Balthasar}, H. and {Bauer}, S. M. and
            {Beck}, C. and {Bello Gonz{\'a}lez}, N. and {Collados}, M. and
            {Hahn}, T. and {Hirzberger}, J. and {Hofmann}, A. and
            {Louis}, R. E. and {Nicklas}, H. and {Okunev}, O. and
            {Mart{\'{\i}}nez Pillet}, V. and {Popow}, E. and {Seelemann}, T. and
            {Volkmer}, R. and {Wittmann}, A. D. and {Woche}, M.},
    title = "{The GREGOR Fabry-P{\'e}rot Interferometer}",
  journal = an,
     year = 2012,
   volume = 333,
    pages = {880},
      doi = {10.1002/asna.201211734}
}

@ARTICLE{Puschmann2011,
   author = {{Puschmann}, K. G. and {Beck}, C.},
    title = "{Application of Speckle and (Multi-Object) Multi-Frame Blind
            Deconvolution Techniques on Imaging and Imaging Spectropolarimetric
            Data}",
  journal = aa,
     year = 2011,
   volume = 533,
    pages = {A21},
      doi = {10.1051/0004-6361/201116904}
}

@INPROCEEDINGS{Puschmann2007,
   author = {{Puschmann}, K. G. and {Kneer}, F. and {Nicklas}, H. and
            {Wittmann}, A. D},
    title = "{From the G{\"o}ttingen Fabry-P{\'e}rot Interferometer to the
            GREGOR FPI}",
booktitle = {Modern Solar Facilities -- Advanced Solar Science},
     year = 2007,
   editor = {{Kneer}, F. and {Puschmann}, K. G. and {Wittmann}, A. D.},
    pages = {45-50}
}

@ARTICLE{Puschmann2006,
   author = {{Puschmann}, K. G. and {Kneer}, F. and {Seelemann}, T. and
            {Wittmann}, A. D.},
    title = "{The New G{\"o}ttingen Fabry-P{\'e}rot Spectrometer for
            Two-Dimensional Observations of the Sun}",
  journal = aa,
     year = 2006,
   volume = 451,
    pages = {1151-1158},
      doi = {10.1051/0004-6361:20054487}
}

@ARTICLE{Pulkkinen2007,
  title    = {Space Weather: Terrestrial Perspective},
  author   = {{Pulkkinen}, T.},
  journal  = lrsp,
  year     = {2007},
  number   = {1},
  volume   = {4},
  url      = {http://www.livingreviews.org/lrsp-2007-1}
}



%====     QQQQ    ==============================================================

@ARTICLE{Qiu2001,
   author = {{Qiu}, J. and {Ding}, M. D. and {Wang}, H. and 
            {Gallagher}, P. T. and {Sato}, J. and {Denker}, C. and
            {Goode}, P. R.},
    title = "{Asymmetric Behavior of H$\alpha$ Footpoint Emission during the
            Early Phase of an Impulsive Flare}",
  journal = apj,
     year = 2001,
   volume = 554,
    pages = {445-450}
}

@ARTICLE{Qiu2000,
   author = {{Qiu}, J. and {Ding}, M. D. and {Wang}, H. and {Denker}, C. and
            {Goode}, P. R.},
    title = "{Ultraviolet and H$\alpha$ Emission in Ellerman Bombs}",
  journal = apjl,
     year = 2000,
   volume = 544,
    pages = {157-161}
}



%====     RRRR    ==============================================================

@ARTICLE{Rast1995,
   author = {{Rast}, M. P.},
    title = "{On the Nature of 'Exploding' Granules and Granule Fragmentation}",
  journal = apj,
     year = 1995,
   volume = 443,
    pages = {863-868}
}

@ARTICLE{Rees2000,
   author = {{Rees}, D. E. and {L{\'o}pez Ariste}, A. and {Thatcher}, J. and
            {Semel}, M.},
    title = "{Fast Inversion of Spectral Lines Using Principal Component
            Analysis. I.\ Fundamentals}",
  journal = aa,
     year = 2000,
   volume = 355,
    pages = {759-768}
}

@ARTICLE{Rempel2011b,
   author = {{Rempel}, M. and {Schlichenmaier}, R.},
    title = "{Sunspot Modeling: From Simplified Models to Radiative MHD
            Simulations}",
  journal = {Liv.\ Rev.\ Sol.\ Phys.},
     year = 2011,
   volume = 8,
    pages = {3},
      doi = {10.12942/lrsp-2011-3}
}

@ARTICLE{Rempel2011c,
   author = {{Rempel}, M.},
    title = "{Subsurface Magnetic Field and Flow Structure of Simulated
            Sunspots}",
  journal = apj,
     year = 2011,
   volume = 740,
    pages = {15}
}

@ARTICLE{Rempel2009a,
   author = {{Rempel}, M. and {Sch{\"u}ssler}, M. and {Cameron}, R. H. and
            {Kn{\"o}lker}, M.},
    title = "{Penumbral Structure and Outflows in Simulated Sunspots}",
  journal = sc,
     year = 2009,
   volume = 325,
    pages = {171-174}
}

@ARTICLE{Rempel2009b,
   author = {{Rempel}, M. and {Sch{\"u}ssler}, M. and {Kn{\"o}lker}, M.},
    title = "{Radiative Magnetohydrodynamic Simulation of Sunspot Structure}",
  journal = apj,
     year = 2009,
   volume = 691,
    pages = {640-649}
}

@TECHREPORT{Renka1982,
     author = {{Renka}, R.},
      title = "{Interpolation of Data on the Surface of a Sphere}",
     number = {ORNL/CSD-108},
institution = {Oak Ridge National Laboratory},
       year = 1982,
}

@ARTICLE{Rezaei2012,
   author = {{Rezaei}, R. and {Bello Gonz{\'a}lez}, N. and {Schlichenmaier}, R.
	},
    title = "{The formation of sunspot penumbra. Magnetic field properties}",
  journal = aa,
archivePrefix = "arXiv",
   eprint = {1111.3189},
     year = 2012,
   volume = 537,
      eid = {A19},
    pages = {A19},
      doi = {10.1051/0004-6361/201117485}
}

@ARTICLE{Rezaei2007,
   author = {{Rezaei}, R. and {Schlichenmaier}, R. and {Schmidt}, W. and
            {Steiner}, O.},
    title = "{Opposite Magnetic Polarity of Two Photospheric Lines in Single
            Spectrum of the Quiet Sun}",
  journal = aa,
     year = 2007,
   volume = 469,
    pages = {L9-L12}
}

@ARTICLE{Rezaei2006,
   author = {{Rezaei}, R. and {Schlichenmaier}, R. and {Beck}, C. and
            {Bellot Rubio}, L. R.},
    title = "{The Flow Field in the Sunspot Canopy}",
  journal = aa,
     year = 2006,
   volume = 454,
    pages = {975-982}
}

@ARTICLE{Rieutord2010,
   author = {{Rieutord}, M. and {Roudier}, T. and {Rincon}, F. and
            {Malherbe}, J.-M. and {Meunier}, N. and {Berger}, T. and
            {Frank}, Z.},
    title = "{On the Power Spectrum of Solar Surface Flows}",
  journal = aa,
     year = 2010,
   volume = 512,
    pages = {A4},
      doi = {10.1051/0004-6361/200913303},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Rimmele2010,
   author = {{Rimmele}, T. R. and {Wagner}, J. and {Keil}, S. and 
            {Elmore}, D. and {Hubbard}, R. and {Hansen}, E. and {Warner}, M. and
            {Jeffers}, P. and {Phelps}, L. and {Marshall}, H. and
            {Goodrich}, B. and {Richards}, K. and {Hegwer}, S. and 
            {Kneale}, R. and {Ditsler}, J.},
    title = "{The Advanced Technology Solar Telescope: Beginning Construction of
            the World's Largest Solar Telescope}",
booktitle = {Ground-Based and Airborne Telescopes III},
     year = 2010,
   series = posp,
   volume = 7733,
   editor = {{Stepp}, L. M. and {Gilmozzi}, R. and {Hall}, H. J.},
    pages = {77330G}
}

@ARTICLE{Rimmele2006,
   author = {{Rimmele}, T. R. and {Marino}, J.},
    title = "{The Evershed Flow. Flow Geometry and its Temporal Evolution}",
  journal = apj,
     year = 2006,
   volume = 646,
    pages = {593-604}
}

@INPROCEEDINGS{Rimmele2005,
   author = {{Rimmele}, T. R. and {Keil}, S. and {Wagner}, J. and {Dalrymple},
            N. and {Goodrich}, B. and {Hansen}, E. and {Hill}, F. and {Hubbard},
            R. and {Phelps}, L. and {Richards}, K. and {Warner}, M.},
    title = "{Advanced Technology Solar Telescope. A Progress Report}",
booktitle = {Solar Physics and Space Weather Instrumentation},
     year = 2005,
   series = posp,
   volume = 5901,
   editor = {{Fineschi}, S. and {Viereck}, R. A.},
    pages = {41-51}
}

@INPROCEEDINGS{Rimmele2004,
   author = {{Rimmele}, T. R. and {Richards}, K. and {Hegwer}, S. and
            {Fletcher}, S. and {Gregory}, S. and {Moretto}, G. and
            {Didkovsky}, L. V. and {Denker}, C. and {Dolgushin}, A. and
            {Goode}, P. R. and {Langlois}, M. and {Marino}, J. and
            {Marquette}, W.},
    title = "{First Results from the NSO/NJIT Solar Adaptive Optics System}",
booktitle = {Telescopes and Instrumentation for Solar Astrophysics},
   series = posp,
     year = 2004,
   volume = 5171,
   editor = {{Fineschi}, S. and {Gummin}, M. A.},
    pages = {179-186}
}

@INPROCEEDINGS{Rimmele2003,
   author = {{Rimmele}, T. R. and {Richards}, K. and {Hegwer}, S. L. and
            {Ren}, D. and {Fletcher}, S. and {Gregory}, S. and
            {Didkovsky}, L. V. and {Denker}, C. and {Marquette}, W. and
            {Marino}, J. and {Goode}, P. R.},
    title = "{Solar Adaptive Optics: A Progress Report}",
booktitle = {Adaptive Optical System Technologies II},
     year = 2003,
   series = posp,
   volume = 4839,
   editor = {{Wizinowich}, P. L. and {Bonaccini}, D.},
    pages = {635-646}
}

@INPROCEEDINGS{Rimmele2000,
   author = {{Rimmele}, T. R.},
    title = "{Solar Adaptive Optics}",
booktitle = {Adaptive Optical Systems Technology},
     year = 2000,
   series = posp,
   volume = 4007,
   editor = {{Wizinowich}, P. L.},
    pages = {218-231}
}

@ARTICLE{Rimmele1995,
   author = {{Rimmele}, T. R.},
    title = "{Sun Center Observations of the Evershed Effect}",
  journal = apj,
     year = 1995,
   volume = 445,
    pages = {511-516}
}

@ARTICLE{Roudier2002,
   author = {{Roudier}, T. and {Bonet}, J. A. and {Sobotka}, M.},
    title = "{Properties of Horizontal Flows Inside and Outside a Solar Pore}",
  journal = aa,
     year = 2002,
   volume = 395,
    pages = {249-255}
}

@ARTICLE{RouppevanderVoort2010,
   author = {{Rouppe van der Voort}, L. and {Bellot Rubio}, L. R. and
            {Ortiz}, A.},
    title = "{Upflows in the Central Dark Lane of Sunspot Light Bridges}",
  journal = apjl,
     year = 2010,
   volume = 718,
    pages = {L78-L82}
}

@INPROCEEDINGS{RouppevanderVoort2006,
   author = {{Rouppe van der Voort}, L. and {van Noort}, M. and
            {Carlsson}, M. and {Hansteen}, V.},
    title = "{High Spatial Resolution Observations of Solar Magnetic Structures}",
booktitle = {Solar MHD Theory and Observations: A High Spatial Resolution Perspective},
     year = 2006,
   series = asp,
   volume = 354,
   editor = {{Leibacher}, J. and {Stein}, R. F. and {Uitenbroek}, H.},
    pages = {37-42}
}


@ARTICLE{RouppevanderVoort2005,
   author = {{Rouppe van der Voort}, L. H. M. and {Hansteen}, V. H. and
            {Carlsson}, M. and {Fossum}, A. and {Marthinussen}, E. and
            {van Noort}, M. J. and {Berger}, T. E.},
    title = "{Solar Magnetic Elements at $0{\farcs}1$ Resolution.
            II.\ Dynamical Evolution}",
  journal = aa,
     year = 2005,
   volume = 435,
    pages = {327-337},
      doi = {10.1051/0004-6361:20042561}
}

@ARTICLE{RouppevanderVoort2004,
   author = {{Rouppe van der Voort}, L. H. M. and {L{\"o}fdahl}, M. G. and
            {Kiselman}, D. and {Scharmer}, G. B.},
    title = "{Penumbral Structure at 0.1 arcsec Resolution. I. General
            Appearance and Power Spectra}",
  journal = aa,
     year = 2004,
   volume = 414,
    pages = {717-726}
}

@ARTICLE{Rucklidge1995,
   author = {{Rucklidge}, A. M. and {Schmidt}, H. U. and {Weiss}, N. O.},
    title = "{The Abrupt Development of Penumbrae in Sunspots}",
  journal = mn,
     year = 1995,
   volume = 273,
    pages = {491-498}
}

@ARTICLE{RuizCobo2008,
   author = {{Ruiz Cobo}, B. and {Bellot Rubio}, L. R.},
    title = "{Heat Transfer in Sunspot Penumbrae. Origin of Dark-Cored Penumbral
            Filaments}",
  journal = aa,
     year = 2008,
   volume = 488,
    pages = {749-756}
}

@ARTICLE{RuizCobo1992,
   author = {{Ruiz Cobo}, B. and {del Toro Iniesta}, J. C.},
    title = "{Inversion of Stokes Profiles}",
  journal = apj,
     year = 1992,
   volume = 398,
    pages = {375-385}
}

@BOOK{Russ2011,
   author = {{Russ}, J. C.},
    title = "{The Image Processing Handbook}",
publisher = "CRC Press",
  address = "Boca Raton, Florida",
     year = 2011
}

@INPROCEEDINGS{Rutten2007,
   author = {{Rutten}, R. J.},
    title = "{Observing the Solar Chromosphere}",
booktitle = {The Physics of Chromospheric Plasmas},
     year = 2007,
   series = asp,
   volume = 368,
   editor = {{Heinzel}, P. and {Dorotovi{\v c}}, I. and {Rutten}, R. J.},
    pages = {27-48}
}

@ARTICLE{Rutten2004a,
   author = {{Rutten}, R. J. and {de Wijn}, A. G. and
            {S{\"u}tterlin}, P.},
   title  = "{DOT Tomography of the Solar Atmosphere. II.
            Reversed Granulation in Ca II H}",
  journal = aa,
     year = 2004,
   volume = 416,
    pages = {333-340}
}

@INPROCEEDINGS{Rutten2004b,
   author = {{Rutten}, R. J. and {Bettonvil}, F. C. M. and
            {Hammerschlag}, R. H. and {J{\"a}gers}, A. P. L. and
            {Leenaarts}, J. and {Snik}, F. and {S{\"u}tterlin}, P. and
            {Tziotziou}, K. and {de Wijn}, A. G.},
    title = "{The Dutch Open Telescope on La Palma}",
booktitle = {Multi-Wavelength Investigations of Solar Activity},
     year = 2004,
   series = iaus,
   volume = 223,
   editor = {{Stepanov}, A. V. and {Benevolenskaya}, E. E. and
            {Kosovichev}, A. G.},
    pages = {597-604}
}

@ARTICLE{Ryutova2008,
   author = {{Ryutova}, M. and {Berger}, T. and {Title}, A.},
    title = "{On the Fine Structure and Formation of Sunspot Penumbrae}",
  journal = apj,
     year = 2008,
   volume = 676,
    pages = {1356-1366}
}



%====     SSSS    ==============================================================

@ARTICLE{SainzDalda2012,
   author = {{Sainz Dalda}, A. and {Vargas Dom{\'{\i}}nguez}, S. and
            {Tarbell}, T. D.},
    title = "{Magnetic Topology of a Naked Sunspot: Is it Really Naked?}",
  journal = apjl,
     year = 2012,
   volume = 746,
      eid = {L13},
    pages = {L13},
      doi = {10.1088/2041-8205/746/1/L13}
}

@ARTICLE{SainzDalda2008,
   author = {{Sainz Dalda}, A. and {Bellot Rubio}, L. R.},
    title = "{Detection of Sea-Serpent Field Lines in Sunspot Penumbrae}",
  journal = aa,
     year = 2008,
   volume = 481,
    pages = {L21-L24}
}

@ARTICLE{SainzDalda2005,
   author = {{Sainz Dalda}, A. and {Mart{\'{\i}}nez Pillet}, V.},
    title = "{Moving Magnetic Features as Prolongation of Penumbral Filaments}",
  journal = apj,
     year = 2005,
   volume = 632,
    pages = {1176-1183}
}

@ARTICLE{SanchezAlmeida2001,
   author = {{S{\'a}nchez Almeida}, J. and {Asensio Ramos}, A. and
            {Trujillo Bueno}, J. and {Cernicharo}, J.},
    title = "{G-Band Spectral Synthesis in Solar Magnetic Concentrations}",
  journal = apj,
     year = 2001,
   volume = 555,
    pages = {978-989}
}

@ARTICLE{SanchezCuberes2005,
   author = {{S{\'a}nchez Cuberes}, M. and {Puschmann}, K. G. and
            {Wiehr}, E.},
    title = "{Spectropolarimetry of a Sunspot at Disk Centre}",
  journal = aa,
     year = 2005,
   volume = 440,
    pages = {345-356},
      doi = {10.1051/0004-6361:20042042}
}

@ARTICLE{Sankarasubramanian2003,
   author = {{Sankarasubramanian}, K. and {Rimmele}, T.},
    title = "{Properties of Magnetic and Velocity Fields in and Around Solar Pores}",
  journal = apj,
     year = 2003,
    volume = 598,
    pages = {689-699}
}

@ARTICLE{Sarazin1990,
   author = {{Sarazin}, M. and {Roddier}, F.},
    title = "{The ESO Differential Image Motion Monitor}",
  journal = aa,
     year = 1990,
   volume = 227,
    pages = {294-300}
}
@ARTICLE{Sasso2011,
   author = {{Sasso}, C. and {Lagg}, A. and {Solanki}, S.~K.},
    title = "{Multicomponent He I 10 830 {\AA} profiles in an active filament}",
  journal = aa,
archivePrefix = "arXiv",
   eprint = {1101.5563},
 primaryClass = "astro-ph.SR",
 keywords = {Sun: chromosphere, magnetic fields, Sun: infrared},
     year = 2011,
   volume = 526,
      eid = {A42},
    pages = {A42},
      doi = {10.1051/0004-6361/200912956},
}

@INPROCEEDINGS{Sasso2007,
   author = {{Sasso}, C. and {Lagg}, A. and {Solanki}, S.~K. and {Aznar Cuadrado}, R. and 
	{Collados}, M.},
    title = "{Full-Stokes Observations and Analysis of He I 10830 {\AA} in a Flaring Region}",
booktitle = {The Physics of Chromospheric Plasmas},
     year = 2007,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 368,
   editor = {{Heinzel}, P. and {Dorotovi{\v c}}, I. and {Rutten}, R.~J.},
    month = may,
    pages = {467},
}

@ARTICLE{Scharmer2008a,
   author = {{Scharmer}, G. B. and {Narayan}, G. and {Hillberg}, T. and
            {de la Cruz Rodriguez}, J. and {L{\"o}fdahl}, M. G. and
            {Kiselman}, D. and {S{\"u}tterlin}, P. and {van Noort}, M. and
            {Lagg}, A.},
    title = "{CRISP Spectropolarimetric Imaging of Penumbral Fine Structure}",
  journal = apjl,
     year = 2008,
   volume = 689,
    pages = {L69-L72}
}

@ARTICLE{Scharmer2008b,
   author = {{Scharmer}, G. B. and {Nordlund}, {\AA}. and
            {Heinemann}, T.},
    title = "{Convection and the Origin of Evershed Flows in Sunspot
            Penumbrae}",
  journal = apjl,
     year = 2008,
   volume = 677,
    pages = {L149-L152}
}

@ARTICLE{Scharmer2006a,
   author = {{Scharmer}, G. B. and {Spruit}, H. C.},
    title = "{Magnetostatic Penumbra Models with Field-Free Gaps}",
  journal = aa,
     year = 2006,
   volume = 460,
    pages = {605-615}
}

@ARTICLE{Scharmer2006b,
   author = {{Scharmer}, G. B.},
    title = "{Comments on the Optimization of High resolution Fabry-P{\'e}rot Filtergraphs}",
  journal = aa,
     year = 2006,
   volume = 447,
    pages = {1111-1120}
}

@INPROCEEDINGS{Scharmer2003a,
   author = {{Scharmer}, G.~B. and {Bjelksjo}, K. and {Korhonen}, T.~K. and 
	{Lindberg}, B. and {Petterson}, B.},
    title = "{The 1-meter Swedish solar telescope}",
booktitle = {Innovative Telescopes and Instrumentation for Solar Astrophysics},
     year = 2003,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 4853,
   editor = {{Keil}, S.~L. and {Avakyan}, S.~V.},
    pages = {341-350}
}

@ARTICLE{Scharmer2002,
   author = {{Scharmer}, G. B. and {Gudiksen}, B. V. and {Kiselman}, D. and
            {L{\"o}fdahl}, M. G. and {Rouppe van der Voort}, L. H. M.},
    title = "{Dark Cores in Sunspot Penumbral Filaments}",
  journal = nat,
     year = 2002,
   volume = 420,
    pages = {151-153}
}

@INCOLLECTION{Scharr2007,
   author = {{Scharr}, H.}, 
    title = "{Optimal Filters for Extended Optical Flow}",
booktitle = "{Complex Motion}",
publisher = "{Springer}",
  address = "{Berlin}",
     year = 2007,
   editor = {{J{\"a}hne}, B. and {Mester}, R. and {Barth}, B. and {Scharr}, H.},
   volume = 3417,
   series = "{Lecture Notes in Computer Sciences}",
    pages = {14-29},
      doi = {10.1007/978-540-69866-1{\_}2}
}

@ARTICLE{Scherrer2012,
   author = {{Scherrer}, P. H. and {Schou}, J. and {Bush}, R. I. and
            {Kosovichev}, A. G. and {Bogart}, R. S. and {Hoeksema}, J. T. and
            {Liu}, Y. and {Duvall}, T. L. and {Zhao}, J. and {Title}, A. M. and
            {Schrijver}, C. J. and {Tarbell}, T. D. and {Tomczyk}, S.},
    title = "{The Helioseismic and Magnetic Imager (HMI) Investigation for the
            Solar Dynamics Observatory (SDO)}",
  journal = sp,
     year = 2012,
   volume = 275,
    pages = {207-227}
}

@ARTICLE{Scherrer1995,
   author = {{Scherrer}, P.~H. and {Bogart}, R.~S. and {Bush}, R.~I. and 
	{Hoeksema}, J.~T. and {Kosovichev}, A.~G. and {Schou}, J. and 
	{Rosenberg}, W. and {Springer}, L. and {Tarbell}, T.~D. and 
	{Title}, A. and {Wolfson}, C.~J. and {Zayer}, I. and {MDI Engineering Team}
	},
    title = "{The Solar Oscillations Investigation - Michelson Doppler Imager}",
  journal = {sp},
     year = 1995,
   volume = 162,
    pages = {129-188},
      doi = {10.1007/BF00733429}
}

@ARTICLE{Schlichenmaier2011,
   author = {{Schlichenmaier}, R. and {Rezaei}, R. and {Bello Gonzalez}, N.},
    title = "{On the Formation of Penumbrae as Observed with the German VTT,
            SOHO/MDI, and SDO/HMI}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1102.0965},
     year = 2011
}

@ARTICLE{Schlichenmaier2010a,
   author = {{Schlichenmaier}, R. and {Rezaei}, R. and
            {Bello Gonz{\'a}lez}, N. and {Waldmann}, T. A.},
    title = "{The Formation of a Sunspot Penumbra}",
  journal = aa,
     year = 2010,
   volume = 512,
    pages = {L1-L4}
}

@ARTICLE{Schlichenmaier2010b,
   author = {{Schlichenmaier}, R. and {Bello Gonz{\'a}lez}, N. and
            {Rezaei}, R. and {Waldmann}, T. A.},
    title = "{The Role of Emerging Bipoles in the Formation of a Sunspot
            Penumbra}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1003.1313},
     year = 2010
}

@ARTICLE{Schlichenmaier2002,
   author = {{Schlichenmaier}, R.},
    title = "{Penumbral Fine Structure. Theoretical Understanding}",
  journal = an,
     year = 2002,
   volume = 323,
    pages = {303-308}
}

@ARTICLE{Schlichenmaier1998a,
   author = {{Schlichenmaier}, R. and {Jahn}, K. and {Schmidt}, H. U.},
    title = "{Magnetic Flux Tubes Evolving in Sunspots. A Model for the
            Penumbral Fine Structure and the Evershed Flow}",
  journal = aa,
     year = 1998,
   volume = 337,
    pages = {897-910}
}

@ARTICLE{Schlichenmaier1998b,
   author = {{Schlichenmaier}, R. and {Jahn}, K. and {Schmidt}, H. U.},
    title = "{A Dynamical Model for the Penumbral Fine Structure and the
            Evershed Effect in Sunspots}",
  journal = apjl,
     year = 1998,
   volume = 493,
    pages = {121-124}
}

@INPROCEEDINGS{Schmidt2009,
   author = {{Schmidt}, D. and {Berkefeld}, T. and {Heidecke}, F. and
            {von der L{\"u}he}, O. and {Soltau}, D.},
    title = "{Testbed for the Multi-Conjugate Adaptive Optics System of the
            Solar Telescope GREGOR}",
booktitle = {Astronomical and Space Optical Systems},
     year = 2009,
   series = posp,
   volume = 7439,
   editor = {{Warren}, P. G. and {Marshall}, C. J. and {Tyson}, R. K. and
            {Lloyd-Hart}, M. and {Heaney}, J. B. and {Kvamme}, E. T.},
    pages = {74390X}
}

@ARTICLE{Schmidt2012,
   author = {{Schmidt}, W. and {von der L{\"u}he}, O. and {Volkmer}, R. and 
            {Denker}, C. and {Solanki}, S. K. and {Balthasar}, H. and
            {Bello Gonzalez}, N. and {Berkefeld}, T. and {Collados}, M. and
            {Fischer}, A. and {Halbgewachs}, C. and {Heidecke}, F. and
            {Hofmann}, A. and {Kneer}, F. and {Lagg}, A. and {Nicklas}, H. and
            {Popow}, E. and {Puschmann}, K. G. and {Schmidt}, D. and 
            {Sigwarth}, M. and {Sobotka}, M. and {Soltau}, D. and
            {Staude}, J. and {Strassmeier}, K. G. and {Waldmann }, T. A.},
    title = "{The 1.5 Meter Solar Telescope GREGOR}",
  journal = an,
     year = 2012,
   volume = 333,
    pages = {796},
      doi = {10.1002/asna.201211725}
}

@ARTICLE{Schmidt2000,
   author = {{Schmidt}, W. and {Schlichenmaier}, R.},
    title = "{Small-Scale Flow Field in a Sunspot Penumbra}",
  journal = aa,
     year = 2000,
   volume = 364,
    pages = {829-834}
}

@ARTICLE{Schmidt2000b,
   author = {{Schmidt}, W. and {Muglach}, K. and {Kn{\"o}lker}, M.},
    title = "{Free-fall Downflow Observed in HE I 1083.0 Nanometers and H{$\beta$}}",
  journal = apj,
 keywords = {Sun: Atmospheric Motions, Sun: Chromosphere, Sun: Infrared},
     year = 2000,
   volume = 544,
    pages = {567-571},
      doi = {10.1086/317169},
}

@ARTICLE{Schmidt1999,
   author = {{Schmidt}, W. and {Stix}, M. and {W{\"o}hl}, H.},
    title = "{Center-to-limb Variation of the Solar Oscillation. New Results
             from MDI Data}",
  journal = aa,
     year = 1999,
   volume = 346,
    pages = {633-640}
}

@ARTICLE{Schmidt1994,
   author = {{Schmidt}, W. and {Knoelker}, M. and {Westendorp Plaza}, C.},
    title = "{Limb observations of the He I 1083.0 NM line}",
  journal = aap,
     year = 1994,
   volume = 287,
    pages = {229-232},
}

@ARTICLE{Schmieder1991,
   author = {{Schmieder}, B. and {Raadu}, M. A. and {Wiik}, J. E.},
    title = "{Fine Structure of Solar Filaments. II.\ Dynamics of Threads and
            Footpoints}",
  journal = aa,
     year = 1991,
   volume = 252,
    pages = {353-365}
}

@ARTICLE{Schrijver2011,
   author = {{Schrijver}, C. J. and {Aulanier}, G. and {Title}, A. M. and
            {Pariat}, E. and {Delann{\'e}e}, C.},
    title = "{The 2011 February 15 X2 Flare, Ribbons, Coronal Front, and Mass
            Ejection: Interpreting the Three-dimensional Views from the Solar
            Dynamics Observatory and STEREO Guided by Magnetohydrodynamic
            Flux-rope Modeling}",
  journal = apj,
     year = 2011,
   volume = 738,
    pages = {167},
      doi = {10.1088/0004-637X/738/2/167}
}

@ARTICLE{Schrijver2008,
   author = {{Schrijver}, C. J. and {DeRosa}, M. L. and {Metcalf}, T. and
            {Barnes}, G. and {Lites}, B. and {Tarbell}, T. and
            {McTiernan}, J. and {Valori}, G. and {Wiegelmann}, T. and
            {Wheatland}, M. S. and {Amari}, T. and {Aulanier}, G. and
            {D{\'e}moulin}, P. and {Fuhrmann}, M. and {Kusano}, K. and
            {R{\'e}gnier}, S. and {Thalmann}, J. K.},
    title = "{Nonlinear Force-Free Field Modeling of a Solar Active Region
            around the Time of a Major Flare and Coronal Mass Ejection}",
  journal = apj,
     year = 2008,
   volume = 675,
    pages = {1637-1644}
}

@ARTICLE{Schrijver1997,
   author = {{Schrijver}, C. J. and {Title}, A. M. and
            {van Ballegooijen}, A. A. and {Hagenaar}, H. J. and {Shine}, R. A.},
    title = "{Sustaining the Quiet Photospheric Network: The Balance of Flux
            Emergence, Fragmentation, Merging, and Cancellation}",
  journal = apj,
     year = 1997,
   volume = 487,
    pages = {424-436}
}

@ARTICLE{Schou2012,
   author = {{Schou}, J. and {Scherrer}, P. H. and {Bush}, R. I. and
            {Wachter}, R. and {Couvidat}, S. and {Rabello-Soares}, M. C. and
            {Bogart}, R. S. and {Hoeksema}, J. T. and {Liu}, Y. and
            {Duvall}, T. L. and {Akin}, D. J. and {Allard}, B. A. and
            {Miles}, J. W. and {Rairden}, R. and {Shine}, R. A. and 
            {Tarbell}, T. D. and {Title}, A. M. and {Wolfson}, C. J. and 
            {Elmore}, D. F. and {Norton}, A. A. and {Tomczyk}, S.},
    title = "{Design and Ground Calibration of the Helioseismic and Magnetic
            Imager (HMI) Instrument on the Solar Dynamics Observatory (SDO)}",
  journal = sp,
     year = 2012,
   volume = 275,
    pages = {229-259},
      doi = {10.1007/s11207-011-9842-2}
}

@ARTICLE{Schou2010,
   author = {{Schou}, J. and {Borrero}, J. M. and {Norton}, A. A. and {Tomczyk},
            S. and {Elmore}, D. and {Card}, G. L.},
    title = "{Polarization Calibration of the Helioseismic and Magnetic Imager
            (HMI) onborad the Solar Dynamics Observatory (SDO)}",
  journal = sp,
     year = 2010,
    pages = {177-206}
}

@ARTICLE{Schroeter1975,
   author = {{Schr{\"o}ter}, E. H. and {W{\"o}hl}, H.},
    title = "{Differential Rotation, Meridional and Random Motions of the Solar
            Ca$^{+}$ Network}",
  journal = sp,
     year = 1975,
   volume = 42,
    pages = {3-16}
}

@ARTICLE{Schuck2006,
   author = {{Schuck}, P. W.},
    title = "{Tracking Magnetic Footpoints with the Magnetic Induction
            Equation}",
  journal = apj,
     year = 2006,
   volume = 646,
    pages = {1358-1391}
}

@ARTICLE{Schuck2005,
   author = {{Schuck}, P. W.},
    title = "{Local Correlation Tracking and the Magnetic Induction Equation}",
  journal = apjl,
     year = 2005,
   volume = 632,
    pages = {L53-L56}
}

@ARTICLE{Schuessler2006,
   author = {{Sch{\"u}ssler}, M. and {V{\"o}gler}, A.},
    title = "{Magnetoconvection in a Sunspot Umbra}",
  journal = apjl,
     year = 2006,
   volume = 641,
    pages = {L73-L76}
}

@ARTICLE{Schuessler2005,
   author = {{Sch{\"u}ssler}, M. and {Rempel}, M.},
    title = "{The Dynamical Disconnection of Sunspots from their Magnetic
            Roots}",
  journal = aa,
     year = 2005,
   volume = 441,
    pages = {337-346}
}

@ARTICLE{Schuessler2003,
   author = {{Sch{\"u}ssler}, M. and {Shelyag}, S. and {Berdyugina}, S. and
            {V{\"o}gler}, A. and {Solanki}, S. K.},
    title = "{Why Solar Magnetic Flux Concentrations are Bright in Molecular
            Bands}",
  journal = apjl,
     year = 2003,
   volume = 597,
    pages = {L173-L176}
}

@ARTICLE{Schwenn2006,
  author   = {{Schwenn}, R.},
  title    = "{Space Weather: The Solar Perspective}",
  journal  = lrsp,
  year     = {2006},
  number   = {2},
  volume   = {3},
  url      = {http://www.livingreviews.org/lrsp-2006-2}
}

@ARTICLE{Schunker2010,
   author = {{Schunker}, H. and {Braun}, D. C.},
    title = "{Newly Identified Properties of Surface Acoustic Power}",
  journal = sp,
     year = 2010,
     note = {in press}
}

@ARTICLE{Shimizu2008,
   author = {{Shimizu}, T. and {Lites}, B. W. and {Katsukawa}, Y. and
            {Ichimoto}, K. and {Suematsu}, Y. and {Tsuneta}, S. and
            {Nagata}, S. and {Kubo}, M. and {Shine}, R. A. and
            {Tarbell}, T. D.},
    title = "{Frequent Occurrence of High-Speed Local Mass Downflows on the
            Solar Surface}",
  journal = apj,
     year = 2008,
   volume = 680,
    pages = {1467-1476}
}

@ARTICLE{Sheeley1972,
   author = {{Sheeley}, Jr., N. R.},
    title = "{Observations of the Horizontal Velocity Field Surrounding
            Sunspots}",
  journal = sp,
     year = 1972,
   volume = 25,
    pages = {98-103}
}

@ARTICLE{Shine2000,
   author = {{Shine}, R. A. and {Simon}, G. W. and {Hurlburt}, N. E.},
    title = "{Supergranule and Mesogranule Evolution}",
  journal = sp,
     year = 2000,
   volume = 193,
    pages = {313-331}
}

@ARTICLE{Shine1994,
   author = {{Shine}, R. A. and {Title}, A. M. and {Tarbell}, T. D. and
            {Smith}, K. and {Frank}, Z. A. and {Scharmer}, G.},
    title = "{High-Resolution Observations of the Evershed Effect in Sunspots}",
  journal = apj,
     year = 1994,
   volume = 430,
    pages = {413-424}
}

@INPROCEEDINGS{Shumko2006,
   author = {{Shumko}, S. and {Yang}, G.},
    title = "{Object-Oriented Communications for the NST's Telescope Control
            System. Design and Implementation}",
booktitle = {Advanced Software and Control for Astronomy},
   series = posp,
     year = 2006,
   volume = 6274,
   editor = {{Lewis}, H. and {Bridger}, A.},
    pages = {62741Q}
}

@INPROCEEDINGS{Shumko2005,
   author = {{Shumko}, S. and {Abramenko}, V. and {Denker}, C. and
            {Goode}, P. and {Tritschler}, A. and {Varsik}, J.},
    title = "{The Visible-Light Magnetograph at the Big Bear Solar Observatory:
            Hardware and Software}",
booktitle = {Astronomical Data Analysis Software and Systems XIV},
     year = 2005,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 347,
   editor = {{Shopbell}, P. and {Britton}, M. and {Ebert}, R.},
    pages = {509-513}
}

@INPROCEEDINGS{Shumko2002,
   author = {{Shumko}, S. and {Denker}, C. J. and {Varsik}, J. and
            {Didkovsky}, L. V. and {Marquette}, W. and {Goode}, P. R. and
            {Wang}, H.},
    title = "{Control and Acquisition Software for the Visible-Light
            Fabry-P{\'e}rot Interferometer at the Big Bear Solar Observatory}",
booktitle = {Advanced Telescope and Instrumentation Control Software II},
     year = 2002,
   series = posp,
   volume = 4848,
   editor = {{Lewis}, H.},
    pages = {483-489}
}

@INPROCEEDINGS{Simon1994,
   author = {{Simon}, G. W. and {Brandt}, P. N. and {November}, L. J. and
            {Scharmer}, G. B. and {Shine}, R. A.},
    title = "{Large-scale Photospheric Motions: First Results from an
            Extraordinary Eleven-Hour Granulation Observation}",
booktitle = {Solar Surface Magnetism},
     year = 1994,
   editor = {{Rutten}, R. J. and {Schrijver}, C. J.},
    pages = {261-270}
}

@ARTICLE{Simon1972,
   author = {{Simon}, G. W. and {Noyes}, R. W.},
    title = "{Solar Rotation as Measured in EUV Chromospheric and Coronal
            Lines}",
  journal = sp,
     year = 1972,
   volume = 26,
    pages = {8-14}
}

@ARTICLE{Sobotka2009,
   author = {{Sobotka}, M. and {Puschmann}, K. G.},
    title = "{Morphology and Evolution of Umbral Dots and their Substructures}",
  journal = aa,
     year = 2009,
   volume = 504,
    pages = {575-581}
}

@ARTICLE{Sobotka2007,
   author = {{Sobotka}, M. and {Roudier}, T.},
    title = "{Properties of Sunspot Moats Derived from Horizontal Motions}",
  journal = aa,
     year = 2007,
   volume = 472,
    pages = {277-282},
      doi = {10.1051/0004-6361:20077552}
}

@ARTICLE{Sobotka1999,
   author = {{Sobotka}, M. and {Brandt}, P. N. and {Simon}, G. W.},
    title = "{Fine Structure in Sunspots. III. Penumbral Grains}",
  journal = aa,
     year = 1999,
   volume = 348,
    pages = {621-626}
}

@ARTICLE{Sobotka1993,
   author = {{Sobotka}, M. and {Bonet}, J. A. and {Vazquez}, M.},
    title = "{A High-Resolution Study of Inhomogeneities in Sunspot Umbrae}",
  journal = apj,
     year = 1993,
   volume = 415,
    pages = {832-846}
}

@ARTICLE{SocasNavarro2005,
   author = {{Socas-Navarro}, H. and {Beckers}, J. and {Brandt}, P. and
            {Briggs}, J. and {Brown}, T. and {Brown}, W. and
            {Collados}, M. and {Denker}, C. and {Fletcher}, S. and
            {Hegwer}, S. and {Hill}, F. and {Horst}, T. and {Komsa}, M. and
            {Kuhn}, J. and {Lecinski}, A. and {Lin}, H. and {Oncley}, S. and
            {Penn}, M. and {Rimmele}, T. and {Streander}, K.},
    title = "{Solar Site Survey for the Advanced Technology Solar Telescope.
            I. Analysis of the Seeing Data}",
  journal = pasp,
     year = 2005,
   volume = 117,
    pages = {1296-1305}
}

@ARTICLE{Solanki2003,
   author = {{Solanki}, S. K.},
    title = "{Sunspots: An Overview}",
  journal = aar,
     year = 2003,
   volume = 11,
    pages = {153-286},
}

@INPROCEEDINGS{socas2001,
   author = {{Socas-Navarro}, H.},
    title = "{Stokes Inversion Techniques: Recent Achievements and
Future Horizons}",
booktitle = {Advanced Solar Polarimetry -- Theory, Observation, and
Instrumentation},
     year = 2001,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 236,
   editor = {{Sigwarth}, M.},
    pages = {487}
}

@ARTICLE{Solanki1993,
   author = {{Solanki}, S. K. and {Montavon}, C. A. P.},
    title = "{Uncombed Fields as the Source of the Broad-Band Circular
            Polarization of Sunspots}",
  journal = aa,
     year = 1993,
   volume = 275,
    pages = {283-292}
}

@ARTICLE{Soltau2012,
   author = {{Soltau}, D. and {Volkmer}, R. and {von der L{\"u}he}, O. and 
            {Berkefeld}, T.},
    title = "{Optical Design of the New Solar Telescope GREGOR}",
  journal = an,
     year = 2012,
   volume = 333,
    pages = {847-853},
      doi = {10.1002/asna.201211730}
}

@INPROCEEDINGS{Soltau2006,
   author = {{Soltau}, D. and {Berkefeld}, T. and {Volkmer}, R.},
    title = "{GREGOR AO as a Tool for Telescope Commissioning}",
booktitle = {Ground-Based and Airborne Telescopes},
     year = 2006,
   series = posp,
   volume = 6267,
   editor = {{Stepp}, L. M.},
    pages = {626711}
}

@INPROCEEDINGS{Spirock2001,
   author = {{Spirock}, T. and {Denker}, C. and {Chen}, H. and {Chae}, J. and
            {Qiu}, J. and {Varsik}, J. and {Wang}, H. and {Goode}, P. R. and
            {Marquette}, W.},
    title = "{The Big Bear Solar Observatory's Digital Vector Magnetograph}",
booktitle = {Advanced Solar Polarimetry -- Theory, Observation, and
            Instrumentation},
     year = 2001,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 236,
   editor = {{Sigwarth}, M.},
    pages = {65-72}
}

@ARTICLE{Spruit2006,
   author = {{Spruit}, H. C. and {Scharmer}, G. B.},
    title = "{Fine Structure, Magnetic Field and Heating of Sunspot Penumbrae}",
  journal = aa,
     year = 2006,
   volume = 447,
    pages = {343-354}
}

@ARTICLE{Spruit1979,
   author = {{Spruit}, H. C.},
    title = "{Convective Collapse of Flux Tubes}",
  journal = sp,
     year = 1979,
   volume = 61,
    pages = {363-378}
}

@ARTICLE{Staude1995,
   author = {{Staude}, J.},
    title = "{Sonnenforschung am Einsteinturm}",
  journal = sterne,
     year = 1995,
   volume = 71,
    pages = {142-150}
}

@ARTICLE{Staude1991,
   author = {{Staude}, J.},
    title = "{Das Sonnenobservatorium Einsteinturm in Potsdam. Erforschung
            solarer Magnetfelder und der Physik von Sonnenflecken}",
  journal = sw,
     year = 1991,
   volume = 30,
    pages = {505-509}
}

@ARTICLE{Stein2011,
   author = {{Stein}, R. F. and {Lagerfj{\"a}rd}, A. and {Nordlund}, {\AA}. and
            {Georgobiani}, D.},
    title = "{Solar Flux Emergence Simulations}",
  journal = sp,
     year = 2011,
   volume = 268,
    pages = {271-282},
      doi = {10.1007/s11207-010-9510-y}
}

@ARTICLE{Stein2006,
   author = {{Stein}, R. F. and {Nordlund}, {\AA}.},
    title = "{Solar Small-Scale Magnetoconvection}",
  journal = apj,
     year = 2006,
   volume = 642,
    pages = {1246-1255}
}

@ARTICLE{Steiner2001,
   author = {{Steiner}, O. and {Hauschildt}, P. H. and {Bruls}, J.},
    title = "{Radiative Properties of Magnetic Elements. I.\ Why are G-band
            Bright Points Bright?}",
  journal = aa,
     year = 2001,
   volume = 372,
    pages = {L13-L16}
}

@INPROCEEDINGS{Steinegger2001,
   author = {{Steinegger}, M. and {Denker}, C. and {Goode}, P. R. and
            {Marquette}, W. H. and {Varsik}, J. and {Wang}, H. and
            {Otruba}, W. and {Freislich}, H. and {Hanslmeier}, A. and
            {Luo}, G. and {Chen}, D. and {Zhang}, Q.},
    title = "{The New Global High-Resolution H$\alpha$ Network: Preliminary
            Results on the Chromospheric Differential Rotation}",
booktitle = {ESA Special Publication},
     year = 2001,
   series = {ESA Special Publication},
   volume = 464,
   editor = {{Wilson}, A. and {Pall{\'e}}, P. L.},
    pages = {315-320}
}

@ARTICLE{Steinegger2000a,
   author = {{Steinegger}, M. and {Hanslmeier}, A. and {Otruba}, W. and
            {Freislich}, H. and {Denker}, C. and {Goode}, P. R. and
            {Marquette}, W. M. and {Varied}, J. and {Wang}, H. and
            {Luo}, G. and {Chen}, D. and {Zhang}, Q.},
    title = "{An Overview of the New Global High-Resolution H$\alpha$
            Network}",
  journal = hob,
     year = 2000,
   volume = 24,
    pages = {179-184}
}

@INPROCEEDINGS{Steinegger2000b,
   author = {{Steinegger}, M. and {Denker}, C. and {Goode}, P. R. and
            {Marquette}, W. H. and {Varsik}, J. and {Wang}, H. and
            {Otruba}, W. and {Freislich}, H. and {Hanslmeier}, A. and
            {Luo}, G. and {Chen}, D. and {Zhang}, Q.},
    title = "{The New Global High-Resolution H$\alpha$ Network. First
            Observations and First Results}",
booktitle = {ESA Special Publication},
     year = 2000,
   series = {ESA Special Publication},
   volume = 463,
   editor = {{Wilson}, A.},
    pages = {617-622}
}

@INPROCEEDINGS{Strassmeier2008a,
   author = {{Strassmeier}, K. G. and {Woche}, M. and {Ilyin}, I. and
            {Popow}, E. and {Bauer}, S.-M. and {Dionies}, F. and
            {Fechner}, T. and {Weber}, M. and {Hofmann}, A. and {Storm}, J. and
            {Materne}, R. and {Bittner}, W. and {Bartus}, J. and
            {Granzer}, T. and {Denker}, C. and {Carroll}, T. and {Kopf}, M. and
            {DiVarano}, I. and {Beckert}, E. and {Lesser}, M.},
    title = "{PEPSI: The Potsdam Echelle Polarimetric and Spectroscopic
            Instrument for the LBT}",
booktitle = {Ground-Based and Airborne Instrumentation for Astronommy},
     year = 2008,
   series = posp,
   volume = 7014,
   editor = {{McLean}, I. S. and {Casali}, M. M.},
    pages = {70140N}
}

@INPROCEEDINGS{Strassmeier2008b,
   author = {{Strassmeier}, K. G. and {Granzer}, T. and {Denker}, C. and
            {Fuhrmann}, C. and {F{\"u}gner}, D. and {Woche}, M. and
            {Divarano}, I. and {Cutispoto}, G. and {Herber}, A. and 
            {Horne}, K. and {Rafanelli}, P. and {Bortoletto}, F. and 
            {Ribas}, I. and {Tosti}, G.},
    title = "{Science with ICE-T: Exoplanets and Stellar/Solar Activity}",
booktitle = {2$^{\rm nd}$ ARENA Conference: The Astrophysical Science Cases
            at Dome C},
     year = 2008,
   series = easps,
   volume = 33,
   editor = {{Zinnecker}, H. and {Epchtein}, N. and {Rauer}, H.},
    pages = {199-206}
}

@INPROCEEDINGS{Strassmeier2007,
   author = {{Strassmeier}, K. G. and {Woche}, M. and {Granzer}, T. and
            {Andersen}, M. I. and {Schmidt}, W. and {Koubsky}, P.},
    title = "{Gregor@Night}",
booktitle = {Modern Solar Facilities -- Advanced Solar Science},
     year = 2007,
   editor = {{Kneer}, F. and {Puschmann}, K. G. and {Wittmann}, A. D.},
    pages = {51-54}
}

@ARTICLE{Strous1996,
   author = {{Strous}, L. H. and {Scharmer}, G. and {Tarbell}, T. D. and
            {Title}, A. M. and {Zwaan}, C.},
    title = "{Phenomena in an Emerging Active Region. I. Horizontal Dynamics}",
  journal = aa,
     year = 1996,
   volume = 306,
    pages = {947-959}
}

@INPROCEEDINGS{Strous1995,
   author = {{Strous}, L. H.},
    title = "{Feature Tracking: Deriving Horizontal Motion and More}",
booktitle = {Helioseismology},
     year = 1995,
   series = {ESA Special Publication},
   volume = 376,
    pages = {213-217}
}

@ARTICLE{Sudol2005,
   author = {{Sudol}, J. J. and {Harvey}, J. W.},
    title = "{Longitudinal Magnetic Field Changes Accompanying Solar Flares}",
  journal = apj,
     year = 2005,
   volume = 635,
    pages = {647-658}
}

@ARTICLE{Suetterlin1998a,
   author = {{S{\"u}tterlin}, P. and {Wiehr}, E.},
    title = "{Temperature Mapping of Sunspots and Pores from Speckle
            Reconstructed Three Colour Photometry}",
  journal = aa,
     year = 1998,
   volume = 336,
    pages = {367-370}
}

@ARTICLE{Suetterlin1998b,
   author = {{S{\"u}tterlin}, P.},
    title = "{Properties of Solar Pores}",
  journal = aa,
     year = 1998,
   volume = 333,
    pages = {305-312}
}

@ARTICLE{Suetterlin1996,
   author = {{S{\"u}tterlin}, P. and {Schr{\"o}ter}, E. H. and
            {Muglach}, K.},
    title = "{Polarimetry of Solar Pores}",
  journal = sp,
     year = 1996,
   volume = 164,
    pages = {311-320}
}

@ARTICLE{Svanda2007,
   author = {{{\v S}vanda}, M. and {Zhao}, J. and {Kosovichev}, A. G.},
    title = "{Comparison of Large-Scale Flows on the Sun Measured by
            Time-Distance Helioseismology and Local Correlation Tracking}",
  journal = sp,
     year = 2007,
   volume = 241,
    pages = {27-37}
}



%====     TTTT    ==============================================================

@ARTICLE{Tan2009,
   author = {{Tan}, C. and {Chen}, P. F. and {Abramenko}, V. and {Wang}, H.},
    title = "{Evolution of Optical Penumbral and Shear Flows Associated with the
            X3.4 Flare of 2006 December 13}",
  journal = apj,
     year = 2009,
   volume = 690,
    pages = {1820-1828}
}

@ARTICLE{tenBruggecate1958,
   author = {{ten Bruggencate}, P. and {Voigt}, H.-H.},
    title = "{The Tower Telescope of the University Observatory G{\"o}ttingen.
            II.\ Improvements and Additional Instrumentation}",
  journal = {Ver{\"o}ffentlichungen der Universit{\"a}ts-Sternwarte zu G{\"o}ttingen},
     year = 1958,
   volume = 122,
    pages = {1-2}
}

@INPROCEEDINGS{Teran2000,
   author = {{Teran}, J. U. and {Porter}, D. S. and {Hileman}, E. A. and
            {Neff}, D. H.},
    title = "{Unique Dome Design for the SOAR Telescope Project}",
booktitle = {Telescope Structures, Enclosures, Controls,
            Assembly/Integration/Validation, and Commissioning},
   series = posp,
     year = 2000,
   volume = 4004,
   editor = {{Sebring}, T. A. and {Andersen}, T.},
    pages = {155-163}
}

@ARTICLE{Teriaca2003,
   author = {{Teriaca}, L. and {Falchi}, A. and {Cauzzi}, G. and {Falciani}, R. and 
	{Smaldone}, L.~A. and {Andretta}, V.},
    title = "{Solar and Heliospheric Observatory/Coronal Diagnostic Spectrograph 
        and Ground-based Observations of a Two-Ribbon Flare: Spatially Resolved 
        Signatures of Chromospheric Evaporation}",
  journal = apj,
     year = 2003,
   volume = 588,
    pages = {596-605},
      doi = {10.1086/373946},
}

@ARTICLE{Thomas2005,
   author = {{Thomas}, J. H.},
    title = "{Flows Along Penumbral Flux Tubes in Sunspots. Instability of
            Super-Alfv{\'e}nic, Serpentine Solutions}",
  journal = aa,
     year = 2005,
   volume = 440,
    pages = {29-32}
}

@ARTICLE{Thomas2002,
   author = {{Thomas}, J. H. and {Weiss}, N. O. and {Tobias}, S. M. and
            {Brummell}, N. H.},
    title = "{Downward Pumping of Magnetic Flux as the Cause of Filamentary
            Structures in Sunspot Penumbrae}",
  journal = nat,
     year = 2002,
   volume = 420,
    pages = {390-393}
}

@ARTICLE{Thomas1993,
   author = {{Thomas}, J. H. and {Montesinos}, B.},
    title = "{A Siphon-Flow Model of the Photospheric Evershed flow in a
            Sunspot}",
  journal = apj,
     year = 1993,
   volume = 407,
    pages = {398-401}
}

@ARTICLE{Thompson1999,
   author = {{Thompson}, B. J. and {Gurman}, J. B. and {Neupert}, W. M. and
            {Newmark}, J. S. and {Delaboudini{\`e}re}, J.-P. and
            {St.\ Cyr}, O. C. and {Stezelberger}, S. and {Dere}, K. P. and
            {Howard}, R. A. and {Michels}, D. J.},
    title = "{SOHO/EIT Observations of the 1997 April 7 Coronal Transient:
            Possible Evidence of Coronal Moreton Waves}",
  journal = apjl,
     year = 1999,
   volume = 517,
    pages = {L151-L154},
      doi = {10.1086/312030}
}

@ARTICLE{Tildesley2004,
   author = {{Tildesley}, M. J. and {Weiss}, N. O.},
    title = "{On the Origin of Filamentary Structure in Sunspot Penumbrae:
            Non-Linear Results}",
  journal = mn,
     year = 2004,
   volume = 350,
    pages = {657-670},
      doi = {10.1111/j.1365-2966.2004.07678.x}
}

@INPROCEEDINGS{Title1998,
   author = {{Title}, A. M. and {Schrijver}, C. J.},
    title = "{The Sun's Magnetic Carpet}",
booktitle = {Cool Stars, Stellar Systems, and the Sun},
     year = 1998,
   series = asp,
   volume = 154,
   editor = {{Donahue}, R. A. and {Bookbinder}, J. A.},
    pages = {345-358}
}

@ARTICLE{Title1993,
   author = {{Title}, A. M. and {Frank}, Z. A. and {Shine}, R. A. and
            {Tarbell}, T. D. and {Topka}, K. P. and {Scharmer}, G. and
            {Schmidt}, W.},
    title = "{On the Magnetic and Velocity Field Geometry of Simple Sunspots}",
  journal = apj,
     year = 1993,
   volume = 403,
    pages = {780-796}
}

@ARTICLE{Title1989,
   author = {{Title}, A. M. and {Tarbell}, T. D. and {Topka}, K. P. and
            {Ferguson}, S. H. and {Shine}, R. A. and {SOUP Team}},
    title = "{Statistical Properties of Solar Granulation Derived from the SOUP
            Instrument on Spacelab 2}",
  journal = apj,
     year = 1989,
   volume = 336,
    pages = {475-494}
}

@ARTICLE{Title1986,
   author = {{Title}, A. M. and {Tarbell}, T. D. and {Acton}, L. and 
            {Duncan}, D. and {Simon}, G. W.},
    title = "{White-Light Movies of the Solar Photosphere from the SOUP
            Instrument on Spacelab}",
  journal = advsr,
     year = 1986,
   volume = 6,
    pages = {253-262}
}

@ARTICLE{Tritschler2006,
   author = {{Tritschler}, A. and {Uitenbroek}, H.},
    title = "{The Contrast of Magnetic Flux Concentrations at Near-Infrared and
            Visible Wavelengths}",
  journal = apj,
     year = 2006,
   volume = 648,
    pages = {741-752}
}

@ARTICLE{Tritschler2004,
   author = {{Tritschler}, A. and {Schlichenmaier}, R. and 
            {Bellot Rubio}, L. R. and {Berkefeld}, T. and {Schelenz}, T.},
    title = "{Two-Dimensional Spectroscopy of a Sunspot. I. Properties of the
            Penumbral Fine Structure}",
  journal = aa,
     year = 2004,
   volume = 415,
    pages = {717-729}
}

@ARTICLE{Tritschler2002,
   author = {{Tritschler}, A. and {Schmidt}, W.},
    title = "{Sunspot Photometry with Phase Diversity. II. Fine-Structure
            Characteristics}",
  journal = aa,
     year = 2002,
   volume = 388,
    pages = {1048-1061}
}

@ARTICLE{Tsiropoula1993,
   author = {{Tsiropoula}, G. and {Alissandrakis}, C. E. and {Schmieder}, B.},
    title = "{The Fine Structure of a Chromospheric Rosette}",
  journal = aa,
     year = 1993,
   volume = 271,
    pages = {574-586}
}

@ARTICLE{Tsiropoula1992,
   author = {{Tsiropoula}, G. and {Georgakilas}, A. A. and
            {Alissandrakis}, C. E. and {Mein}, P.},
    title = "{Time Evolution of Arch Filaments}",
  journal = aa,
     year = 1992,
   volume = 262,
    pages = {587-596}
}

@ARTICLE{Tsuneta2008,
   author = {{Tsuneta}, S. and {Ichimoto}, K. and {Katsukawa}, Y. and {Nagata},
            S. and {Otsubo}, M. and {Shimizu}, T. and {Suematsu}, Y. and
            {Nakagiri}, M. and {Noguchi}, M. and {Tarbell}, T. and {Title}, A.
            and {Shine}, R. and {Rosenberg}, W. and {Hoffmann}, C. and
            {Jurcevich}, B. and {Kushner}, G. and {Levay}, M. and {Lites}, B.
            and {Elmore}, D. and {Matsushita}, T. and {Kawaguchi}, N. and
            {Saito}, H. and {Mikami}, I. and {Hill}, L. D. and {Owens}, J. K.},
    title = "{The Solar Optical Telescope for the Hinode Mission: An Overview}",
  journal = sp,
     year = 2008,
   volume = 249,
    pages = {167-196},
      doi = {10.1007/s11207-008-9174-z}
}

@ARTICLE{Tziotziou2003,
   author = {{Tziotziou}, K. and {Tsiropoula}, G. and {Mein}, P.},
    title = "{On the Nature of the Chromospheric Fine Structure. I.\ Dynamics of
            Dark Mottles and Grains}",
  journal = aa,
     year = 2003,
   volume = 402,
    pages = {361-372}
}

@ARTICLE{Tziotziou2001,
   author = {{Tziotziou}, K. and {Heinzel}, P. and {Mein}, P. and
           {Mein}, N.},
    title = "{Non-LTE Inversion of Chromospheric Ca\,\textsc{ii} Cloud-Like
            Features}",
  journal = aa,
     year = 2001,
   volume = 366,
    pages = {686-698}
}



%====     UUUU    ==============================================================

@ARTICLE{Uitenbroek2006,
   author = {{Uitenbroek}, H. and {Balasubramaniam}, K. S. and
            {Tritschler}, A.},
    title = "{Evidence for a Siphon Flow Ending near the Edge of a Pore}",
  journal = apj,
     year = 2006,
   volume = 645,
    pages = {776-781}
}

@ARTICLE{Ulrich1970,
   author = {{Ulrich}, R. K.},
    title = "{The Five-Minute Oscillations on the Solar Surface}",
  journal = apj,
     year = 1970,
   volume = 162,
    pages = {993-1002}
}



%====     VVVV    ==============================================================

@ARTICLE{vonAlvensleben1957,
   author = {{von Alvensleben}, A.},
    title = "{Apparatekonturen, Gittergeister und Streulicht der beiden neuen
            Plangitter am G{\"o}ttinger Sonnenturm}",
  journal = zap,
     year = 1957,
   volume = 43,
    pages = {63-84}
}

@ARTICLE{vanNoort2008,
   author = {{van Noort}, M. J. and {Rouppe van der Voort}, L. H. M.},
    title = "{Stokes Imaging Polarimetry Using Image Restoration at the Swedish
            1-m Solar Telescope}",
  journal = aa,
     year = 2008,
   volume = 489,
    pages = {429-440},
      doi = {10.1051/0004-6361:200809959}
}

@INPROCEEDINGS{vanNoort2006,
   author = {{van Noort}, M. and {Rouppe van der Voort}, L. and
            {L{\"o}fdahl}, M.},
    title = "{Solar Image Restoration by use of Multi-Object Multi-Frame Blind
            Deconvolution}",
booktitle = {Solar MHD Theory and Observations: A High Spatial Resolution
            Perspective},
     year = 2006,
   series = asp,
   volume = 354,
   editor = {{Leibacher}, J. and {Stein}, R. F. and {Uitenbroek}, H.},
    pages = {55-60}
}

@ARTICLE{vanNoort2005,
   author = {{van Noort}, M. and {Rouppe van der Voort}, L. and
            {L{\"o}fdahl}, M. G.},
    title = "{Solar Image Restoration by Use of Multi-frame Blind Deconvolution
            with Multiple Objects and Phase Diversity}",
  journal = sp,
     year = 2005,
   volume = 228,
    pages = {191-215},
      doi = {10.1007/s11207-005-5782-z}
}

@ARTICLE{VargasDominguez2010,
   author = {{Vargas Dom{\'{\i}}nguez}, S. and {de Vicente}, A. and
            {Bonet}, J. A. and {Mart{\'{\i}}nez Pillet}, V.},
    title = "{Characterization of Horizontal Flows around Solar Pores
            from High-Resolution Time Series of Images.}",
  journal = aa,
     year = 2010,
   volume = 516,
    pages = {A91}
}

@ARTICLE{VargasDominguez2008,
   author = {{Vargas Dom{\'{\i}}nguez}, S. and {Rouppe van der Voort}, L. and 
            {Bonet}, J. A. and {Mart{\'{\i}}nez Pillet}, V. and
            {Van Noort}, M. and {Katsukawa}, Y.},
    title = "{Moat Flow in the Vicinity of Sunspots for Various Penumbral
            Configurations}",
  journal = apj,
     year = 2008,
   volume = 679,
    pages = {900-909},
      doi = {10.1086/587139}
}

@ARTICLE{VargasDominguez2007,
   author = {{Vargas Dom{\'{\i}}nguez}, S. and {Bonet}, J. A. and
            {Mart{\'{\i}}nez Pillet}, V. and {Katsukawa}, Y. and
            {Kitakoshi}, Y. and {Rouppe van der Voort}, L.},
    title = "{On the Moat-Penumbra Relation}",
  journal = apjl,
     year = 2007,
   volume = 660,
    pages = {165-168}
}

@INPROCEEDINGS{Varsik2006,
   author = {{Varsik}, J. R. and {Yang}, G.},
    title = "{Design of a Telescope Pointing and Tracking Subsystem for the Big
            Bear Solar Observatory New Solar Telescope}",
booktitle = {Advanced Software and Control for Astronomy},
   series = posp,
     year = 2006,
   volume = 6274,
   editor = {{Lewis}, H. and {Bridger}, A.},
    pages = {62741T}
}

@ARTICLE{Verdoni2007,
   author = {{Verdoni}, A. P. and {Denker}, C.},
    title = "{The Local Seeing Environment at Big Bear Solar Observatory}",
  journal = pasp,
     year = 2007,
   volume = 119,
    pages = {793-804}
}

@INPROCEEDINGS{Verdoni2006,
   author = {{Verdoni}, A. P. and {Denker}, C.},
    title = "{The Thermal Control Systems of the New Solar Telescope at Big
            Bear Solar Observatory}",
booktitle = {Ground-Based and Airborne Telescopes},
   series = posp,
     year = 2006,
   volume = 6267,
   editor = {{Stepp}, L. M.},
    pages = {62670M}
}

@ARTICLE{Verma2014,
   author = {{Verma}, M. and {Denker}, C.},
    title = "{Horizontal Flow Fields Observed in Hinode G-band Images. IV.\
            Statistical Properties of the Dynamical Environment around Pores}",
  journal = aa,
     year = 2014,
   volume = 563,
      eid = {A112},
    pages = {A112},
      doi = {10.1051/0004-6361/201322476} 
}

@ARTICLE{Verma2013,
   author = {{Verma}, M. and {Steffen}, M. and {Denker}, C.},
    title = "{Evaluating Local Correlation Tracking Using CO5BOLD Simulations of
            Solar Granulation}",
  journal = aa,
     year = 2013,
   volume = 555,
      eid = {A136},
    pages = {A136},
      doi = {10.1051/0004-6361/201321628}
}

@ARTICLE{Verma2012a,
   author = {{Verma}, M. and {Balthasar}, H. and {Deng}, N. and {Liu}, C. and
            {Shimizu}, T. and {Wang}, H. and {Denker}, C.},
    title = "{Horizontal Flow Fields Observed in Hinode G-band Images. II.\ Flow
            Fields in the Final Stages of Sunspot Decay}",
  journal = aa,
     year = 2012,
   volume = 538,
    pages = {A109}
}

@ARTICLE{Verma2012b,
   author = {{Verma}, M. and {Denker}, C.},
    title = "{Horizontal Flow Fields Observed in Hinode G-band Images. III.\
            The Decay of a Satellite Sunspot and the Role of Magnetic Flux
            Removal in Flaring}",
  journal = aa,
     year = 2012,
   volume = 545,
    pages = {A192}
}

@ARTICLE{Verma2011,
   author = {{Verma}, M. and {Denker}, C.},
    title = "{Horizontal Flow Fields Observed in Hinode G-Band Images. I.\
            Methods}",
  journal = aa,
     year = 2011,
   volume = 529,
    pages = {A153},
      doi = {10.1051/0004-6361/201016358}
}

@ARTICLE{Vernazza1981,
   author = {{Vernazza}, J. E. and {Avrett}, E. H. and {Loeser}, R.},
    title = "{Structure of the Solar Chromosphere. III.\ Models of the EUV
            Brightness Components of the Quiet-Sun}",
  journal = apjss,
     year = 1981,
   volume = 45,
    pages = {635-725},
      doi = {10.1086/190731}
}

@ARTICLE{Vernin1994,
   author = {{Vernin}, J. and {Munoz-Tunon}, C.},
    title = "{Optical Seeing at La Palma Observatory. II. Intensive Site Testing
            Campaign at the Nordic Optical Telescope}",
  journal = aa,
     year = 1994,
   volume = 284,
    pages = {311-318}
}

@ARTICLE{Villarino2006,
   author = {{Villarino}, M. B.},
    title = "{A Note on the Accuracy of Ramanujan's Approximative Formula for
            the Perimeter of an Ellipse}",
  journal = {J. Ineq. Pure Appl. Math.},
     year = 2006,
   volume = 7,
    pages = {21}
}

@ARTICLE{Viereck2004,
   author = {{Viereck}, R. A. and {Floyd}, L. E. and {Crane}, P. C. and
            {Woods}, T. N. and {Knapp}, B. G. and {Rottman}, G. and
            {Weber}, M. and {Puga}, L. C. and {DeLand}, M. T.},
    title = "{A Composite Mg\,\textsc{ii} Index Spanning from 1978 to 2003}",
  journal = {Space Weather},
     year = 2004,
   volume = 2,
    pages = {S10005}
}

@ARTICLE{Viereck1999,
   author = {{Viereck}, R. A. and {Puga}, L. C.},
    title = "{The NOAA Mg\,\textsc{ii} Core-to-Wing Solar Index: Construction of
            a 20-Year Time Series of Chromospheric Variability from Multiple
            Satellites}",
  journal = jgr,
     year = 1999,
   volume = 104,
    pages = {9995-10006}
}

@ARTICLE{Voegler2007,
   author = {{V{\"o}gler}, A. and {Sch{\"u}ssler}, M.},
    title = "{A Solar Surface Dynamo}",
  journal = aa,
     year = 2007,
   volume = 465,
    pages = {L43-L46},
      doi = {10.1051/0004-6361:20077253},
}

@ARTICLE{Voegler2005,
   author = {{V{\"o}gler}, A. and {Shelyag}, S. and {Sch{\"u}ssler}, M. and 
            {Cattaneo}, F. and {Emonet}, T. and {Linde}, T.},
    title = "{Simulations of Magneto-Convection in the Solar Photosphere. 
            Equations, Methods, and Results of the MURaM Code}",
  journal = aa,
     year = 2005,
   volume = 429,
    pages = {335-351},
      doi = {10.1051/0004-6361:20041507}
}

@ARTICLE{Vogler2005,
   author = {{Vogler}, F. L. and {Brandt}, P. N. and {Otruba}, W. and
            {Hanslmeier}, A.},
    title = "{Solar Irradiance Variations Modelled from Ca\,{\sc ii}\,K Excess
             and Magnetic Field}",
  journal = hob,
     year = 2005,
   volume = 29,
    pages = {79-88}
}

@ARTICLE{Volkmer2012,
   author = {{Volkmer}, R. and {Eisentr{\"a}ger}, P. and {Emde}, P. and {Fischer}, A. and 
	{von der L{\"u}he}, O. and {Nicklas}, H. and {Soltau}, D. and 
	{Schmidt}, W. and {Weis}, U.},
    title = "{Mechanical design of the solar telescope GREGOR}",
  journal = an,
 keywords = {instrumentation: high angular resolution, methods: observational, Sun: general, telescopes},
     year = 2012,
   volume = 333,
    pages = {816},
      doi = {10.1002/asna.201211740},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Volkmer2010a,
   author = {{Volkmer}, R. and {von der L{\"u}he}, O. and {Denker}, C. and
            {Solanki}, S. and {Balthasar}, H. and {Berkefeld}, T. and
            {Caligari}, P. and {Collados Vera}, M. and {Halbgewachs}, C. and
            {Heidecke}, F. and {Hofmann}, A. and {Klva{\v n}a}, M. and
            {Kneer}, F. and {Lagg}, A. and {Schmidt}, W. and {Sobotka}, M. and
            {Soltau}, D. and {Strassmeier}, K. G.},
    title = "{GREGOR Telescope: Start of Commissioning}",
booktitle = {Ground-Based and Airborne Telescopes III},
   series = posp,
     year = 2010,
   volume = {7733},
   editor = {{Stepp}, L. M. and {Gilmozzi}, R. and {Hall}, H. J.},
    pages = {77330K}
}

@ARTICLE{Volkmer2010b,
   author = {{Volkmer}, R. and {von der L{\"u}he}, O. and {Denker}, C. and
            {Solanki}, S. and {Balthasar}, H. and {Berkefeld}, T. and
            {Caligari}, P. and {Collados}, M. and {Fischer}, A. and
            {Halbgewachs}, C. and {Heidecke}, F. and {Hofmann}, A. and
            {Klva{\v n}a}, M. and {Kneer}, F. and {Lagg}, A. and {Popow}, E. and
            {Schmidt}, D. and {Schmidt}, W. and {Sobotka}, M. and
            {Soltau}, D. and {Strassmeier}, K. G.},
    title = "{GREGOR Solar Telescope}",
  journal = an,
     year = 2010,
   volume = 331,
    pages = {624-627}
}

@INPROCEEDINGS{Volkmer2008,
   author = {{Volkmer}, R.},
    title = "{Thermal Characteristics of the Solar Telescope GREGOR}",
booktitle = {Ground-Based and Airborne Telescopes II},
     year = 2008,
   series = posp,
   volume = 7012,
   editor = {Stepp, L. M. and {Gilmozzi}, R.},
    pages = {70120K}
}

@INPROCEEDINGS{Volkmer2007,
   author = {{Volkmer}, R. and {von der L{\"u}he}, O. and {Kneer}, F. and
            {Staude}, J. and {Balthasar}, H. and {Berkefeld}, T. and
            {Caligari}, P. and {Collados}, M. and {Halbgewachs}, C. and
            {Heidecke}, F. and {Hofmann}, A. and {Klva{\v n}a}, M. and
            {Sobotka}, M. and {Nicklas}, H. and {Popow}, E. and
            {Puschmann}, K. G. and {Schmidt}, W. and {Soltau}, D. and
            {Strassmeier}, K. G. and {Wittmann}, A. D.},
    title = "{New High Resolution Solar Telescope GREGOR}",
booktitle = {Modern Solar Facilities -- Advanced Solar Science},
     year = 2007,
   editor = {{Kneer}, F. and {Puschmann}, K. G. and {Wittmann}, A. D.},
    pages = {39-44}
}

@INPROCEEDINGS{Volkmer2006,
   author = {{Volkmer}, R. and {von der L{\"u}he}, O. and {Kneer}, F. and
            {Staude}, J. and {Berkefeld}, T. and {Caligari}, P. and
            {Halbgewachs}, C. and {Heidecke}, F. and {Schmidt}, W. and
            {Soltau}, D. and {Nicklas}, H. and {Wittmann}, A. and
            {Balthasar}, H. and {Hofmann}, A. and {Strassmeier}, K. and
            {Sobotka}, M. and {Klva{\v n}a}, M. and {Collados}, M.},
    title = "{The New 1.5-Meter Solar Telescope GREGOR: First-Light and Start
            of Commissioning}",
booktitle = {Ground-Based and Airborne Telescopes},
     year = 2006,
   series = posp,
   volume = 6267,
   editor = {{Stepp}, L. M.},
    pages = {62670W}
}

@INPROCEEDINGS{Volkmer2005,
   author = {{Volkmer}, R. and {von der L{\"u}he}, O. and {Kneer}, F. and
            {Staude}, J. and {Berkefeld}, T. and {Caligari}, P. and
            {Halbgewachs}, C. and {Schmidt}, W. and {Soltau}, D. and
            {Nicklas}, H. and {Wittmann}, A. and {Balthasar}, H. and
            {Hofmann}, A. and {Strassmeier}, K. and {Sobotka}, M. and
            {Klva{\v n}a}, M. and {Collados}, M.},
    title = "{The New 1.5-Meter Solar Telescope GREGOR: Progress Report and
            Results of Performance Tests}",
booktitle = {Solar Physics and Space Weather Instrumentation},
   series = posp,
     year = 2005,
   volume = 5901,
   editor = {{Fineschi}, S. and {Viereck}, R. A.},
    pages = {75-83}
}


@INPROCEEDINGS{vonderLuehe2003,
   author = {{von der L{\"u}he}, O. and {Soltau}, D. and {Berkefeld}, T. and 
            {Schelenz}, T.},
     year = 2003,
    title = "{KAOS: Adaptive Optics System for the Vacuum Tower Telescope at
            Teide Observatory}",
   editor = {{Keil}, S. L. and {Avakyan}, S. V.},
booktitle = {Innovative Telescopes and Instrumentation for Solar Astrophysics},
   series = posp,
   volume = 4853,
    pages = {187-193}
}


@ARTICLE{vonderLuehe2001,
   author = {{von der L{\"u}he}, O. and {Schmidt}, W. and {Soltau}, D. and
            {Berkefeld}, T. and {Kneer}, F. and {Staude}, J.},
    title = "{GREGOR: A 1.5-Meter Telescope for Solar Research}",
  journal = an,
     year = 2001,
   volume = 322,
    pages = {353-360}
}

@ARTICLE{vonderLuehe1998,
   author = {{von der L{\"u}he}, O.},
    title = "{High-Resolution Observations with the German Vacuum Tower
            Telescope on Tenerife}",
  journal = nar,
     year = 1998,
   volume = 42,
    pages = {493-497},
      doi = {10.1016/S1387-6473(98)00060-8}
}


%====     WWWW    ==============================================================

@ARTICLE{Wachter2011,
   author = {{Wachter}, R. and {Schou}, J. and {Rabello-Soares}, M. C. and
            {Miles}, J. W. and {Duvall}, T. L. and {Bush}, R. I.},
    title = "{Image Quality of the Helioseismic and Magnetic Imager (HMI)
            Onboard the Solar Dynamics Observatory (SDO)}",
  journal = sp,
     year = 2011,
    pages = {19-43}
}

@ARTICLE{Walton2003,
   author = {{Walton}, S. R. and {Preminger}, D. G. and {Chapman}, G. A.},
    title = "{The Contribution of Faculae and Network to Long-Term Changes in
            the Total Solar Irradiance}",
  journal = apj,
     year = 2003,
   volume = 590,

    pages = {1088-1094}
}

@INPROCEEDINGS{Wagner2008,
   author = {{Wagner}, J. and {Rimmele}, T. R. and {Keil}, S. and
            {Hubbard}, R. and {Hansen}, E. and {Phelps}, L. and {Warner}, M. and
            {Goodrich}, B. and {Richards}, K. and {Hegwer}, S. and
            {Kneale}, R. and {Ditsler}, J.},
    title = "{Advanced Technology Solar Telescope: A Progress Report}",
booktitle = {Ground-Based and Airborne Telescopes II},
     year = 2008,
   series = posp,
   volume = 7012,
   editor = {{Stepp}, L. M. and {Gilmozzi}, R.},
    pages = {70120I}
}

@INPROCEEDINGS{Wagner2006,
   author = {{Wagner}, J. and {Rimmele}, T. R. and {Keil}, S. and {Barr}, J. and
            {Dalrymple}, N. and {Ditsler}, J. and {Goodrich}, B. and
            {Hansen}, E. and {Hegwer}, S. and {Hill}, F. and {Hubbard}, R. and
            {Phelps}, L. and {Price}, R. and {Richards}, K. and {Warner}, M.},
    title = "{Advanced Technology Solar Telescope: A Progress Report}",
booktitle = {Ground-Based and Airborne Telescopes},
     year = 2006,
   series = posp,
   volume = 6267,
   editor = {{Stepp}, L. M.},
    pages = {626709}
}

@ARTICLE{Wang2011,
   author = {{Wang}, S. and {Liu}, C. and {Liu}, R. and {Deng}, N. and
            {Liu}, Y. and {Wang}, H.},
    title = "{First Flare-Related Rapid Change of Photospheric Magnetic Field
            Observed by Solar Dynamics Observatory}",
  journal = {ArXiv e-prints},
   pages = {1103.0027},
     year = 2011
}

@ARTICLE{Wang2008,
   author = {{Wang}, H. and {Jing}, J. and {Tan}, C. and {Wiegelmann}, T. and
            {Kubo}, M.},
    title = "{Study of Magnetic Channel Structure in Active Region 10930}",
  journal = apj,
     year = 2008,
   volume = 687,
    pages = {658-667}
}

@ARTICLE{Wang2006,
   author = {{Wang}, J.},
    title = "{Reconnection in the Lower Solar Atmosphere and Coronal Mass Ejections}",
  journal = advsr,
     year = 2006,
   volume = 38,
    pages = {1887-1893}
}

@ARTICLE{Wang2004,
   author = {{Wang}, H. and {Liu}, C. and {Qiu}, J. and {Deng}, N. and
            {Goode}, P. R. and {Denker}, C.},
    title = "{Rapid Penumbral Decay following Three X-Class Solar Flares}",
  journal = apjl,
     year = 2004,
   volume = 601,
    pages = {195-198}
}

@ARTICLE{Wang2002,
   author = {{Wang}, H. and {Spirock}, T. J. and {Qiu}, J. and {Ji}, H. and
            {Yurchyshyn}, V. and {Moon}, Y.-J. and {Denker}, C. and
            {Goode}, P. R.},
    title = "{Rapid Changes of Magnetic Fields Associated with Six X-Class
            Flares}",
  journal = apj,
     year = 2002,
   volume = 576,
    pages = {497-504}
}

@ARTICLE{Wang2001,
   author = {{Wang}, J. and {Wang}, H. and {Goode}, P. R. and
            {Spirock}, T. J. and {Lee}, C.-Y. and {Ravindra}, N. M. and
            {Ma}, J. and {Denker}, C.},
    title = "{Optical Design of Near-Infrared Birefringent Filter System and
            Measurement of Birefringent Index of Calcite at 1.56 $\mu$m}",
  journal = oe,
     year = 2001,
   volume = 40,
    pages = {1016-1023}
}

@ARTICLE{Wang2000a,
   author = {{Wang}, H. and {Goode}, P. R. and {Denker}, C. and {Yang}, G. and
            {Yurchyshyn}, V. and {Nitta}, N. and {Gurman}, J. B. and
            {St. Cyr}, C. and {Kosovichev}, A. G.},
    title = "{Comparison of the 1998 April 29 M6.8 and 1998 November 5 M8.4
            Flares}",
  journal = apj,
     year = 2000,
   volume = 536,
    pages = {971-981}
}

@ARTICLE{Wang2000b,
   author = {{Wang}, J. and {Li}, W. and {Denker}, C. and {Lee}, C. and
            {Wang}, H. and {Goode}, P. R. and {McAllister}, A. and
            {Martin}, S. F.},
    title = "{Minifilament Eruption on the Quiet Sun. I. Observations at
            H$\alpha$ Central Line}",
  journal = apj,
     year = 2000,
   volume = 530,
    pages = {1071-1084}
}

@INPROCEEDINGS{Wang2000c,
   author = {{Wang}, J. and {Wang}, H. and {Spirock}, T. J. and {Lee}, C. and
            {Ravindra}, N. M. and {Ma}, J. and {Goode}, P. R. and
            {Denker}, C.},
    title = "{Optical Design of a Near-Infrared Birefringent Filter System and
            Measurement of Birefringence Index of Calcite}",
booktitle = {Current Developments in Lens Design and Optical Systems
            Engineering},
     year = 2000,
   series = posp,
   volume = 4093,
   editor = {{Fischer}, R. E. and {Johnson}, R. B. and {Smith}, W. J. and
            {Swantner}, W. H.},
    pages = {481-489}
}

@ARTICLE{Wang2000d,
   author = {{Wang}, H. and {Qiu}, J. and {Denker}, C. and {Spirock}, T. and
            {Chen}, H. and {Goode}, P. R.},
    title = "{High-Cadence Observations of an Impulsive Flare}",
  journal = apj,
     year = 2000,
   volume = 542,
    pages = {1080-1087}
}

@ARTICLE{Wang1998a,
   author = {{Wang}, H.},
    title = "{Comparison of H{$\alpha$} and He\,{\sc ii} $\lambda$304
            Macrospicules}",
  journal = apj,
     year = 1998,
   volume = 509,
    pages = {461-470}
}

@ARTICLE{Wang1998b,
   author = {{Wang}, H. and {Denker}, C. and {Spirock}, T. and
            {Goode}, P. R. and {Yang}, S. and {Marquette}, W. and
            {Varsik}, J. and {Fear}, R. J. and {Nenow}, J. and
            {Dingley}, D. D.},
    title = "{New Digital Magnetograph at Big Bear Solar Observatory}",
  journal = sp,
     year = 1998,
   volume = 183,
    pages = {1-13}
}

@ARTICLE{Wang1998c,
   author = {{Wang}, H. and {Johannesson}, A. and {Stage}, M. and {Lee}, C. and
            {Zirin}, H.},
    title = "{Study of H$\alpha$ Jets on the Quiet Sun}",
  journal = sp,
     year = 1998,
   volume = 178,
    pages = {55-69}
}

@ARTICLE{Wang1992,
   author = {{Wang}, H. and {Zirin}, H.},
    title = "{Flows around Sunspots and Pores}",
  journal = sp,
     year = 1992,
   volume = 140,
    pages = {41-54}
}

@ARTICLE{Warren1996,
   author = {{Warren}, H. P. and {Mariska}, J. T. and {Lean}, J. and
            {Marquette}, W. and {Johannesson}, A.},
    title = "{Modeling Solar Extreme Ultraviolet Irradiance Variability Using
            Emission Measure Distributions}",
  journal = grl,
     year = 1996,
   volume = 23,
    pages = {2207-2210}
}

@ARTICLE{WedemeyerBoehm2009,
   author = {{Wedemeyer-B{\"o}hm}, S. and {Lagg}, A. and {Nordlund}, {\AA}.},
    title = "{Coupling from the Photosphere to the Chromosphere and the
            Corona}",
  journal = ssr,
     year = 2009,
   volume = 144,
    pages = {317-350},
      doi = {10.1007/s11214-008-9447-8}
}

@ARTICLE{Weigelt1983,
   author = {{Weigelt}, G. and {Wirnitzer}, B.},
    title = "{Image Reconstruction by the Speckle-Masking Method}",
  journal = ol,
     year = 1983,
   volume = 8,
    pages = {389-391}
}

@ARTICLE{Weiss2002,
   author = {{Weiss}, N. O.},
    title = "{Umbral and Penumbral Magnetoconvection}",
  journal = an,
     year = 2002,
   volume = 323,
    pages = {371-376}
}

@ARTICLE{Wells1981,
   author = {{Wells}, D. C. and {Greisen}, E. W. and {Harten}, R. H.},
    title = "{FITS -- A Flexible Image Transport System}",
  journal = aas,
     year = 1981,
   volume = 44,
    pages = {363-370}
}

@ARTICLE{Welsch2012,
   author = {{Welsch}, B. T. and {Kusano}, K. and {Yamamoto}, T. T. and
            {Muglach}, K.},
    title = "{Decorrelation Times of Photospheric Fields and Flows}",
  journal = apj,
     year = 2012,
   volume = 747,
    pages = {130},
      doi = {10.1088/0004-637X/747/2/130}
}

@ARTICLE{Welsch2007,
   author = {{Welsch}, B. T. and {Abbett}, W. P. and {De Rosa}, M. L. and
            {Fisher}, G. H. and {Georgoulis}, M. K. and {Kusano}, K. and
            {Longcope}, D. W. and {Ravindra}, B. and {Schuck}, P. W.},
    title = "{Tests and Comparisons of Velocity-Inversion Techniques}",
  journal = apj,
     year = 2007,
   volume = 670,
    pages = {1434-1452}
}

@BOOK{Wilderotter2005,
   author = {{Wilderotter}, H.},
    title = "{Ein Turm f{\"u}r Albert Einstein. Potsdam, das Licht und die
            Erforschung des Himmels}",
publisher = {L{\&}H Verlag, Hamburg},
     year = 2005
}

@ARTICLE{Wilken1997,
   author = {{Wilken}, V. and {de Boer}, C. R. and {Denker}, C. and
            {Kneer}, F.},
    title = "{Speckle Measurements of the Centre-to-Limb Variation of the Solar
            Granulation}",
  journal = aa,
     year = 1997,
   volume = 325,
    pages = {819-824}
}

@ARTICLE{Woodhouse2004,
   author = {{Woodhouse}, C. A.},
    title = "{A Paleo Perspective on Hydroclimatic Variability in the Western
            United States}",
  journal = aqs,
     year = 2004,
   volume = 66,
   pages = {346-356}
}

@ARTICLE{Woods1997,
   author = {{Woods}, T. N. and {Rottman}, G. J.},
    title = "{Solar Lyman$\alpha$ Irradiance Measurements During Two Solar
            Cycles}",
  journal = jgr,
     year = 1997,
   volume = 102,
    pages = {8769-8780}
}



%====     XXXX    ==============================================================

@ARTICLE{Xu2006,
   author = {{Xu}, Y. and {Cao}, W. and {Liu}, C. and {Yang}, G. and
            {Jing}, J. and {Denker}, C. and {Emslie}, A. G. and {Wang}, H.},
    title = "{High-Resolution Observations of Multiwavelength Emissions During
            Two X-Class White-Light Flares}",
  journal = apj,
     year = 2006,
   volume = 641,
    pages = {1210-1216}
}

@ARTICLE{Xu2005,
   author = {{Xu}, Y. and {Cao}, W. and {Ma}, J. and {Hartkorn}, K. and
            {Jing}, J. and {Denker}, C. and {Wang}, H.},
    title = "{Properties of Small Dark Features Observed in the Pure
            Near-Infrared and Visible Continua}",
  journal = apjl,
     year = 2005,
   volume = 628,
    pages = {167-170}
}

@ARTICLE{Xu2004a,
   author = {{Xu}, Y. and {Yang}, G. and {Qiu}, J. and {Spirock}, T. J. and
            {Jing}, J. and {Denker}, C. and {Wang}, H.},
    title = "{Visible and Near-Infrared Contrast of Faculae in Active Region
            NOAA 8518}",
  journal = chinaa,
     year = 2004,
   volume = 4,
    pages = {481-489}
}

@ARTICLE{Xu2004b,
   author = {{Xu}, Y. and {Cao}, W. and {Liu}, C. and {Yang}, G. and
            {Qiu}, J. and {Jing}, J. and {Denker}, C. and {Wang}, H.},
    title = "{Near-Infrared Observations at 1.56 Microns of the 2003 October 29
            X10 White-Light Flare}",
  journal = apjl,
     year = 2004,
   volume = 607,
    pages = {131-134}
}

@INPROCEEDINGS{Xu2003,
   author = {{Xu}, Y. and {Wang}, H. and {Denker}, C. and {Yang}, G. and
            {Spirock}, T. J. and {Qiu}, J.},
    title = "{Comparison of Facular Contrast in the Visible and Near-Infrared}",
booktitle = {Current Theoretical Models and Future High Resolution Solar
            Observations: Preparing for ATST},
     year = 2003,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 286,
   editor = {{Pevtsov}, A. A. and {Uitenbroek}, H.},
    pages = {201-208}
}



%====     YYYY    ==============================================================

@INPROCEEDINGS{Yang2006a,
   author = {{Yang}, G. and {Varsik}, J. R. and {Shumko}, S. and
            {Denker}, C. and {Choi}, S. and {Wang}, H.},
    title = "{The Telescope Control System of the New Solar Telescope at Big
            Bear Solar Observatory}",
booktitle = {Advanced Software and Control for Astronomy},
   series = posp,
     year = 2006,
   volume = 6274,
   editor = {{Lewis}, H. and {Bridger}, A.},
    pages = {62741Y}
}

@INPROCEEDINGS{Yang2006b,
   author = {{Yang}, G.},
    title = "{Design and Implementation of the Primary and Secondary Mirror
            Control System for NST}",
booktitle = {Advanced Software and Control for Astronomy},
   series = posp,
     year = 2006,
   volume = 6274,
   editor = {{Lewis}, H. and {Bridger}, A.},
    pages = {62740Z}
}

@ARTICLE{Yang2004,
   author = {{Yang}, G. and {Xu}, Y. and {Cao}, W. and {Wang}, H. and
            {Denker}, C. and {Rimmele}, T. R.},
    title = "{Photospheric Shear Flows Along the Magnetic Neutral Line of
            Active Region 10486 Prior to an X10 Flare}",
  journal = apjl,
     year = 2004,
   volume = 617,
    pages = {151-154}
}

@ARTICLE{Yang2003a,
   author = {{Yang}, G. and {Xu}, Y. and {Wang}, H. and {Denker}, C.},
    title = "{High Spatial Resolution Observations of Pores and the Formation
            of a Rudimentary Penumbra}",
  journal = apj,
     year = 2003,
   volume = 597,
    pages = {1190-1199}
}

@INPROCEEDINGS{Yang2003b,
   author = {{Yang}, G. and {Denker}, C. and {Xu}, Y. and {Wang}, H.},
    title = "{Speckle Masking Imaging of Pores in Solar Active Region NOAA
            9439}",
booktitle = {Current Theoretical Models and Future High Resolution Solar
            Observations: Preparing for ATST},
     year = 2003,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 286,
   editor = {{Pevtsov}, A. A. and {Uitenbroek}, H.},
    pages = {317-324}
}

@ARTICLE{Yi1995,
   author = {{Yi}, Z. and {Molowny-Horas}, R.},
    title = "{Correlation Tracking Technique for Measurement of Transverse
            Chromospheric Motions}",
  journal = aa,
     year = 1995,
   volume = 295,
    pages = {199-205}
}

@ARTICLE{Yurchyshyn2006,
   author = {{Yurchyshyn}, V. and {Liu}, C. and {Abramenko}, V. and
            {Krall}, J.},
    title = "{The May 13, 2005 Eruption: Observations, Data Analysis and
            Interpretation}",
  journal = sp,
     year = 2006,
   volume = 239,
    pages = {317-335},
      doi = {10.1007/s11207-006-0177-3}
}



%====     ZZZZ    ==============================================================

@ARTICLE{Zhang2007,
   author = {{Zhang}, J. and {Li}, L. and {Song}, Q.},
    title = "{Interaction between a Fast Rotating Sunspot and Ephemeral Regions
            as the Origin of the Major Solar Event on 2006 December 13}",
  journal = apjl,
     year = 2007,
   volume = 662,
    pages = {L35-L38}
}

@ARTICLE{Zhao2010,
   author = {{Zhao}, J. and {Kosovichev}, A. G. and {Sekii}, T.},
    title = "{High-Resolution Helioseismic Imaging of Subsurface Structures and
            Flows of a Solar Active Region Observed by Hinode}",
  journal = apj,
     year = 2010,
   volume = 708,
    pages = {304-313}
}

@ARTICLE{Zhou2007,
   author = {{Zhou}, G. and {Wang}, J. and {Wang}, Y. and {Zhang}, Y.},
    title = "{Quasi-Simultaneous Flux Emergence in the Events of
            October--November 2003}",
  journal = sp,
     year = 2007,
   volume = 244,
    pages = {13-24}
}

@ARTICLE{Zirin1993,
   author = {{Zirin},  H and {Wang}, H.},
    title = "{Narrow Lanes of Transverse Magnetic Field in Sunspots}",
  journal = nat,
     year = 1993,
   volume = 363,
    pages = {426-428}
}

@BOOK{Zirin1988a,
   author = {{Zirin}, H.},
    title = "{Astrophysics of the Sun}",
booktitle = {Cambridge and New York, Cambridge University Press},
     year = 1988
}

@ARTICLE{Zirin1988b,
   author = {{Zirin}, H. and {Mosher}, J. M.},
    title = "{The Caltech Solar Site Survey, 1965--1967}",
  journal = sp,
     year = 1988,
   volume = 115,
    pages = {183-201}
}

@ARTICLE{Zuccarello2009a,
   author = {{Zuccarello}, F. and {Romano}, P. and {Guglielmino}, S. L. and
            {Centrone}, M. and {Criscuoli}, S. and {Ermolli}, I. and
            {Berrilli}, F. and {Del Moro}, D.},
    title = "{Observation of Bipolar Moving Magnetic Features Streaming out from
            a Naked Spot}",
  journal = aa,
     year = 2009,
   volume = 500,
    pages = {L5-L8}
}

@ARTICLE{Zuccarello2009b,
   author = {{Zuccarello}, F. and {Guglielmino}, S. L. and {Battiato}, V. and 
            {Contarino}, L. and {Spadaro}, D. and {Romano}, P.},
    title = "{Emergence and Evolution of Active and Ephemeral Regions:
            Comparison Between Observations and Models}",
  journal = {Acta Geophys.},
     year = 2009,
   volume = 57,
    pages = {15-23},
      doi = {10.2478/s11600-008-0057-3}
}

@INPROCEEDINGS{Zwaan1992,
   author = {{Zwaan}, C.},
    title = "{The Evolution of Sunspots}",
booktitle = {Sunspots. Theory and Observations},
   series = {NATO ASIC Proc.},
     year = 1992,
   volume = 375,
   editor = {{Thomas}, J. H. and {Weiss}, N. O.},
    pages = {75-100}
}

@ARTICLE{Zwaan1985,
   author = {{Zwaan}, C.},
    title = "{The Emergence of Magnetic Flux}",
  journal = sp,
     year = 1985,
   volume = 100,
    pages = {397-414},
      doi = {10.1007/BF00158438}
}

